Influence Maximization with Spontaneous User Adoption

We incorporate self activation into influence propagation and propose the self-activation independent cascade (SAIC) model: nodes may be self activated besides being selected as seeds, and influence propagates from both selected seeds and self activated nodes. Self activation reflects the real-world scenarios such as people naturally share product recommendations with their friends even without marketing intervention. It also leads to two new forms of optimization problems: (a) {\em preemptive influence maximization (PIM)}, which aims to find $k$ nodes that, if self-activated, can reach the most number of nodes before other self-activated nodes; and (b) {\em boosted preemptive influence maximization (BPIM)}, which aims to select $k$ seeds that are guaranteed to be activated and can reach the most number of nodes before other self-activated nodes. We propose scalable algorithms for PIM and BPIM and prove that they achieve $1-\varepsilon$ approximation for PIM and $1-1/e-\varepsilon$ approximation for BPIM, for any $\varepsilon > 0$. Through extensive tests on real-world graphs, we demonstrate that our algorithms outperform the baseline algorithms significantly for the PIM problem in solution quality, and also outperform the baselines for BPIM when self-activation behaviors are non-uniform across nodes.

==> sec_conclusion.tex <==
%\section{Conclusion} \label{sec:conclude}
%
%In this paper, we study the multi-round influence maximization (MRIM) task, and
%	propose algorithms for solving both the the non-adaptive and adaptive MRIM problems.
%Due to space constraints, we prove theoretically that our algorithms are constant approximation of the optimal solutions in our full technical report \cite{MRIMfull2018}.
%We improve the scalability of the adaptive MRIM algorithm using the state-of-the-art 
%	RR set technique.
%The experimental results demonstrate that our algorithms are effective over the baseline
%	algorithms derived from classical single-round algorithms, and the degree of adaptiveness
%	shows significant effect in improving the influence performance.

%There are several future directions from this research.
%One direction is to design new algorithms to further improve the approximation ratio
%	or the efficiency of the algorithms.
%Another direction is to conduct a thorough study of the online MRIM problem
%	beyond simple heuristic solutions in~\cite{LeiMMCS15}, 
%	following the rigorous theoretical treatment laid 
%	out for the offline MRIM problem.
%Other variants such as competitive multi-round influence maximization may also be explored.

==> sec_method.tex <==
\section{Model and Problem Definition} \label{sec:model}

\wei{Clear explanation of independence of propagation between different rounds, and a node
	activated in previous rounds does not mean it is active in the current round. But when
	consider the overall activation, it is counted once.}

\subsection{Multi-Round Diffusion Model}
In this paper, we focus on the well-studied {\em triggering model} \cite{kempe03}
as the basic diffusion model. 
A social network is modeled as a directed graph $G=(V,E)$, 
where $V$ is a finite set of vertices or nodes, 
and $E \subseteq V \times V$ is the set of 
directed edges connecting pairs of nodes.
%For a node $u \in V$, its outgoing edge $(u,v) \in E$
%or incoming edge $(v,u) \in E$.
The diffusion of information or influence proceeds in discrete time steps $\tau = 0, 1, 2, \dots$. 
%We use $S^{(\tau)}$ %\footnote{We define $S_{-1}=\emptyset$.} 
%    to denotes the set of nodes 
%    that are active at time $\tau$.
At time $\tau=0$, the {\em seed set} $S_0$ is selected to be active, and also 
each node $v$ independently chooses a random {\em triggering set} $T(v)$ 
according to some distribution over subsets of its in-neighbors. 
At each time $\tau\ge 1$, an inactive node $v$ becomes active if at least 
one node in $T(v)$  is active by time $\tau-1$. %($u\in S^{(\tau-1)}$).
The diffusion process ends when there is no more nodes activated in a time step.
We remark that the classical Independent Cascade (IC) model is a special case of the triggering model.
In the IC model, 
    every edge $(u,v) \in E$ is associated with a probability $p_{uv} \in [0, 1]$, 
    and $p_{uv}$ is set to zero if $(u,v) \notin E$.
Each triggering set $T(v)$ is generated by independently sampling $(u,v)$ with probability $p_{uv}$
and including $u$ in $T(v)$ if the sampling of $(u,v)$ is successful.

The triggering model can be equivalently described as propagations in {\em live-edge graphs}.
Given a class of triggering sets $\{T(v)\}_{v\in V}$, we can construct the live-edge graph
$L = (V, E(L))$, where $E(L) = \{(u,v) \mid v\in V, u\in T(v)\}$, and
each edge $(u,v)\in L$ is called a {\em live edge}.
It is easy to see that the propagation in the triggering model is the same as the deterministic
propagation in the corresponding live-edge graph $L$: if $A$ is the set of active nodes
at time $\tau-1$, then all directed out-neighbors of nodes in $A$ will be active
by time $\tau$.
An important metric in any diffusion model is the {\em influence spread},
    the expected number of active nodes when the propagation from the given  
    seed set $S_0$ ends, denoted as $\sigma(S_0)$.
Let $\Gamma(G,S)$ denote the set of nodes in graph $G$ that can be reached from the node set $S$.
Then, by the above equivalent live-edge graph model, we have
$\sigma(S_0) = \E[|\Gamma(L,S_0)|]$, where the expectation is taken over the distribution
of live-edge graphs. 

A set function $f:V\rightarrow \R$ is called {\em submodular} if
for all $S\subseteq T \subseteq V$ and $u \in V\setminus T$, 
$f(S\cup \{u\}) - f(S) \ge f(T \cup \{u\}) - f(T)$.
Intuitively, submodularity characterizes the diminishing return property often occurring
in economics and operation research.
Moreover, a set function $f$ is called {\em monotone} if for all $S\subseteq T \subseteq V$,
$f(S) \le f(T)$.
It is shown in~\cite{kempe03} that influence spread $\sigma$ for the triggering model
is a monotone submodular function .
A non-negative monotone submodular function allows a greedy solution to
its maximization problem subject to a cardinality constraint, with an
approximation ratio $1-1/e$, where $e$ is the base of the natural logarithm~\cite{NWF78}.
This is the technical foundation for most influence maximization tasks.


With the above background settled, we now define the Multi-Round Triggering (MRT) model,
    to study the multi-round diffusion behavior as motivated in the introduction.
The MRT model includes $T$ rounds of influence diffusions, and they are independent among different rounds.
In each round $t \in [T]$, the diffusion starts from a separate seed set $S_t$ with up to $k$ nodes,
    and it follows the dynamic in the classical triggering model described previously.
Since one node can be repeatedly selected as the seed set in different rounds, 
    to clarify the round, we use pair notation $(u, t)$ to denote a node $u$ of the seed set in the $t$-th round.
To be consistent,
    we redefine $S_t$ to be all $(u,t)$ with different $u$.
By the equivalence between the triggering model and the live-edge graph model, 
    the MRT model can be viewed as $T$ independent propagations in the $T$ live-edge graphs $L_1, L_2, \dots, L_T$, 
    which are drawn independently from the same distribution based on the triggering model. 
The total active nodes in $T$ rounds is counted by $\left|\bigcup_{t=1}^T \Gamma(L_t, S_t)\right|$, where $\Gamma(L_t, S_t)$ is the set of final active nodes in round $t$.
%\lichao{The propagation between different rounds is independent, 
%and every node can be activated and affect its neighourhoods in any round.
%However, in the MRT model,  the {\em influence spread} corresponds to the total final number of activation nodes which only counts the activated node once in all rounds, 
%e.g. one node is activated in every round and its final influnce is only one.}
Given a class of seed set $\bS:=\bigcup_{t=1}^TS_t$, the {\em influence spread} $\rho$ in the MRT model is
defined as 
\begin{equation*}
\rho(\bS)=\E\left[\abs{\bigcup_{t=1}^T \Gamma(L_t, S_t)}\right],
\end{equation*}
where the expectation is taken over the distribution of all live-edge graphs 
$L_1, L_2, \ldots, L_T$.




%\begin{definition}\textbf{( Independent Cascade model)} 
%    
%    The independent cascade (IC) model takes the social
%    graph $G=(V,E)$,
%    the influence probability $p(\cdot)$ on all edges, 
%    and the initial seed set $S_0$ as the input, 
%    and generates the active sets $S_t$ for all $t\geq 1$ 
%    by the following randomized operation rule.
%    At every time step $t\geq 1$, 
%    first set $S_t$ to be $S_{t-1}$; 
%    next for every inactive node $ v \notin S_{t-1}$, 
%    for every node $u \in N^{in}(v) \cap (S_{t-1} \setminus S_{t-2})$, 
%    $u$ executes an activation attempt by performing a Bernoulli trial
%    (flipping an independent coin) with success probability $p(u,v)$; 
%    if successful we add $v$ into S$_t$ and
%    say $u$ activates $v$ at time $t$. 
%    If multiple nodes activate $v$ at time $t$ , 
%    the end effect is the same ? $v$ is added to $S_t$.
%\end{definition}


\subsection{Multi-Round Influence Maximization}

The classical influence maximization problem is to choose a seed set $S_0$ of size at most $k$
to maximize the influence spread $\sigma(S_0)$. %, in the classical triggering model.
For the Multi-Round Influence Maximization (MRIM) problem, the goal is to select at most $k$ seed nodes of each
round, such that the influence spread in $T$ rounds is maximized.
We first introduce its non-adaptive version formally defined as follows.

\begin{definition}
	The {\em non-adaptive} Multi-Round Influence Maximization (MRIM) under the MRT model
	is the optimization task where
	the input includes the directed graph $G=(V,E)$, the triggering set distribution for every node
	in the MRT model, the number of rounds $T$, and each-round budget $k$, and the goal
	is to find $T$ seed sets $S_1^*$, $S_2^*$, \dots, $S_T^*$ with each seed set having at most
	$k$ nodes, such that the total influence spread is maximized, i.e.,
	\begin{equation*}
		\bS^* = S_1^* \cup \dots\cup S_T^* = \argmax_{\bS: |S_i| \leq k} \rho(\bS).
	\end{equation*}
\end{definition}
The non-adaptiveness refers to the definition one needs to find $T$ seed sets all at once
before the propagation starts.
In practice, one may be able to observe the propagation results in previous rounds and
select the seed set for the next round based on the previous results to increase the influence spread.
This leads to the adaptive version.
To formulate the {\em adaptive} MRIM requires the setup of the 
adaptive optimization framework, and we defer to Section~\ref{sec:AMRIMDef} for
its formal definition.

We remark that in both the non-adaptive and adaptive versions, the seed sets in different
rounds are not necessarily different.
In fact, in many cases it is important to repeatedly select influential nodes in multiple
rounds to achieve better total influence spread.
This is qualitatively different from the classical one-round influence maximization, 
where it makes no sense to select one node multiple times as seeds.
On the other hand, always selecting the same seed set may not be desirable either.
Our experimental results will also demonstrate that algorithms specifically designed
for MRIM perform significantly better than the algorithms both simply 
	selecting $Tk$ seeds and repeatedly selecting the same $k$ seeds
	over all $T$ rounds using classical single-round algorithms.
This indicates that an independent
study of MRIM is important.
Note that the classical influence maximization is a special case of MRIM with
$T=1$.



\section{Non-Adaptive MRIM} \label{sec:nonadaptive}

\wei{explain the submodularity of node-round pairs. Explain partition matroid constraint, and
show our MRIM problem is an instance of submodular maximization under matroid constraint.}

We now study the non-adaptive MRIM problem.
Since the traditional influence maximization problem is a special case, the non-adaptive MRIM problem is also NP-hard.
We overcome the NP-hardness by designing approximation algorithms exploiting the property
of the influence model.
\lichao{modified}
Non-adaptive MRIM has cross-round and within-round settings for seed selection in multiple rounds, and
we are going to talk about these two different settings in this section.

\subsection{Cross-Round Non-adaptive MRIM}

For cross-round non-adaptive MRIM problem, 
each time we can select a node from any round to maximize the influence while at most $k$ seeds are selected for each round.
The cross-round non-adaptive MRIM problem is NP-hard.
We overcome the NP-hardness by designing approximation algorithms exploiting the property
of the influence model.
In particular, we find that the MRT model exhibits the interesting {\em cross-round-submodular}
property, as we now explain.

Let $\bS = \{(u, t) | u \in V, t \in [T]\}$.
The number of node-round pairs in any round $t \in [T]$ is at most $k$.
We also focus the $i$-th seed node pair $(u, t')$ by using the notation $\bS = ( (u, t'), \bS_{-i})$, 
where $\bS_{-i}$ is the vector excluding the $i$-th node in $\bS$.
In the MRT model, we first notice that when we fix other sets $\bS_{-i}$ and view
$\rho$ as a set function for $(u,t')$, by a similar reasoning as the classical
triggering model, we can show that $\rho ( (u, t'), \bS_{-i})$ as a function of $(u, t')$
is monotone and submodular.
For any two $\bS^A=\{(u, t)^A\}$ and $\bS^B=\{(u, t)^B\}$, we say $\bS^A \subseteq \bS^B$ if the node $(u, t') \in \bS^A$,
then $(u, t') \in \bS^B$.

\begin{restatable}{lemma}{outersubmodular} \label{lem:outersubmodular}
	Influence spread $\rho(\bS)$ for the cross-round MRT model is monotone and submodular when treating
	$\bS$ as a node-round pair set, namely,
	(a) Monotonicity: For any $\bS^A \subseteq \bS^B$, we have $\rho(\bS^A)\leq\rho(\bS^B)$;
	and (b) Submodularity: 
	For any $\bS^A \subseteq \bS^B$ and any available node $(u, t) \in \cV$ that means the total number of chosen seeds of $t$-th round is less than $k$ , we have $\rho(\bS^A,(u, t))-\rho(\bS^A) \geq \rho(\bS^B, (u, t))-\rho(\cS^B)$.
\end{restatable}

%The above result shows that in the MRT model, influence spread $\rho$ is both monotone and submodular
%for each global set $\cS$.
%With above setting, 

However, the cross-round non-adaptive MRT is also a partition matroid model.
$\cV$ is a non-empty collection of disjoint sets of $V$, also called independent sets,
which have the property that $S^B \in \cV$, 
and $S^A \subset \cV$ implies $S^B \in \cV$. 
The independent sets $\cV$ forms a matroid $M = (V, \cV)$.
Since the limitation of each round $k$ is between 0 and $|\cV|$,
and $S_i '$ for each round.


Every seed set $S_i$ is independent with at most k seeds where $0 \leq k \leq |V|$. 
Then the sets that are independent sets in this way form the independent sets of a matroid, 
called a partition matroid.
The seed sets $S_i$ are called the blocks of the partition matroid.

\begin{lemma} \label{lem:pm}
	While cross-round MRT is a partition matroid setting and $\rho(\cdot)$ holds monotone and submodular properties,
	the greedy Influence spread $\rho(\bS^g)$ is at least $\frac{1}{2}$ of optimal solution $\rho(\bS^*)$.
\end{lemma}

We refer to this as the {\em global-submodular} property.
Based on this property, we design a greedy algorithm {\em GlobalGreedy} as shown in
Algorithm~\ref{alg:globalgreedy}.
The loop of the algorithm is to greedily select $Tk$ nodes,
the best $\cS^g$ is achieved by a greedy approximation 
in the loop, hence the name of {\em GlobalGreedy}.

%\begin{algorithm}[t]
%	%\SetKwComment{tcp}{\tiny // }{}%
%	\caption{{\em GlobalGreedy}: Greedy algorithm for the global non-adaptive MRIM} \label{alg:globalgreedy}
%	\KwIn{Graph $G=(V,E)$, integers $T$ and $k$, triggering set distributions, $\cV$ is set with $k$ copies of $V$: $\cV = \{V_i\}$ }
%	\KwOut{$\cS^g = \{u_i^g\}$.}
%	
%	Set $\cS^g$ to the empty set $\emptyset$\;
%	\For{$i = 1, 2, \dots, Tk$}{ 
%		for all $u_i\in \cV\setminus \cS^g$, simulate $R$ times the diffusion process
%		for seed sets $\cS^g \cup \{u_i\}$ to obtain
%		influence spread estimate $\hat{\rho}(\cS^g\cup \{u\} )$\;
%		\label{line:simulate}
%		$v_{i} \leftarrow \argmax_{u\in V\setminus \cS^g} \hat{\rho}(\cS^g \cup \{u_i\} )$\; %-\rho(S_1,S_2,\dots,S_i)$
%		$\cS^g \leftarrow \cS^g \cup \{v_{i}\}$\;
%	}
%	\textbf{return} $\cS^g = \{u_i^g\}$.
%\end{algorithm}

Because the global greedy structure of the algorithm, we have the following
guarantee for the algorithm.

\begin{theorem} \label{thm:globalnonadaptive}
	Let $\cS^*$ be the optimal solution of the global MRIM problem.
	For every $\varepsilon > 0$ and every $\ell > 0$, with probability at least
	$1-\frac{1}{n^\ell}$, the output $\cS^g$ of the {\em GlobalGreedy} algorithm 
	satisfies
	\begin{equation}
	\rho(\cS^g) \geq \left(\frac{1}{2} - \varepsilon\right) \rho(\cS^*),
	\end{equation}
	if each estimate $\hat{\rho}()$
	uses $R=\lceil 31 k^2n\log(2kn^{\ell+1} T)/\varepsilon^2 \rceil$ simulations.
	In this case, the total running time is $O(k^3\ell Tn^2m\log(n T)/\varepsilon^2)$, 
	assuming each simulation finishes in $O(m)$ time.
\end{theorem}
\begin{proof}[Proof (Sketch)]
	The proof follows the same structure as the proof of Theorem 3.7 in~\cite{chen2013information}, but
	it needs to accommodate the new double greedy algorithm structure and the double submodular
	property.
	let $\varepsilon_1 = e^{(1-1/e)} \varepsilon/2$.
	From the inner-submoduarlity property of the MRT model and 
	the proof of Theorem 3.7 in~\cite{chen2013information} based on the Chernoff bound,
	we can conclude that when $R\ge \lceil 27 k^2n\log(2kn^{\ell+1} T)/\varepsilon_1^2 \rceil$,
	for each round $i \in [T]$, with probability at least $1- \frac{1}{n^\ell T}$, 
	the seed set $S_i^g$ found by {\DoubleGreedy} is a $(1-1/e - \varepsilon_1)$ approximation
	of the optimal solution for round $i$ maximizing the marginal gain of
	$\rho(S_1, \ldots, S_{i-1}, S) - \rho(S_1, \ldots, S_{i-1}) $.
	Using the union bound, we know that with probability at least $1- \frac{1}{n^\ell}$,
	for all $i\in [T]$ seed set $S_i^g$ is an $(1-1/e - \varepsilon_1)$ approximation
	of the optimal solution for round $i$.
	
	Now at each greedy step, if the new item found is not the one giving the best marginal contribution
	but an $\alpha$ approximation of the optimal marginal solution, an easy extension of
	\cite{NWF78}, already reported in~\cite{GS07}, show that the greedy algorithm can give
	a $1-e^{-\alpha}$ approximate solution to the sumodular maximization problem.
	In our case, consider the outer level when treating each subset $S_i$ as an item, Lemma~\ref{lem:outersubmodular} shows that $\rho$ is also submodular in this case 
	(the outer-submodularity), and we just argued in the previous paragraph that
	in each round, the selected $S_i^g$ is a $(1-1/e - \varepsilon_1)$ approximation.
	Therefore, the final output $\cS^g = (S_1, \ldots, S_g)$ satisfies
	\begin{equation*}
		\rho(\cS^g) \ge (1-e^{-(1-1/e-\varepsilon_1)}) \rho(\cS^*).
	\end{equation*}
	Because $\varepsilon_1 = e^{(1-1/e)} \varepsilon/2$, it is easy to verify that 
	$1-e^{-(1-1/e-\varepsilon_1)} \ge 1-e^{-(1-1/e)} - \varepsilon$ in this case, and
	it is sufficient to have $R=\lceil 31 k^2T^2n\log(2kn^{\ell+1} T)/\varepsilon^2 \rceil$.
	Finally, the total running time is simply 
	$O(TknRm) = O(k^3\ell T^3n^2m\log(n T)/\varepsilon^2)$.
\end{proof}



\subsection{Within-Round MRIM}

\weiran{the following is pasted from section 2.1.}
Note that the order of the sets $S_1, S_2, \ldots, S_T$ does not matter, and $\rho$
is only determined by the nonempty sets, so we can equivalently view $\rho$
as a set function over a set of subsets of $V$, $\{S_1, S_2, \ldots, S_T\}$.
However, since we allow subsets to repeat, $\{S_1, S_2, \ldots, S_T\}$ is a multi-set.
which also can be represented by the pairs with round $\{(u,t) | u \in V, t \in [T]\}$.
Sometimes, we choose to use its vector representation for convenience.

In particular, we find that the MRT model exhibits the interesting {\em double-submodular}
property, as we now explain.

Let $\cS = (S_1, \ldots, S_T)$. 
When focusing on one subset $S_i$, we also use the notation $\cS = (S_i, \cS_{-i})$, 
where $\cS_{-i}$ is the vector excluding the $i$-th entry in $\cS$.
In the MRT model, we first notice that when we fix other sets $\cS_{-i}$ and view
$\rho$ as a set function for $S_i$, by a similar reasoning as the classical
triggering model, we can show that $\rho(S_i, \cS_{-i})$ as a function of $S_i$
is monotone and submodular.
Moreover, as we mentioned earlier, we can also treat $\cS = (S_1, \ldots, S_T)$ as
a multi-set of subsets, ignoring all empty subsets among $S_i$'s. 
The following lemma shows that $\rho$ is also monotone and submodular when viewed
as a function of multi-set of subsets.
For any two $\cS^A=(S_1^A, \dots, S_t^A)$ and $\cS^B=(S_1^B, \dots, S_t^B)$, we say $\cS^A \subseteq \cS^B$ if either $S^A_i = S^B_i$ or $S^A_i = \emptyset$ holds for every $i\in[t]$,
which means $\cS^B$ includes $\cS^A$ when treating them as multi-sets.

\begin{lemma} \label{lem:outersubmodular}
	Influence spread $\rho(\cS)$ for the MRT model is monotone and submodular when treating
	$\cS$ as multi-sets, namely,
	(a) Monotonicity: For any $\cS^A \subseteq \cS^B$, we have $\rho(\cS^A)\leq\rho(\cS^B)$;
	and (b) Submodularity: 
	For any $\cS^A \subseteq \cS^B$ and any $S_{t+1}\subseteq V$, we have $\rho(\cS^A,S_{t+1})-\rho(\cS^A) \geq \rho(\cS^B,S_{t+1})-\rho(\cS^B)$.
\end{lemma}
\begin{proof}
	The proof of monotonicity is straightforward, so we next consider submodularity.
	According to the definition of the influence spread, we have
	\begin{align*}
		&\rho(\cS^A,S_{t+1})-\rho(\cS^A) \geq \rho(\cS^B,S_{t+1})-\rho(\cS^B) \\
		&\Leftrightarrow \E[|\cup_{i=1}^t \Gamma(L_i,S_i^A) \cup \Gamma(L_{t+1},S_{t+1})|] - \E[|\cup_{i=1}^t \Gamma(L_i,S_i^A)|] \\
		& \geq  \E[|\cup_{i=1}^t \Gamma(L_i,S_i^B) \cup \Gamma(L_{t+1},S_{t+1})|] - \E[|\cup_{i=1}^t \Gamma(L_i,S_i^B)|].
	\end{align*}
	%	If we can prove that for any fixed $L_1, L_2, \dots, L_{T+1}$, the following holds, then the above also holds.
	%	\begin{align*}
	%		& |\cup_{i=1}^T \Gamma(L_i,S_i^A) \cup \Gamma(L_{T+1},S_{T+1})| - |\cup_{i=1}^T \Gamma(L_i,S_i^A)| \\
	%		& \geq  |\cup_{i=1}^T \Gamma(L_i,S_i^B) \cup \Gamma(L_{T+1},S_{T+1})| - |\cup_{i=1}^T \Gamma(L_i,S_i^B)|
	%	\end{align*}
	Then it is sufficient to show that
	\begin{align}\label{proofeq:1}
		& \cup_{i=1}^t \Gamma(L_i,S_i^A) \cup \Gamma(L_{t+1},S_{t+1}) \setminus \cup_{i=1}^t \Gamma(L_i,S_i^A) \nonumber\\
		& \supseteq  \cup_{i=1}^t \Gamma(L_i,S_i^B) \cup \Gamma(L_{t+1},S_{t+1}) \setminus \cup_{i=1}^t \Gamma(L_i,S_i^B).
	\end{align}
	
	For any node $u \in \cup_{i=1}^t \Gamma(L_i,S_i^B) \cup \Gamma(L_{t+1},S_{t+1}) \setminus \cup_{i=1}^t \Gamma(L_i,S_i^B)$, 
	$u$ is reachable from $S_{t+1}$ in $L_{t+1}$, 
	but not reachable from $S_{i}^B$ in $L_{i}$ for any $i\in[t]$.
	Since $\cS^A_T\subseteq \cS^B_T$, $S_i^A = S_i^B$ or $S_i^A = \emptyset$, for any $i\in[t]$. 
	Thus $u$ is also not reachable from $S_{i}^A$ in $L_{i}$ for any $i\in[t]$.
	Therefore, we conclude that $u \in \cup_{i=1}^t \Gamma(L_i,S_i^A) \cup \Gamma(L_{t+1},S_{t+1}) \setminus \cup_{i=1}^t \Gamma(L_i,S_i^A)$.
	Thus the submodularity holds.
	%    
	%    This implies that $u$ is reachable from $(S_x,x)$ under $\phi_B$. 
	%    Since $\cE_A \subseteq \cE_B$ and $\phi_A = \phi_B$, 
	%    Under a realization $\phi_A$, it must be the case that $u$ is not reachable from $\cE_A$ 
	%    but is reachable from $\cE_A \cup (S_x,x)$, 
	%    and thus $u \in \bigcup_{S \in \cE_A \cup x} \Gamma(L_S, S) \setminus \bigcup_{S \in \cE_A} \Gamma(L_S, S) $.
	%    Thus, function $|\bigcup \Gamma(\cdot) |$ is submodular, which means $\rho(\cdot)$ is submodular.
	%    \begin{align}
	%    & \rho(\cE_A \cup (S_x,x)) - \rho(\cE_A) \geq \rho(\cE_B \cup (S_x,x)) - \rho(\cE_B).\label{eq:a1} \\
	%    & \Leftrightarrow  \nonumber \\ 
	%    & \E\left[ \left|\bigcup_{S \in \cE_A \cup (S_x,x)} \Gamma(L_S, S) \right| \right] 
	%    - \E \left[ \left|\bigcup_{S \in \cE_A} \Gamma(L_S, S) \right| \right] \\
	%    & \geq \E \left[\left|\bigcup_{S \in \cE_B \cup (S_x,x)} \Gamma(L_S, S) \right| \right] 
	%    - \E\left[ \left|\bigcup_{S \in \cE_B} \Gamma(L_S, S) \right| \right]  \label{eq:a2} \\
	%    & \Leftarrow \nonumber \\ 
	%    & \forall L_S \mbox{ with } S \in \cE_B \cup (S_x,x), \\
	%    & \left|\bigcup_{S \in \cE_A \cup (S_x,x)} \Gamma(L_S, S) \right| 
	%    - \left|\bigcup_{S \in \cE_A} \Gamma(L_S, S) \right| \\
	%    & \geq \left|\bigcup_{S \in \cE_B \cup (S_x,x)} \Gamma(L_S, S) \right| 
	%    - \left|\bigcup_{S \in \cE_B} \Gamma(L_S, S) \right|  \label{eq:a3}
	%    \end{align}
	%    
	%    We want to prove the Equation \ref{eq:a1}, but it is not straightforward.
	%    Then, we can prove the Equation \ref{eq:a2} which takes expectation on both sides of the function,
	%    and it is equivalent with Equation \ref{eq:a1}.
	%    Equation \ref{eq:a3} is sufficient to Equation \ref{eq:a2}, so we can prove Equation Equation \ref{eq:a3} works, then
	%    Equation \ref{eq:a2} works.
	%    
	%    Now, we want to prove the Equation Equation \ref{eq:a3}.
	%    In RIC model, each time we have a random live-edge graph
	%    and we find the best set of seeds from the graph. 
	%    We apply couple live-edge graph strategy to prove the Equation 6 works.
	%    For super multi-sets $\cE_A$ and $\cE_B$, we have two realization $\phi_A$ and $\phi_B$.
	%    However, we let two realizations are same, 
	%    then we have two live-edge graph sets $\mathcal{L_A} = \mathcal{L_B} = \{L_1, L_2, ..., L_T\}$.
	%    
	%    By the definition of submodularity, 
	%    it is sufficient to show that for any two subsets $\cE_A \subseteq \cE_B \subseteq \mathcal{O}$,
	%    and a set $x \in \mathcal{O} \setminus \cE_B$, we have:
	%    
	%    \begin{align}
	%    & \forall L_S \mbox{ with } S \in \cE_B \cup (S_x,x),  
	%    \bigcup_{S \in \cE_A \cup (S_x,x)} \Gamma(L_S, S) \setminus \bigcup_{S \in \cE_A} \Gamma(L_S, S) \\
	%    & \supseteq  \bigcup_{S \in \cE_B \cup (S_x,x)} \Gamma(L_S, S) \setminus \bigcup_{S \in \cE_B} \Gamma(L_S, S) \label{eq:a4}
	%    \end{align}
	%        
	% Now, we want to show Equation  with coupled strategy to prove Equation 5 and 4.
	% If we take expectation with $\mathcal{L_B}$ on both sides of Equation 6, the left
	% hand side(LHS) is same with LHS of Equation 5. 
	% Since $\mathcal{L_A}$ is coupled with $\cE_B$, we first take expectation with  $\mathcal{L_A}$
	% on right hand side(RHS), the result is same with RHS of Equation 5. Then, we take
	% expectation with $\mathcal{L_B} \setminus \mathcal{L_A}$ on RHS, 
	% we have the same result since the value of RHS after expectation with $\mathcal{L_A}$ is a constant.
	% Now, we prove Equation 6 is sufficient for Equation 5 with coupled condition.
	% Since Equation 5 is equivalent with Equation 4, we prove the Equation 4 is submodular.
	%    
\end{proof}

The above result shows that in the MRT model, influence spread $\rho$ is both submodular
for each individual set $S_i$ ({\em inner-submodularity}) and submodular for the multi-set of subsets
	({\em outer-submodularity}).
We refer to this as the {\em double-submodular} property.
Based on this property, we design a greedy algorithm {\DoubleGreedy} as shown in
Algorithm~\ref{alg:greedy}.
The inner loop of the algorithm is to greedily select $k$ nodes for round $i$, while
the outer loop is to iterate through the $T$ rounds.
The outer loop can be viewed as the outer-level greedy algorithm trying to select
the best $k$ seeds of the next round, and it is achieved by a greedy approximation 
in the inner loop, hence the name of {\DoubleGreedy}.

\begin{algorithm}[t]
	%\SetKwComment{tcp}{\tiny // }{}%
	\caption{{\DoubleGreedy}: Greedy algorithm for the non-adaptive MRIM} \label{alg:greedy}
	\KwIn{Graph $G=(V,E)$, integers $T$ and $k$, triggering set distributions.}
	\KwOut{$\cS^g = (S_1^g, S_2^g, \dots, S_T^g)$.}
	
	Set $S_1^g, S_2^g, \dots, S_T^g$ to the empty set $\emptyset$\;
	\For{$i = 1, 2, \dots, T$}{ 
		\For{$j = 1, 2, \dots, k$}{
			for all $u\in V\setminus S_i^g$, simulate $R$ times the diffusion process
			for seed sets $S_1^g, \ldots, S_{i-1}^g$, and $S_{i}^g \cup \{u\}$ to obtain
			influence spread estimate $\hat{\rho}(S_1^g, S_2^g, \dots, S_i^g\cup \{u\} )$\;
			\label{line:simulate}
			$v_{i,j} \leftarrow \argmax_{u\in V\setminus S_i^g} \hat{\rho}(S_1^g, S_2^g, \dots, S_i^g\cup \{u\} )$\; %-\rho(S_1,S_2,\dots,S_i)$
			$S_i^g \leftarrow S_i^g \cup \{v_{i,j}\}$\;
		}
	}
	\textbf{return} $\cS^g = (S_1^g, S_2^g, \dots, S_T^g)$.
\end{algorithm}



%====
%
%Totally, we have $T$ rounds, and in the $i$-th round, 
%the propagation starts with a seed set $S_i$, and after the propagation ends
%the set of influenced nodes is denoted as $V(\Phi_i(S_i))$.
%Equivalently, we can think of it as generating a random live-edge graph $L_i$, and then 
%$V(\Phi_i(S_i)) = \Gamma(L_i, S_i)$, that is, $V(\Phi_i(S_i))$ is a random realization that
%the set of nodes that can be reached from seed set $S_i$ through the random live-edge graph $L_i$
%in $i$-th round.
%
%We have $\cE = \{(S_1, 1), \ldots, (S_T, T)\}$ in $T$ rounds. 
%For brevity we will assume $\cS = \{S_1, \ldots, S_T\}$, which is a multi-set of subsets of $V$, 
%i.e., $S_i$ can be $S_j$ when $i \neq j$ and $i,j \leq T$.
%The total influence (rewards) is the union of all activated nodes (including initial seeds) from all $T$ rounds, 
%and is defined as 
%
%\begin{align*}
%    &V(\Phi(\cE)) =	V(\Phi_{(L_1,\ldots, L_T) \sim \cL^T}(\cS)) \\
%    & = V(\Phi_{(L_1,\ldots, L_T) \sim \cL^T}(\{S_1, S_2, \ldots, S_T\}))\\
%    & = \bigcup_{i=1}^T  V(\Phi_{L_i}(S_i)).
%\end{align*}
%
%The total influence spread is the expected size of total influence set, that is,
%\begin{align}
%    \rho(\cE) = \rho(\cS) 
%    & =  \E[|V(\Phi(\cE))|] \\
%    &= \E[|V(\Phi_{(L_1,\ldots, L_T) \sim \cL^T}(\cS))|] \\
%    &= \E \left[ \left | \bigcup_{i=1}^T  V(\Phi_{L_i}(S_i))  \right | \right]\\
%    &= \E_{(L_1,\ldots, L_T) \sim \cL^T}\left[ \left | \bigcup_{i=1}^T \Gamma(L_i, S_i)  \right |  \right].
%\end{align}
%
%
%%RIC is just the same as IC model: to selects up to $k$ seeds in the graph $G$.
%%Finally, RIC returns the best union result 
%%$\mathcal{S^*} = ({S^1}^*, {S^2}^*, ..., {S^N}^*$).
%%Note that IC model is a special case of RIC model when $N = 1$.
%%The technical definition of RIC is given below.
%
%% \begin{definition}\textbf{(Repeative Independent cascade model)} 
%% The repeative independent cascade (RIC) model takes the social
%% graph $G=(V,E)$, the influence probability $p(.)$ on all edges.
%% and the initial seed set, $\cS = ({S^1}, {S^2}, ..., {S^N}$) as the input, 
%% and generates the active set $\cS_0 = (S^0_{t^0}, S^1_{t^1}, ..., S^N_{t^N}$) 
%% for each $t^i \geq 1$, $i \in [N]$, 
%% by the following randomized operation rule.
%% In the $i$-th repeat time, at every time step $t^i\geq 1$,
%% first set $S^i_{t^i}$ to be $S^i_{t^i-1}$; 
%% next for every inactive node $ v \notin S^i_{t-1}$, 
%% for every node $u \in N^{in}(v) \cap (S^i_{t^i-1} \setminus S^i_{t^i-2})$, 
%% $u$ executes an activation attempt by performing a Bernoulli trial
%% (flipping an independent coin) with success probability $p(u,v)$; 
%% if successful we add $v$ into $S^i_{t^i}$ and
%% say $u$ activates $v$ at time $t^i$. 
%% If multiple nodes activate $v$ at time $t^i$ , 
%% the end effect is the same ? $v$ is added to $S^i_{t}$.
%% When $i = 1$, the input and the output of RIC is same as IC.
%% \end{definition}
%
%%In RIC model, the influence diffusion process is different with
%%IC model. To achieve the goal of a viral marketing campaign with IC,
%%we need to model the new influence diffusion process with RIC model,
%%and to design an efficient way of identifying which nodes to
%%target in the network with RIC model.
%%
%%We first introduce the notations of RIC model. 
%%$S_i$ denotes a unique seed set with $k$ seeds. 
%%If $S_i = S_j$, we have two sets with same seeds.
%%Due to $S_i$ is a unique seed set, if $i \neq j$
%%$S_i \neq S_j$. 
%%In RIC, we will repeat to select $k$ seeds.
%%The key things we need to know is that we can 
%%select same seed set as previous with the greedy algorithm.
%%Then, we use $\cS = \{(S_1,1),(S_1,2),...,(S_i,n)\}$ to represent
%%all the seed sets we choose, where $(S_i, n)$: $S_i$ is the unique seed sets,
%%and $n$ is the number of times of $S_i$ is selected. 
%%We name $\cS$ as super multi-set, 
%%where all elements are set of seeds which can be repeated.
%%For example, $(S_3, 5)$ represent the $5$-th time $S_3$ is selected.
%%Note that, if $(S_3, 5) \in \cS$, 
%%definitely we have $(S_3, i) \in \cS$, where $1 \leq i \leq 4$.
%%$\cA$ and $\cB$ are two super multi-sets. 
%%If $\cA \subseteq \cB$, any $(S_i,n) \in \cA$, 
%%then $(S_i,n) \in \cB$. 
%%About $\cE_B \setminus \cA$, 
%%we need to remove the repeated sets from $\cA$ in $\cE_B$.
%%$|S_i|_A$ denotes the total repeated times in $\cA$, 
%%and $|S_i|_B$ denotes the total repeated times in $\cE_B$.
%%When $S_i \in \cA$ and $S_i \in \cE_B$,
%%if $|S_i|_B - |S_i|_A > 0$, 
%%$(S_i, n), where \; n \in [|S_i|_B - |S_i|_A], \in \cE_B \setminus \cA$.
%%Otherwise, $(S_i, n), where \; n \geq 1, \notin \cE_B \setminus \cA$.
%%$\rho(.)$ is the influence function of RIC, 
%%e.g. $\rho(\cA)$ represent the all the influenced seeds when we repeat to choose
%%set of seeds as $\cA$. $\rho(\cA)$ is defined as below:
%%
%%\begin{equation}
%%\rho(\cA) =  \sum_{L \in \mathcal{L}} Pr(L_1)Pr(L_2)...Pr(L_{T}) \left|\bigcup_{(S,n) \in \cA} \Gamma(L_S, S) \right| 
%% = \E\left[ \bigcup_{(S,n) \in \cA} \Gamma(L_S, S) \right]
%%\end{equation}
%%
%%where $T = |\cA|$, 
%%$\mathcal{L}$ is a set contains all live-edge graph with each repeated seeds selection,
%%and $\Gamma(L_S, S)$ denotes the influenced seeds with live-edge graph $L_S$ 
%%with the $n$-th seed set of $S$. 
%
%\begin{problem}\label{prob:im} \textbf{(Influence maximization on RIC model)} 
%    is the following stochastic optimization problem: 
%    Given a social graph $G = (V,E)$ 
%    with influence probability $p(u,v) \;or\; p_{uv}\in [0,1]$
%    on every edge $(u,v) \in E$,
%    a stochastic diffusion model on $G$, and a budget with $T$ total repeat rounds
%    and $k$ maximum seeds of each round.
%    To find the best items $\cE$ is equivalent to find the best $dom(\cE) = S$,
%    a multi-set of seed sets $\cE^* \Leftrightarrow \cS^* = \{S_1^*, S_2^*, \ldots, S_T^*\}$ 
%    with $|S_i| \leq k$,
%    such that the total influence spread $\rho(\cS)$ under the RIC model is maximized. That is, 
%    compute $\cS^* = \{S_1^*, S_2^*, \ldots, S_T^*\}$ such that
%    \begin{equation}
%    \mathcal{S^*} =  \{S_1^*, S_2^*, \ldots, S_T^*\} = \argmax_{\cS=\{S_1, S_2, \ldots, S_T\}: |S_i| \leq k} \rho(\cS).
%    \end{equation}
%\end{problem} 
%
%Similar to IC, RIC is also computationally hard.
%
%To solve this problem, we need to prove two important properties
%in terms of the influence spread function $\rho (\cdot)$:
%submodularity and monotonicity. 
%Before proving submodularity and monotonicity,
%we need to introduce some basic properties in our problem.
%
%Both definitions of submodularity and monotonicity are introduced
%in the appendix.
%
%Before we prove the monotonicity and submodularity
%of $\rho(\cdot)$ of RIC, we first introduce the notations of RIC model.
%First, let assume two sets with $T$ items $\cE_A$, and $\cE_B$, 
%where $\cE_A = {(S^A_1,1), \ldots, (S^A_T, T)}$,  $\cE_B = {(S^B_1,1), \ldots, (S^B_T, T)}$ and $\cE_A \subseteq \cE_B$.
%If $\cE_A \subseteq \cE_B$ and we have $(S^A_i,i) \in \cE_A$ and $(S^B_i, i) \in \cE_B$ in $i$-th round, 
%$S^A_i = S^B_i$ or $S^A_i = \emptyset$.


% $\cS$ is a multi-set of seed sets, 
% where each elements is set with $k$ seeds and can be repeated.
% $\cA$ and $\cE_B$ are two super multi-sets. 
% If $\cA \subseteq \cE_B$, any $S_i \in \cA$,
% we must have $S_i \in cB$, 
% and $count_{\cA}(S_i) \leq count_{\cE_B}(S_i)$
% About $\cE_B \setminus \cA$, 
% we need to remove the repeated sets from $\cA$ in $\cE_B$.
% $|S_i|_A$ denotes the total repeated times in $\cA$, 
% and $|S_i|_B$ denotes the total repeated times in $\cE_B$.
% When $S_i \in \cA$ and $S_i \in \cE_B$,
% if $|S_i|_B - |S_i|_A > 0$, 
% $(S_i, n), where \; n \in [|S_i|_B - |S_i|_A], \in \cE_B \setminus \cA$.
% Otherwise, $(S_i, n), where \; n \geq 1, \notin \cE_B \setminus \cA$.
% $\rho(.)$ is the influence function of RIC, 
% e.g. $\rho(\cA)$ represent the all the influenced seeds when we repeat to choose
% set of seeds as $\cA$.

%\begin{theorem}The influence spread function $\rho (.)$ in
%    RIC model is monotone and submodular(double-submodular).
%\end{theorem}
%
% The monotonicity of RIC model is straightforward.
%    
%    % Then, we need to prove its submodularity.
%    % Here, we will introduce a new definition called double-submodularity. the we need to prove double-submodularity.
%    % Double-submodularity contains first-order submodularity and second-order-submodularity.
%    % First-order submodular want to prove that in $i$-th repeat time,
%    % the influence spread function $\rho _f(.)$ is submodular and monotone when we have
%    % $k$ budget. Since repeat time of RIC model is same as IC model,
%    % the influence spread function in IC model is submodular and monotone,
%    % so the first-order influence spread function in RIC is also submodular and monotone.
%    
%    Here, we start to prove the submodularity $\rho(.)$ in RIC model.
%    $\cE_A$ and $\cE_B$ are two item sets. 
%    Here, we have $\cE_A \subseteq \cE_B \subseteq \mathcal{E_{ALL}}$.
%    and $(S_x,x) \in \mathcal{E_{ALL}} \setminus \cE_B$, which means $(S_x,x) \notin \cE_B$.
%    It also means, in $x$-th round, $S^B_x = \emptyset$.
%    To prove the submodularity $\rho(.)$,
%    and we want to prove $\rho(\cE_A \cup (S_x,x)) - \rho(\cE_A) \geq \rho(\cE_B \cup (S_x,x)) - \rho(\cE_B)$.
%    
%    ====
%    
%Due to the hardness of RIC model, non-adaptive influence maximization of RIC is also hard to compute.
%Then, we introduce a greedy approach to partly overcome the combinatorial source of hardness, 
%and use Monte Carlo simulations to overcome the influence computation source of hardness.
%
%The greedy algorithm may not perform well in general, but when set function $f$ is monotone
%and submodular, it provides an approximation guarantee, as shown by the following classic
%theorem. Since this is a crucial theorem for our algorithm design, we reproduce the proof below.

Because the logical double greedy structure of the algorithm, we have the following
guarantee for the algorithm.

\begin{theorem} \label{thm:nonadaptive}
Let $\cS^*$ be the optimal solution of the MRIM problem.
For every $\varepsilon > 0$ and every $\ell > 0$, with probability at least
	$1-\frac{1}{n^\ell}$, the output $\cS^g$ of the {\DoubleGreedy} algorithm 
satisfies
\begin{equation}
\rho(\cS^g) \geq \left(1 - e^{-(1-\frac{1}{e}) } - \varepsilon\right) \rho(\cS^*),
\end{equation}
if each estimate $\hat{\rho}()$
 uses $R=\lceil 31 k^2n\log(2kn^{\ell+1} T)/\varepsilon^2 \rceil$ simulations.
 In this case, the total running time is $O(k^3\ell Tn^2m\log(n T)/\varepsilon^2)$, 
 	assuming each simulation finishes in $O(m)$ time.
\end{theorem}
\begin{proof}[Proof (Sketch)]
The proof follows the same structure as the proof of Theorem 3.7 in~\cite{chen2013information}, but
	it needs to accommodate the new double greedy algorithm structure and the double submodular
	property.
let $\varepsilon_1 = e^{(1-1/e)} \varepsilon/2$.
From the inner-submoduarlity property of the MRT model and 
	the proof of Theorem 3.7 in~\cite{chen2013information} based on the Chernoff bound,
	we can conclude that when $R\ge \lceil 27 k^2n\log(2kn^{\ell+1} T)/\varepsilon_1^2 \rceil$,
	for each round $i \in [T]$, with probability at least $1- \frac{1}{n^\ell T}$, 
	the seed set $S_i^g$ found by {\DoubleGreedy} is a $(1-1/e - \varepsilon_1)$ approximation
	of the optimal solution for round $i$ maximizing the marginal gain of
	$\rho(S_1, \ldots, S_{i-1}, S) - \rho(S_1, \ldots, S_{i-1}) $.
Using the union bound, we know that with probability at least $1- \frac{1}{n^\ell}$,
	for all $i\in [T]$ seed set $S_i^g$ is an $(1-1/e - \varepsilon_1)$ approximation
	of the optimal solution for round $i$.

Now at each greedy step, if the new item found is not the one giving the best marginal contribution
	but an $\alpha$ approximation of the optimal marginal solution, an easy extension of
	\cite{NWF78}, already reported in~\cite{GS07}, show that the greedy algorithm can give
	a $1-e^{-\alpha}$ approximate solution to the sumodular maximization problem.
In our case, consider the outer level when treating each subset $S_i$ as an item, Lemma~\ref{lem:outersubmodular} shows that $\rho$ is also submodular in this case 
	(the outer-submodularity), and we just argued in the previous paragraph that
	in each round, the selected $S_i^g$ is a $(1-1/e - \varepsilon_1)$ approximation.
Therefore, the final output $\cS^g = (S_1, \ldots, S_g)$ satisfies
\begin{equation*}
\rho(\cS^g) \ge (1-e^{-(1-1/e-\varepsilon_1)}) \rho(\cS^*).
\end{equation*}
Because $\varepsilon_1 = e^{(1-1/e)} \varepsilon/2$, it is easy to verify that 
	$1-e^{-(1-1/e-\varepsilon_1)} \ge 1-e^{-(1-1/e)} - \varepsilon$ in this case, and
	it is sufficient to have $R=\lceil 31 k^2n\log(2kn^{\ell+1} T)/\varepsilon^2 \rceil$.
Finally, the total running time is simply 
	$O(TknRm) = O(k^3\ell Tn^2m\log(n T)/\varepsilon^2)$.
\end{proof}

\subsection{RIS-based Algorithm}
\begin{lemma} \label{lem:MRRRset}
	For any seed set sequence $\cS=(S_1, S_2, \ldots, S_T)$, 
\begin{equation}
\rho(\cS) = n \cdot \E[\I\{\exists i\in [T], S_i\cap R^i \ne \emptyset \}], \label{eq:MRRRset}
\end{equation}
	where the expectation is taken over the randomness of RR set sequence $(R^1, R^2, \ldots, R^T)$.
\end{lemma}



\section{Adaptive MRIM}\label{sec:AMRIM}

In this section, we study the adaptive MRIM problem. 
Informally, adaptive MRIM is the problem where at the beginning of each round $i$, 
	the propagation results in previous rounds are observed and can be used as feedback
	for round $i$ to select better seeds.
The formal description of the problem follows the framework and terminology
	provided in~\cite{GoloKrause11}.
After its formal definition, we then argue about the adaptive submodularity property, 
	propose the adaptive greedy policy and analyze its performance.


\subsection{Notations and Definition}\label{sec:AMRIMDef}


We call $(S_i, i)$ an {\em item}, where $S_i$ is the seed set chosen in the $i$-th round,
and $i$ is the round number.
We explicitly use the round number $i$ to differentiate the same set that could appear
	in different rounds.
Let $\cE$ be the set of all the possible items.
For each item $(S_i, i)$,  after the propagation, the nodes and edges participated in
	propagation is observed as the feedback.
Formally, the feedback is referred to as a {\em state}, which is the subgraph of
	live-edge graph $L_i$ that can be reached by $S_i$.
A {\em realization} is a function $\phi: \cE \rightarrow O$ mapping 
	every possible item $(S_i, i)$ to a state, where $O$ is the set of all the possible states.
Realization $\phi$ represents one possible propagation from any possible seed set in any round.
We use $L^\phi_i$ to represent the live-edge graph in the round $i$ that determines
	the propagation in the round.
%\wei{I think I need this representation. Please check if any of the proofs need this 
%	notation.}
We say that $\phi(S_i,i)$ is the state of $(S_i, i)$ under realization $\phi$. 
We use $\Phi$ to denote a random realization, and the randomness comes from 
	random live-edge graphs $L_1, \ldots, L_T$.
For the adaptive MRIM, in each round $i$, we pick
an item $(S_i, i)$, see its state $\Phi(S_i,i)$, pick the next item $(S_{i+1},i+1)$,
see its state, and so on. 
After each pick, previous observations can be represented as a
{\em partial realization} $\psi$, a function from some subset of $\cE$ to their states.
For notational convenience, we represent $\psi$ as a relation, so that $\psi \subseteq \cE \times \textit{O}$
equals $\{((S_i,i),o): \psi(S_i,i)=o\}$. 
We define $\dom(\psi) = \{ (S_i, i): \exists o, ((S_i, i), o) \in \psi \}$
as the {\em domain} of $\psi$.
A partial realization $\psi$ is {\em consistent with} a realization $\phi$ if they are equal everywhere in the domain of $\psi$,
denoted as $\phi \sim \psi$. 
If $\psi$ and $\psi'$ are both consistent with some $\phi$, and $\dom(\psi) \subseteq \dom(\psi')$,
$\psi$ is a {\em subrealization} of $\psi'$, also denoted as $\psi \subseteq \psi'$.

%\subsection{Policy}

A {\em policy} $\pi$ is an adaptive strategy for picking items based on partial realizations in $\cE$.
In each round, $\pi$ will pick the next set of seeds $\pi(\psi)$ 
	based on the partial realization $\psi$ so far.
If the partial ralization $\psi$ is not in the domain of $\pi$, 
	the policy terminates (stops picking items). 
We use $\dom(\pi)$ to denote the domain of $\pi$. 
Technically, we require that $\dom(\pi)$ be closed under subrealizations: 
If $\psi' \in \dom(\pi)$ and $\psi$ is a subrealization of $\psi'$ then $\psi \in \dom(\pi)$.
We use the notation $E(\pi, \phi)$ to refer to the set of items selected by $\pi$ under realization $\phi$.
The set of items in $E(\pi, \phi)$ is always in the form 
	$\{(S_1, 1), (S_2, 2), \ldots, (S_t, t)\}$, so sometimes we also refer to it as 
	sequence of seed sets.

We wish to maximize, subject to some constraints, 
a utility function $f: 2^\cE \times O^\cE \rightarrow \R_{\geq 0}$ that depends on the picked items and 
the states of them. 
In the adaptive MRIM, $f(\{(S_1, 1), (S_2, 2), \ldots, (S_t, t)\}, \phi)$ 
	is the total number of active nodes in the $t$ rounds from the respective seed sets,
	namely $|\cup_{i=1}^t \Gamma(L^\phi_i, S_i)|$.
Based on the above notations, the expected utility of a policy $\pi$ is
$f_{\avg}(\pi) = \E_\Phi [f(E(\pi, \Phi),\Phi)]$ where the expectation is taken over 
	the randomness of $\Phi$.
Namely, $f_{\avg}(\pi)$ is the expected number of active nodes under the adaptive policy $\pi$.
Let $\Pi_{T,k}$ be the set of all policies that select seed sets in at most $T$ rounds and
	each seed set has at most $k$ nodes.
The goal of the adaptive MRIM is to find the best policy $\pi$ such that:

\begin{equation*}
\pi^* = \argmax_{\pi \in \Pi_{T,k}} f_{\avg}(\pi).
\end{equation*}
%\wei{We need notation $\Pi_{T,k}$ to talk about the constraints explicitly.}

\vspace{-0.1 in}
\subsection{Adaptive Submodularity and Adaptive Greedy Policy}
\label{sec:adagreedy}


Given a partial realization $\psi$ of $i-1$ rounds with 
$\dom(\psi) = \{(S_1, 1), (S_2, 2), \dots, (S_{i-1}, i-1)\}$, 
and seed set $S_{i}$ for the $i$-th round, 
the {\em conditional expected marginal benefit of item} $(S_{i},i)$ conditioned on having observed $\psi$ 
%denoted $\Delta( (S_{i+1}, i+1) | \psi)$, 
    is defined as
    \begin{align*}
        \Delta((S_{i},i) | \psi) 
         = \E_\Phi \left[ f(\dom(\psi) \cup \{(S_{i},i)\}, \Phi) - f(\dom(\psi), \Phi) \mid \Phi \sim \psi \right]. 
    \end{align*}
We also define the {\em conditional expected marginal gain} of a policy $\pi$ as
\begin{align*}
    \Delta(\pi | \psi) 
    = \E \left[ f(\dom(\psi) \cup E(\pi, \Phi), \Phi) - f(\dom(\psi), \Phi) \mid \Phi \sim \psi \right].
\end{align*}
We now show the adaptive monotonicity and submodularity for the adaptive MRIM.

\begin{lemma}[Adaptive Monotonicity] 
    %A function $\rho: \cS \rightarrow \R_{\geq 0}$ is adaptive monotone with respect
    %to distribution $\Phi$ if the conditional expected marginal benefit of any set of seeds $S_i$ is nonnegative,
    For all $i>0$, for all partial realization $\psi$ with $i-1$ rounds and $\Pr[\Phi \sim \psi]>0$, and for all item $(S_i, i)$ we have:
    \begin{equation*}
    \Delta((S_i,i) | \psi) \geq 0.
    \end{equation*}
\end{lemma}
%\begin{proof} The adaptive monotonicity is straightforward.
%\end{proof}

\begin{lemma}[Adaptive Submodularity] \label{lem:adaSubmodular}
%    A function $\rho: \cS \rightarrow \R_{\geq 0}$ is adaptive submodular with respect
%    to distribution $\Phi$ if the conditional expected marginal benefit of any fixed set of seeds $S_i$ does not increase as
%    more rounds are played and their states are observed. Formally, $\rho$ is adaptive submodular,
    For all $i>0$, for all partial realization $\psi$ with $i-1$ rounds and partial realization $\psi'$ such that $\psi'$ is a subrealization of $\psi$, i.e., $\psi' \subseteq \psi$,
%     and $|\dom(\psi)| = i - 1$, 
    and for all item $(S_{i},i)$, we have
    \begin{equation*}
    \Delta((S_{i},i) | \psi') \geq  \Delta((S_{i},i) | \psi).
    \end{equation*}
\end{lemma}
The proof of this lemma requires a careful analysis of the partial realization
	in the MRT model.
Due to the space constraint, it is included in our full report as an anonymous file
	\cite{fullreport}.

%Note that, $\Delta((S_{i'},i | \psi) = \Delta((S_{i'},i') | \psi) \geq \Delta((S_{i'},i') | \psi')$, where |$\psi$| = $i - 1$ and |$\psi$'| = $i' - 1$ and $i' \geq i$.

Following the framework of~\cite{GoloKrause11}, adaptive monotonicity and adaptive submodularity
	enables an adaptive greedy policy with a constant approximation of the optimal
	adaptive policy.
Algorithm~\ref{alg:adaptivegreedy} provides the greedy adaptive policy for MRIM, 
	{\alg{AdaGreedy}.
Note that adaptive algorithms operate at per round base --- it takes feedback from the
	previous rounds and select the item in the current round, and then obtain new feedback.
Thus we present \alg{AdaGreedy} for a generic round $i$.
Besides the problem input such as the graph $G$, the triggering model parameters, and
	seed set budget $k$, \alg{AdaGreedy} takes the set of already activated nodes $A_{i-1}$ 
	as the feedback from the previous rounds, and aims at find the seed set $S_i$
	of size $k$ to maximize the expected marginal gain $\Delta((S_{i},i) | \psi)$, which
	is the expected number of newly activated nodes in round $i$.
However, this problem is NP-hard, so we use a Monte Carlo greedy approximation
	$\alg{MC-Greedy}$ algorithm to find an approximate solution.
The rationale is that maximizing the expected marginal gain $\Delta((S_{i},i) | \psi)$
	is equivalent to the weighted influence maximization task in which we treat nodes in $A_{i-1}$ with
	weight $0$ and other nodes with weight $1$, and we maximize the expected total
	weight of the influenced nodes.
By \cite{mossel2007}, we know that the weighted version is also monotone and submodular, 
so we could use a greedy algorithm to obtain a seed set $S_i$
as a $(1-1/e -\varepsilon)$ approximation of the best seed set for round $i$.
We could use $R$ Monte Carlo simulations to estimate the weighted influence spread,
and $R$ is determined by the desired approximation accuracy $\varepsilon$.
Once the seed set $S_i$ is selected for round $i$, the actual propagation from $S_i$
	will be observed, and the active node set $A_i$ will be updated as the feedback for
	the next round.
	
The following theorem summarizes the correctness and the time complexity of \alg{AdaGreedy}.

\begin{algorithm}[t] 
	%\SetKwComment{tcp}{\tiny // }{}%
	\caption{\alg{AdaGreedy}: Greedy policy for round $i$ 
		of the adaptive MRIM} \label{alg:adaptivegreedy}
	\KwIn{Graph $G=(V,E)$, triggering set distributions, round number $T$, budget $k$,
		simulation count $R$, 
		activated nodes by round $i-1$ $A_{i-1}$.}
	\KwOut{Seed set $S_i$, updated active nodes $A_i$}
	
	$S_i\leftarrow $ \alg{MC-Greedy($G, A_{i-1}, k, R$)} \{Monte Carlo greedy algorithm to find $k$ seeds with influence spread outside $A_{i-1}$\}\;
%	$S_i \leftarrow \argmax_{S\subseteq V: |S|\le k} \Delta((S,i) | \psi) $\;
	Observe the propagation of $S_i$ and updates the activated nodes $A_i$\;
	\textbf{return} $(S_i,i)$, $A_i$
\end{algorithm}

%
%
%Influence maximization of ARIM is also hard to compute.
%Then, we introduce a greedy approach to partly overcome the combinatorial source of hardness, 
%and use Monte Carlo simulations to overcome the influence computation source of hardness.
%
%The greedy algorithm may not perform well in general, but when set function $f$ is monotone
%and submodular, it provides an approximation guarantee, as shown by the following classic
%theorem. Since this is a crucial theorem for our algorithm design, we reproduce the proof below.
%
%\wei{This is the citation for the general greedy approximation when we could assign
%    different weights to the nodes: \cite{mossel2007}
%}


\begin{theorem} \label{thm:AdaGreedy}
	Let $\pi^{\ag}$ represents the policy corresponding to the \alg{AdaGreedy} algorithm. 
	For any $\varepsilon > 0$ and $\ell > 0$, 
		if we use $R=\lceil 31 k^2n\log(2kn^{\ell+1} T)/\varepsilon^2 \rceil$ simulations
		for each influence spread estimation, then
		with probability at least $1-\frac{1}{n^\ell}$, 
	\begin{equation}
f_{\avg}(\pi^{\ag}) \geq \left(1 - e^{-(1-\frac{1}{e})}-\varepsilon \right) f_{\avg}(\pi^*).
\end{equation}
 In this case, the total running time for $T$-round \alg{AdaGreedy}
 	is $O(k^3\ell Tn^2m\log(n T)/\varepsilon^2)$.
\end{theorem}

\vspace{-0.15 in}
\begin{proof}[Proof (Sketch)]
From the general result of Theorem 5.2 in~\cite{GoloKrause11}, we know that
	if in each round we find an $\alpha$ approximation of the best solution of the round,
	then the greedy adaptive policy is an $1-e^{-\alpha}$ approximation of the optimal
	greedy policy $\pi^*$.
Then, following essentially the same high probability argument as in the proof sketch of 
	Theorem~\ref{thm:nonadaptive}, we could conclude that
	when using $R=\lceil 31 k^2n\log(2kn^{\ell+1} T)/\varepsilon^2 \rceil$
	Monte Carlo simulations for each influence spread estimation, with probability
	at least $1-\frac{1}{n^\ell}$, in all rounds the selected $S_i$ 
	is an $1-1/e - \varepsilon_1$ approximation, with $\varepsilon_1 = e^{(1-1/e)} \varepsilon/2$.
Together with Theorem 5.2 in~\cite{GoloKrause11}, we have that
	with probability at least $1-\frac{1}{n^\ell}$, 
	$f_{\avg}(\pi^{\ag}) \geq \left(1 - e^{-(1-\frac{1}{e})}-\varepsilon \right) f_{\avg}(\pi^*)$.
The running time is $O(TknRm) = O(k^3\ell Tn^2m\log(n T)/\varepsilon^2)$.
\end{proof}



%\begin{theorem}
%    Fix any $\alpha \geq 1$. If $f(\cdot)$ is adaptive monontone and adaptive submodular with respect to the distribution $f(\pi)$, 
%    and $\pi$ is an $\alpha$-approximate greedy policy, then for all policies $\pi^*$
%    
%    % Let $\cS = \{S_1,S_2,...,S_T\}$, 
%    %     where $S_i$ is selected by policy $\pi$ and previous records $\psi$ and $|S_i| \leq k$.
%    % $\pi^* \in argmax_{|\cS| \leq k}\; \rho(\cS)$ be the set maximizing
%    % $f(\pi)$ among all super multi-sets with size at most $k$.
%    % If set function $\rho$ is monotone and submodular and $\rho({\emptyset,\emptyset,...,\emptyset}) = 0$,
%    % then for the set $S^g$ computed by Greedy$(k; \rho)$, we have
%    
%    \begin{equation}
%    f(\pi^g) \geq (1 - \frac{1}{e^{\alpha}}) f(\pi^*).
%    \end{equation}
%    
%    where $e$ is the base of natural logarithm.
%\end{theorem}
%

%\wei{
%    There is an algorithm design problem. 
%    How to use RR-set (Reverse Reachable set) approach to efficiently do ARIM, and the idea
%    is to reuse the RR-sets of the first round to all later rounds.
%    For RR-set algorithm, please use the IMM algorithm in \cite{tang15}, which is also based
%    on prior work \cite{tang14,BorgsBrautbarChayesLucier}.
%}

\vspace{-0.2 in}
\subsection{Scalable Implementation with RR Sets} \label{sec:AdaIMM}

As can be seen from Theorem~\ref{thm:AdaGreedy}, the \alg{AdaGreedy} algorithm is not
	very efficient.
In this section, we utilize the approach of reverse-reachable (RR) sets~\cite{BorgsBrautbarChayesLucier,tang14,tang15} to significantly speed up the
	algorithm.

For  $v\in V$, a {\em reverse-reachable (RR) set $R_v$ rooted at $v$} 
	is by reverse simulating the propagation from $v$ in the triggering model, and 
	put all nodes reached into $R$.
Equivalently, we can sample a live-edge graph $L$, and $R_v$ is the set of all nodes
	that can reach $v$ in $L$.
We denote $v = \rroot(R_v)$.
When we do not fix the root, then a (random) RR set is generated by picking a root
	$v$ uniformly at random from $V$, and then generate the RR set rooted at $v$.

The RR set has the following important property. 
If $R$ is a random RR set, then for any seed set $S\subseteq V$, its influence spread
\begin{equation}
\sigma(S) = n \cdot \E[\I\{ S\cap R \ne \emptyset \}], \label{eq:RRset}
\end{equation}
where $\I\{\}$ is the indicator
	function and the expectation is taken over the randomness of $R$.
The property implies we can sample enough RR sets to accurately estimate 
	the influence spread of $S$.
More importantly, the sample set of RR sets can be use to estimate the influence spread
	of {\em all} possible seed sets, and by Eq.~\eqref{eq:RRset} the optimal seed set
	is equivalently the optimal set of nodes that intersect with (a.k.a. cover) 
	the most number of
	RR sets in the sample set, which is a max-cover problem.
Therefore, a series of near-linear-time algorithms are
	developed~\cite{BorgsBrautbarChayesLucier,tang14,tang15} based on the above observation.
All RR-set algorithms have the same structure of two phases.
In Phase 1, the number of RR sets need be estimated, and in Phase 2, these RR sets are
	generated and greedy algorithm is used on these RR sets to find the $k$ nodes
	that cover the most number of RR sets.
All algorithms has the same Phase 2, but Phase 1 is being improved from one to another
	so that less and less RR sets are needed.

In our adaptive setting, as already mentioned in Section~\ref{sec:adagreedy}, 
	some nodes $A_{i-1}$ are already activated, so they won't
	contribute to the influence spread in round $i$.
Therefore, we are working on the weighted influence maximization problem, where nodes
	in $A_{i-1}$ has weight $0$ and nodes in $V\setminus A_{i-1}$ has weight $1$.
Let $\sigma^{-A_{i-1}}(S)$ be the weighted influence spread according to the above weight.
Let $R^{-A_{i-1}}$ be a random RR set where the root $v$ is selected from $V\setminus A_{i-1}$
	uniformly at random, and then reverse simulate from $v$ to get the RR set.
Then we obtain the result similar to Eq.~\eqref{eq:RRset}:
\begin{lemma} \label{lem:ARRset}
For any seed set $S\subseteq V$, 
\begin{equation}
\sigma^{-A_{i-1}}(S) = (n-|A_{i-1}|) \cdot \E[\I\{ S\cap R^{-A_{i-1}} \ne \emptyset \}], \label{eq:AdaRRset}
\end{equation}
where the expectation is taken over the randomness of $R^{-A_{i-1}}$.
\end{lemma}
\begin{proof}
	\begin{align}
	& \E[\I\{ S\cap R^{-A_{i-1}} \ne \emptyset \}]  \nonumber \\
	& = \sum_{v\in V\setminus A_{i-1}} \Pr\{v =\rroot(R^{-A_{i-1}}) \} \cdot \nonumber \\
	& \quad \quad \E[\I\{ S\cap R^{-A_{i-1}} \ne \emptyset \} \mid v =\rroot(R^{-A_{i-1}})] 
		\nonumber \\
	& = \frac{1}{n-|A_{i-1}|} \sum_{v\in V\setminus A_{i-1}} 
		\E[\I\{ S\cap R_v^{-A_{i-1}} \ne \emptyset \} ] \nonumber  \\
	& = \frac{1}{n-|A_{i-1}|} \sum_{v\in V\setminus A_{i-1}} 
		\E[\I\{ v\in \Gamma(L, S)\} ] \label{eq:RRset2L} \allowdisplaybreaks \\
	& = \frac{1}{n-|A_{i-1}|} \E \left[ \sum_{v\in V\setminus A_{i-1}} \I\{ v\in \Gamma(L, S)\} \right] \nonumber \\
	& = \frac{1}{n-|A_{i-1}|} \E[|\Gamma(L, S) \setminus A_{i-1} | ] \nonumber \\
	& =  \frac{1}{n-|A_{i-1}|} \sigma^{-A_{i-1}}(S), \nonumber 
\end{align}
where Eq.~\eqref{eq:RRset2L} is based on the equivalence between RR sets and live-edge graphs,
	and the expectation from this point on is taken over the random live-edge graphs $L$. 
\end{proof}



Therefore, with Eq.~\eqref{eq:AdaRRset}, the same RR-set based algorithm can be used,
	and we only need to properly change the RR-set generation process and the
	estimation process.
Algorithm~\ref{alg:aimm} provides the pseudocode for the \alg{AdaIMM} algorithm, which
	is based on the \alg{IMM} algorithm in~\cite{tang15}.
For convenience, we mark the part different from \alg{IMM} in blue.
Phase 1 of the algorithm estimate the number $\theta$ of RR sets needed by estimating
	the lower bound $LB$ of the optimal spread value.
This estimation is by iteratively halving a threshold value $x_i$, and for each
	$x_i$ value, generate $\theta_j$ RR sets (lines~\ref{line:genRRset1b}--\ref{line:genRRset1e}),
	and find the seed set $S_j$ from the current RR sets (line~\ref{line:nodeselect1}), 
	and check
	if the current $x_i$ is good enough for the lower bound estimate
	(line~\ref{line:checkLB}), where $F_{\cR_i}(S_j)$ is the fraction of RR sets
	in $\cR_i$ that are covered by $S_j$.
Procedure $\alg{NodeSelection}(\cR_i,k)$ is to greedily select $k$ nodes that covers
	the most number of RR sets in $\cR_i$, and it is the same as in~\cite{tang15}, so it
	is omitted.
In Phase 2, $\theta$ RR sets are generated and node $S_i$ is selected greedily
	by procedure $\alg{NodeSelection}(\cR_i,k)$.
Finally, propagation from $S_i$ are observed and the activated nodes are used as the
	feedback for the next round.
	
The main differences from the standard \alg{IMM} include several points.
First, whenever we generate new RR sets in round $i$, we only start from roots in
	$V \setminus A_{i-1}$ (lines~\ref{line:sample1} and~\ref{line:sample2}), as explained by Lemma~\ref{lem:ARRset}.
Second, when we estimate the influence spread, we need to adjust it using
	$n_a = n - |A_{i-1}|$ (lines~\ref{line:for1}, \ref{line:assignx}, \ref{line:estimate1}, \ref{line:estimate2}),
	again by Lemma~\ref{lem:ARRset}.
Third, we need to adjust $\ell$ to be $\ell + \log(2T)/\log n$,
	and $\varepsilon$ to $\varepsilon_1 = e^{(1-1/e)} \varepsilon/2$.
This is to guarantee that in each round we have probability at least $1 - 1/(n^\ell T)$ to
	have $S_i$ as a $(1-1/e - \varepsilon_1)$ approximation, so that the result for the
	total $T$ rounds would come out correctly as stated in the following theorem.

\begin{algorithm}[t] 
	%\SetKwComment{tcp}{\tiny // }{}%
	\caption{{\alg{AdaIMM}}: Adaptive IMM algorithm for round $i$ } \label{alg:aimm}
	\KwIn{Graph $G=(V,E)$, round number $T$, budget $k$, accuracy parameters $(\varepsilon, \ell)$, triggering set distributions, all active nodes by round $i-1$ $A_{i-1}$}
	%	\KwIn{\newalg{[from round $i-1$] all active nodes by round $i-1$
	%			$A_{i-1}$, newly activated nodes $A^{\new}_{i-1}$, adaptive RR-sets
	%			$\cR_{i-1}$ , optimal value lower bound threshold $x_{i-1}$}}
	\KwOut{seed set $S_i$, \newalg{and updated active nodes $A_i$}}

    
	\tcp{Phase 1: Estimating the number of RR sets needed, $\theta$}
	
	%	\newalg{delete all $R \in \cR_{i-1}$ with $\rroot(R) \in A^{\new}_{i-1}$}\;
	%	\label{line:updateRRset}
	
	%	\For{$a \in A$}{
	%		%\label{line:simulate}
	%		\For{$R \in \cR_{i-1}$}{
	%			\If {root($R$) == $a$}{
	%				delete $R$\;}
	%		}
	%	}
	%	\newalg{$\cR_{i} \leftarrow \cR_{i-1}$}; 
	\newalg{$n_a \leftarrow n - |A_{i-1}|$}; 
    \newalg{$\ell \leftarrow \ell + \log (2T) / \log n $};
	\newalg{$\varepsilon = e^{(1-1/e)} \varepsilon/2$}\;
	$\varepsilon' \leftarrow \sqrt{2} \cdot \varepsilon $; 
	$\cR_{i} \leftarrow \emptyset$\;
	$\alpha \leftarrow \sqrt{\ell \log{n} + \log{2}}$;
	$\beta \leftarrow \sqrt{(1-1/e)\cdot (\log{\binom{n}{k}}+\alpha^2)}$\;
	% 	$\lambda' \leftarrow \frac{(2+\frac{2}{3}\varepsilon') \cdot (\log{\binom{n}{k}}+\ell \cdot \log{n}+\log{\log_2{n}})\cdot n}{\varepsilon'^2}$\;
	$\lambda' \leftarrow [(2+\frac{2}{3}\varepsilon') \cdot (\log{\binom{n}{k}}+\ell \cdot \log{n}+\log{\log_2{n}})\cdot n]/\varepsilon'^2$\;
	$\lambda^* \leftarrow 2 n \cdot ((1-1/e) \cdot \alpha + \beta)^2 \cdot \varepsilon^{-2}$\;
	\For{$j = 1 \; to \; \log_2{(\newalg{n_a} - 1)}$ \label{line:for1}}{
		%\label{line:simulate}
		%		\eIf {$A_{i-1} = \emptyset$} {$x_i \leftarrow n/2^j$\;}
		%		{\newalg{$x_i \leftarrow (x_{i-1}-|A^{\new}_{i-1}|)/2^{(j-1)}$}\;} \label{line:updatex}
		$x_i \leftarrow \newalg{n_a}/2^j$\; \label{line:assignx}
		$\theta_j \leftarrow \lambda'/x_i$\; \label{line:genRRset1b} 
		\While{$|\cR_i| < \theta_j$}{
			Select a node $v$ from \newalg{$V \setminus A_{i-1}$} uniformly at random\; \label{line:sample1}
			Generate RR set $R$ from $v$, and insert it into $\cR_i$\; 
		}\label{line:genRRset1e} 
		$S_j \leftarrow \NodeSelection(\cR_i,k)$\; \label{line:nodeselect1}
		\If{$\newalg{n_a} \cdot F_{\cR_i}(S_j) \geq (1 + \varepsilon') \cdot x_i$}{
			\label{line:estimate1}
			$LB \leftarrow \newalg{n_a} \cdot F_{\cR_i}(S_j)/(1 + \varepsilon')$\; 
			\label{line:estimate2}
			break\;
		} 
	}
	$\theta \leftarrow \lambda^* / LB$\;
	\While{$|\cR_i| \leq \theta$}{ \label{line:checkLB}
		Select a node $v$ from \newalg{$V \setminus A_{i-1}$} uniformly at random\;\label{line:sample2}
		Generate $R$ for $v$, and insert it into $\cR_i$\; 		
	}
	
	\tcp{Phase 2: Generate $\theta$ RR sets and select seed nodes}
	$S_i \leftarrow \NodeSelection(\cR_i,k)$ \;
	\newalg{Observe the propagation from $S_i$ in round $i$, update
		the set of activated nodes to $A_i$}\; 
	
	return $S_i$, \newalg{$A_i$}.
\end{algorithm}

\begin{theorem} \label{thm:AdaIMM}
	Let $\pi^{\ai}$ represents the policy corresponding to the \alg{AdaIMM} algorithm. 
For any $\varepsilon > 0$ and $\ell > 0$, with probability at least $1-\frac{1}{n^\ell}$, 
\begin{equation}
f_{\avg}(\pi^{\ai}) \geq \left(1 - e^{-(1-\frac{1}{e})}-\varepsilon \right) f_{\avg}(\pi^*).
\end{equation}
In this case, the total running time for $T$-round \alg{AdaIMM}
is $O(T(k + \ell)(n + m)\log{(nT)}/\varepsilon^2)$.
\end{theorem}
\begin{proof}[Proof (Sketch)]
Let $\varepsilon_1 = e^{(1-1/e)} \varepsilon/2$, 
	$\ell' = \ell + \log (2T) / \log n $.
As explained already, one round \alg{AdaIMM} is essentially the same as \alg{IMM}
	with parameters $\varepsilon_1$ and $\ell'$.
Thus, following the result in~\cite{tang15}, we know that for each round $i$,
	with probability at least $ 1 - 2/n^{\ell'} = 1 - 1/(n^\ell T)$, 
	output $S_i$ is a $(1 - 1/e - \varepsilon_1)$ approximation of the
	best seed set for this round.
Then following the similar arguments as in Theorems~\ref{thm:nonadaptive} and~\ref{thm:AdaGreedy},
	we know that across all $T$ rounds, 
	with probability at least $1 - 1/n^\ell$,
\begin{align*}
f_{\avg}(\pi^{\ai}) &  \geq \left(1 - e^{-(1-\frac{1}{e} - \varepsilon_1)}\right) f_{\avg}(\pi^*)\\
& \ge \left(1 - e^{-(1-\frac{1}{e})}-\varepsilon \right) f_{\avg}(\pi^*).
\end{align*}
Thus, the theorem holds.
\end{proof}

Theorem~\ref{thm:AdaIMM} clearly shows that the \alg{AdaIMM} algorithm is near linear time,
	and its theoretical time complexity bound is much better than
	the one in Theorem~\ref{thm:AdaGreedy} for the \alg{AdaGreedy} algorithm.
	
In practice, we can further improve the \alg{AdaIMM} algorithm by incremental computation.
In particular, RR sets generated in the previous $i-1$ rounds can be used for round $i$,
	and we only need to remove those rooted at nodes in $A_{i-1}$.
Searching the lower bound $LB$ can also be made faster by utilizing the $x_{i-1}$ already
	obtained in the previous round.
Our experiments would use such improvements for \alg{AdaIMM}.

%RR-sets is an efficient way to optimize the node selection in practise.
%In this section, we are going to talk about applying RR-sets of MRIM.
%After revisiting some basic concepts of RR-sets and its approach,
%we give a new definition named adaptive RR-sets of MRIM.
%Then, we will separately discuss using RR-sets on non-adaptive and adaptive MRIM.
%
%\subsection{Revisiting RR-sets and Practise Approach}
%
%The type of node sets sampled by previous works\cite{}
%is referred to as random RR sets, defined as follows:
%
%\begin{definition} \textbf{Reverse Reachable Set}
%    Let $v$ be a node in $V$. 
%    A reverse reachable ($RR$) set for $v$ is generated by first sampling a graph $g$ from $G$, 
%    and then taking the set of nodes in $g$ that can reach $v$. 
%    A random $RR$ set is an $RR$ set for a node selected uniformly at random from $V$ .
%\end{definition}
%
%Intuitively, if a node $u$ appears in an $RR$ set of another node $v$,
%then a diffusion process from a seed set containing $u$ should have a
%certain probability to activate $v$. This connection between $RR$ sets
%and node activation is formalized in the following lemma.
%
%\begin{lemma}\label{lemma:rr-sets}
%    For any seed set $S$ and any node $v$, 
%    the probability that a diffusion process from $S$ can activate $v$ equals
%    the probability that $S$ overlaps an RR set for $v$.
%\end{lemma}
%
%Based on Lemma \ref{lemma:rr-sets}, the node selection phase of \cite{} 
%adopts the following approach for influence maximization:
%
%\begin{enumerate}
%    \item Generate a sizable set $R$ of independent random $RR$ sets.
%    \item Consider the maximum coverage problem 
%    \cite{} of selecting $k$ nodes to cover the maximum number of $RR$ sets in $R$.
%    Apply the standard greedy algorithm to obtain a ($1 - 1/e$)-approximate solution $S^*$
%    $k$ to the problem. 
%    \item Return $S^*_k$ as the answer for influence maximization.
%\end{enumerate}
%
%\subsection{MRIM of RR-sets}
%
%For non-multi-round IM model,
%let $R_1, R_2, \ldots, R_{\theta}$ be the sequence of 
%random RR sets generated in the sampling phase of IMM. 
%Let $S$ be any set of nodes in $G$,
%and $x_i$ ($i \in [1, \theta]$) be a random variable 
%that equals 0 if $S \cap R_i = \emptyset$,
%and 1 otherwise. By Lemma 1 and the linearity of expectation,
%
%\begin{equation}
%\E[\sigma(S)] = \frac{n}{\theta} \cdot \E[\sum^{\theta}_{i = 1} x_i]
%\end{equation}
%
%However, multi-round diffusion model and its influence maximization are different due to its multi-rounds.
%We define the marginal rewards and offer a new approach to generate the
%RR-sets of multi-round IM model. R
%
%After first round, we need to simulate a forward simulation to simulate
%a real-life spread and receive the feedback.
%Then, we generate the RR-sets for next round node selection. 
%However, the activated node can not be used as root for generating the RR-sets,
%since any node can not be activated twice by definition of multi-round diffusion model.
%The original definition and the approach to generate the RR-sets are no longer
%suitable for the influence maximization under the multi-round diffusion model. 
%Therefore, we give a new definition of the adaptive RR-sets of MRIM.
%
%\begin{definition} \textbf{Adaptive Reverse Reachable Set}
%    Given a set $A$ including all activated nodes in previous rounds,
%    an adaptive reverse reachable ($RR$) set for $v \in V/A$ is generated by first sampling a graph $g$ from $G$, 
%    and then taking the set of nodes in $g$ that can reach $v$. 
%    A random $RR$ set is an $RR$ set for a node selected uniformly at random from $V$ .
%\end{definition}
%
%Based on the adaptive RR set, we give a new lemma based on it.
%
%\begin{lemma}\label{lemma:adaptive_rr-sets}
%	In i-th round, 
%	for any seed set $S_i$ and any node $v \in V \setminus A$, 
%	the probability that a diffusion process from $S$ can activate $v$ equals
%	the probability that $S$ overlaps an adaptive RR set for $v$.
%\end{lemma}
%
%For multi-round diffusion model, the expectation influence of current round 
%is the marginal rewards while receiving the feedback information until now.
%Let $R^A_1, R^A_2, \ldots, R^A_{\theta}$ be the sequence of 
%random adaptive RR sets (denoted as $\cR^A$) generated in the sampling phase of adaptive-IMM. 
%Let $S_i$ be any set of nodes in $G$ in $i$-th round,
%and $x^A_i$ ($i \in [1, \theta]$) be a random variable 
%that equals 0 if $S_i \cap R^A_i = \emptyset$,
%and 1 otherwise. Let $A$ is set of activated nodes till now.
%By Lemma \ref{lemma:rr-sets} and the linearity of marginal rewards of $S_i$ in $i$-th round,
%
%\begin{equation}
%	\E[(\rho(S_i; A)] = \frac{n}{\theta} \cdot \E[\sum^{\theta}_{i = 1} x^A_i]
%\end{equation}
%
%By using Lemma \ref{lemma:adaptive_rr-sets}, we have:
%
%\begin{proof}
%	\begin{align*}
%		& \E[(\rho(S_i; A)] \\
%		& = \sum_{L_i} Pr(L_i) (\left|\Gamma(L_i, S_i)\right| -|A|)
%		= \sum_{L_i} Pr(L_i) (\left|\Gamma(L_i, S_i) -A\right|)\\
%		% & \Leftrightarrow  \nonumber \\ 
%		& =  \sum_{L_i} Pr(L_i) \sum_{v \in V} \bbI\{S_i \cap R_v, v \notin A , {L_i} \neq \emptyset\} \\
%		& =  \sum_{L_i} Pr(L_i)\sum_{v \in V \setminus A} \bbI\{S_i \cap R^A_v, {L_i} \neq \emptyset\} \\
%		%& = \frac{1}{n-|A|} \sum_{L_i} Pr(L_i) \sum_{v \in V \setminus A} \bbI\{S_i \cap R^A_v, {L_i} \neq \emptyset\} \cdot ( n - |A|) \\
%		& = \E \left[\sum_{v \in V \setminus A} \bbI\{S_i \cap R^A_v\} \right] 
%		 = \frac{ n - |A|}{n - |A|} \E \left[\sum_{i = 1}^{n - |A|} \bbI\{S_i \cap R^A_i\} \right]\\
%		& = \frac{ n - |A|}{\theta} \E \left[\sum_{i = 1}^{\theta} \bbI\{S_i \cap R^A_i\} \right]
%	\end{align*}
%\end{proof}


%\subsection{Performance and Efficiency}
%
%In each round, comparing to original IMM algorithm,
%adaptive-IMM uses the feedbacks from previous rounds for samples generation.
%The node selection algorithm is the same as the original IMM.
%Comparing to the original IMM algorithm, 
%the difference is we create the adaptive RR-sets
%instead RR-sets based on previous feedback information. 
%However, the time complexity of generating adaptive RR-sets is the 
%same as the original approach which is linear. 
%The forward simulation between each round is simulating real-life spread which 
%won't cost more time of the algorithm. 
%Therefore, the time complexity of each round is the same as IMM which is $O((k + l)(n + m)\log{n}/\varepsilon^2)$ expected time.
%The total time complexity of multi-round influence maximization is 
%$O(T(k + l)(n + m)\log{n}/\varepsilon^2)$.
%
%Due to the property multi-round diffusion model,
%one node can not be activated twice.
%To analysis the performance of each round of adaptive MRIM, 
%we need to know which and how many nodes have been activated in previous rounds.
%$n_a$ denotes the maximum number nodes can be activated in this round which is less than $n$ usually after first round.
%However, intuitively,both greedy algorithm and optimal solution will decrease the maximum number of nodes with feedbacks from previous rounds.
%Then, in i-th round, adaptive IMM algorithm guarantees $(1 - 1/e -\varepsilon)$
%approximation to the respective optimal solutions.
%However, due to double greedy, adaptive MRIM guarantees $1 - e^{-(1/e)}) - \varepsilon'$
%approximation with $\pi^g$ to the respective optimal policy $\pi^*$.

==> sec_namrim.tex <==
\section{Boosted Influence Maximization} \label{sec:nonadaptive}

%\wei{explain the submodularity of node-round pairs. Explain partition matroid constraint, and
%    show our MRIM problem is an instance of submodular maximization under matroid constraint.}

Let $\cV_t = \{(v,t) \mid v \in V\}$ be the set of all possible nodes in round $t$ (e.g., $\cS_t \subseteq \cV_t$), and
$\cV := \bigcup_{t = 1}^T \cV_t $.
%\wei{To be consistent with the pair notation, I also use $\cV_t$. Please change all later sections
%	accordingly.}
We first show that the influence spread function $\rho$ for the MRT model is monotone and submodular.


\begin{restatable}{lemma}{mrtsubmodular} \label{lem:mrtsubmodular}
    Influence spread $\rho(\cS)$ for the MRT model satisfies
    (a) monotonicity: for any $\cS^A \subseteq \cS^B \subseteq \cV$,  $\rho(\cS^A)\leq\rho(\cS^B)$;
    and (b) submodularity: 
    for any $\cS^A \subseteq \cS^B \subseteq \cV$ and any pair $(v, t) \in \cV\setminus \cS^B$, % that means the total number of chosen seeds of $t$-th round is less than $k$ , 
    $\rho(\cS^A \cup \{(v, t)\})-\rho(\cS^A) \geq \rho(\cS^B \cup \{(v, t)\})-\rho(\cS^B)$.
\end{restatable}
\begin{proof}
	The proof of monotonicity is straightforward, so we next consider submodularity.
	According to the definition of the influence spread, we have
	\begin{align*}
		&\rho(\cS^A \cup \{(v,t)\})-\rho(\cS^A) \geq \rho(\cS^B \cup \{(v,t)\})-\rho(\cS^B) \\
		\Leftrightarrow & \E\left[\left|\bigcup_{i=1}^T \Gamma(L_i,S_i^A) \setminus \Gamma(L_t,S_t^A) \cup \Gamma(L_t,S_t^A \cup \{v\})\right|\right] \\
		&- \E\left[\left|\bigcup_{i=1}^T \Gamma(L_i,S_i^A)\right|\right] \\
		\Leftrightarrow & \E\left[\left|\bigcup_{i=1}^T \Gamma(L_i,S_i^A) \cup \Gamma(L_t,S_t^A \cup \{v\})\right|\right] - \E\left[\left|\bigcup_{i=1}^T \Gamma(L_i,S_i^A)\right|\right] \\
		\geq &  \E\left[\left|\bigcup_{i=1}^T \Gamma(L_i,S_i^B) \setminus \Gamma(L_t,S_t^B) \cup \Gamma(L_{t+1},S_t^A \cup \{v\})\right|\right] \\
		&- \E\left[\left|\bigcup_{i=1}^T \Gamma(L_i,S_i^B)\right|\right] \\
		\Leftrightarrow & \E\left[\left|\bigcup_{i=1}^T \Gamma(L_i,S_i^B) \cup \Gamma(L_t,S_t^B \cup \{v\})\right|\right] - \E\left[\left|\bigcup_{i=1}^T \Gamma(L_i,S_i^A)\right|\right]. \\
	\end{align*}
	%	If we can prove that for any fixed $L_1, L_2, \dots, L_{T+1}$, the following holds, then the above also holds.
	%	\begin{align*}
	%		& |\bigcup_{i=1}^T \Gamma(L_i,S_i^A) \cup \Gamma(L_{T+1},S_{T+1})| - |\bigcup_{i=1}^T \Gamma(L_i,S_i^A)| \\
	%		& \geq  |\bigcup_{i=1}^T \Gamma(L_i,S_i^B) \cup \Gamma(L_{T+1},S_{T+1})| - |\bigcup_{i=1}^T \Gamma(L_i,S_i^B)|
	%	\end{align*}
	Then it is sufficient to show that
	\begin{align}\label{proofeq:1}
		& \bigcup_{i=1}^T \Gamma(L_i,S_i^A) \cup \Gamma(L_{t},S_t^A \cup \{v\}) \setminus \bigcup_{i=1}^T \Gamma(L_i,S_i^A) \nonumber\\
		& \supseteq  \bigcup_{i=1}^T \Gamma(L_i,S_i^B) \cup \Gamma(L_{t},S_t^B \cup \{v\}) \setminus \bigcup_{i=1}^T \Gamma(L_i,S_i^B).
	\end{align}
	
	For a node $u \in \bigcup_{i=1}^T \Gamma(L_i,S_i^B) \cup \Gamma(L_{t},S_t^B \cup \{v\}) \setminus \bigcup_{i=1}^T \Gamma(L_i,S_i^B)$, 
	$u$ is reachable from $S_t^B \cup \{v\}$ in $L_{t}$, 
	but not reachable from $S_{i}^B$ in $L_{i}$ for any $i\in[T]$.
	Thus $u$ is also not reachable from $S_{i}^A$ in $L_{i}$ for any $i\in[t]$.
	Therefore, we conclude that $u \in \bigcup_{i=1}^T \Gamma(L_i,S_i^A) \cup \Gamma(L_{t},S_{t}^A \cup \{v\}) \setminus \bigcup_{i=1}^T \Gamma(L_i,S_i^A)$.
	Thus the submodularity holds.
\end{proof}



%The above lemma can directly lead to the monotonicity and submodularity of influence spread $\sigma$ in the classical triggering model by setting $T=1$.
%    
The monotonicity and submodularity above are the theoretical basis of designing and analyzing greedy algorithms for the non-adaptive MRIM.
In the following sections, we will consider two different settings separately for seed node selection: within-round and cross-round.
For the within-round setting, 
    one needs to determine the seed sets round by round,
    while for the cross-round setting,
    one is allowed to select nodes crossing rounds.
    

==> sec_pim.tex <==
\section{Preemptive Influence Maximization}\label{sec:PIM}

We now study the adaptive MRIM problem. 
Informally, at the beginning of each round, 
one need to determine the seed set for the current round based on 
	the propagation results observed  in previous rounds. % are observed and can be used as feedback
%	for the current round to select better seeds.
The formal definition follows the framework and terminology
	provided in~\cite{GoloKrause11} and will be given in Section~\ref{sec:AMRIMDef}.
We then argue about the adaptive submodularity property, 
	propose the adaptive greedy policy and analyze its performance in Section~\ref{sec:adagreedy}.


\subsection{Notations and Definition}\label{sec:AMRIMDef}


We call $(S_t, t)$ an {\em item}, where $S_t$ is the seed set chosen in round $t$.
%We explicitly use the round number $t$ to differentiate the same set that could appear
%	in different rounds.
Let $\cE$ be the set of all the possible items.
For each item $(S_t, t)$,  after the propagation, the nodes and edges participated in the
	propagation are observed as the feedback.
Formally, the feedback is referred to as a {\em state}, which is the subgraph of
	live-edge graph $L_t$ that can be reached by $S_t$.
A {\em realization} is a function $\phi: \cE \rightarrow O$ mapping 
	every possible item $(S_t, t)$ to a state, where $O$ is the set of all possible states.
Realization $\phi$ represents one possible propagation from a possible seed set in a round.
%We say that
Let $\phi(S_t,t)$ denote the state of $(S_t, t)$ under realization $\phi$. 
We use $\Phi$ to denote a random realization, and the randomness comes from 
	random live-edge graphs $L_1, \ldots, L_T$.
For the adaptive MRIM, in each round $t$, we pick
an item $(S_t, t)$, see its state $\Phi(S_t,t)$, pick the next item $(S_{t+1},t+1)$,
see its state, and so on. 
After each pick, previous observations can be represented as a
{\em partial realization} $\psi$, a function from some subset of $\cE$ to their states.
For notational convenience, we represent $\psi$ as a relation, so that $\psi \subseteq \cE \times \textit{O}$
equals $\{((S_t,t),o)\colon \psi(S_t,t)=o\}$. 
We define $\dom(\psi) = \{ (S_t, t)\colon \exists o, ((S_t, t), o) \in \psi \}$
as the {\em domain} of $\psi$.
A partial realization $\psi$ is {\em consistent with} a realization $\phi$ if they are equal everywhere in the domain of $\psi$,
denoted as $\phi \sim \psi$. 
If $\psi$ and $\psi'$ are both consistent with some $\phi$, and $\dom(\psi) \subseteq \dom(\psi')$,
$\psi$ is a {\em subrealization} of $\psi'$, also denoted as $\psi \subseteq \psi'$.

%\subsection{Policy}

A {\em policy} $\pi$ is an adaptive strategy for picking items based on partial realizations in $\cE$.
In each round, $\pi$ will pick the next set of seeds $\pi(\psi)$ 
	based on partial realization $\psi$ so far.
If partial realization $\psi$ is not in the domain of $\pi$, 
	the policy stops picking items. 
We use $\dom(\pi)$ to denote the domain of $\pi$. 
Technically, we require that $\dom(\pi)$ be closed under subrealizations: 
If $\psi' \in \dom(\pi)$ and $\psi$ is a subrealization of $\psi'$ then $\psi \in \dom(\pi)$.
We use the notation $E(\pi, \phi)$ to refer to the set of items selected by $\pi$ under realization $\phi$.
The set of items in $E(\pi, \phi)$ is always in the form 
	$\{(S_1, 1), \ldots, (S_t, t)\}$, so sometimes we also refer to it as 
	sequence of seed sets.

We wish to maximize, subject to some constraints, 
a utility function $f\colon 2^\cE \times O^\cE \rightarrow \R_{\geq 0}$ that depends on the picked items and 
the states of them. 
In the adaptive MRIM, $f(\{(S_1, 1), \ldots, (S_t, t)\}, \phi)$ 
	is the total number of active nodes by round $t$ from the respective seed sets,
	i.e., $|\bigcup_{i=1}^t \Gamma(L^\phi_i, S_i)|$ where $L^\phi_t$ is the live-edge graph of round $t$.
Based on the above notations, the expected utility of a policy $\pi$ is
$f_{\avg}(\pi) = \E_\Phi [f(E(\pi, \Phi),\Phi)]$ where the expectation is taken over 
	the randomness of $\Phi$.
Namely, $f_{\avg}(\pi)$ is the expected number of active nodes under policy $\pi$.
Let $\Pi_{T,k}$ be the set of all policies that select seed sets in at most $T$ rounds and
	each seed set has at most $k$ nodes.
The goal of the adaptive MRIM is to find the best policy $\pi$ such that:
$\pi^* = \argmax_{\pi \in \Pi_{T,k}} f_{\avg}(\pi)$.
%\begin{equation*}
%\pi^* = \argmax_{\pi \in \Pi_{T,k}} f_{\avg}(\pi).
%\end{equation*}
%\wei{We need notation $\Pi_{T,k}$ to talk about the constraints explicitly.}


\subsection{Adaptive Submodularity and Greedy Policy}
\label{sec:adagreedy}


Given a partial realization $\psi$ of $t-1$ rounds with 
$\dom(\psi) = \{(S_1, 1), (S_2, 2), \dots, (S_{t-1}, t-1)\}$, 
and the seed set $S_{t}$ for round $t$, 
the {\em conditional expected marginal benefit} of item $(S_{t},t)$ conditioned on having observed $\psi$ 
%denoted $\Delta( (S_{i+1}, i+1) | \psi)$, 
    is defined as
    \begin{align*}
        \Delta((S_{t},t) | \psi) 
         = \E_\Phi \left[ f(\dom(\psi) \cup \{(S_{t},t)\}, \Phi) - f(\dom(\psi), \Phi) \mid \Phi \sim \psi \right]. 
    \end{align*}
The {\em conditional expected marginal gain} of a policy $\pi$ is defined as
\begin{align*}
    \Delta(\pi | \psi) 
    = \E \left[ f(\dom(\psi) \cup E(\pi, \Phi), \Phi) - f(\dom(\psi), \Phi) \mid \Phi \sim \psi \right].
\end{align*}
The adaptive MRIM satisfies the adaptive monotonicity and submodularity shown as below.
The proofs require a careful analysis of the partial realization in the MRT model and is given in \OnlyInShort{\cite{sun2018multi}.} \OnlyInFull{the appendix.}

\begin{restatable}{lemma}{adamonotone}[Adaptive Monotonicity] 
    %A function $\rho: \cS \rightarrow \R_{\geq 0}$ is adaptive monotone with respect
    %to distribution $\Phi$ if the conditional expected marginal benefit of any set of seeds $S_i$ is nonnegative,
    For all $t>0$, for all partial realization $\psi$ with $t-1$ rounds and $\Pr[\Phi \sim \psi]>0$, and for all item $(S_t, t)$, we have:
    \begin{equation*}
    \Delta((S_t,t) | \psi) \geq 0.
    \end{equation*}
\end{restatable}
%\begin{proof} The adaptive monotonicity is straightforward.
%\end{proof}

\begin{restatable}{lemma}{adasubmodular}[Adaptive Submodularity] \label{lem:adaSubmodular}
%    A function $\rho: \cS \rightarrow \R_{\geq 0}$ is adaptive submodular with respect
%    to distribution $\Phi$ if the conditional expected marginal benefit of any fixed set of seeds $S_i$ does not increase as
%    more rounds are played and their states are observed. Formally, $\rho$ is adaptive submodular,
    For all $t>0$, for all partial realization $\psi$ with $i-1$ rounds and partial realization $\psi'$ such that $\psi'$ is a subrealization of $\psi$, i.e., $\psi' \subseteq \psi$,
%     and $|\dom(\psi)| = t - 1$, 
    and for all item $(S_{i},i)$, we have
    \begin{equation*}
    \Delta((S_{t},t) | \psi') \geq  \Delta((S_{t},t) | \psi).
    \end{equation*}
\end{restatable}

%Due to the space constraint, it is included in our full report as an anonymous file
%	\cite{fullreport}.

%Note that, $\Delta((S_{i'},i | \psi) = \Delta((S_{i'},i') | \psi) \geq \Delta((S_{i'},i') | \psi')$, where |$\psi$| = $i - 1$ and |$\psi$'| = $i' - 1$ and $i' \geq i$.

Following the framework of~\cite{GoloKrause11}, adaptive monotonicity and adaptive submodularity
	enable an adaptive greedy policy with a constant approximation of the optimal
	adaptive policy.
{\alg{AdaGreedy} (Algorithm~\ref{alg:adaptivegreedy}) is the greedy adaptive policy for MRIM.
Note that adaptive algorithms operate at per round base --- it takes feedback from
	previous rounds and selects the item for the current round, and then obtain new feedback.
Thus we present \alg{AdaGreedy} for a generic round $t$.
Besides the problem input such as the graph $G$, the triggering model parameters, 
	seed set budget $k$, and simulation number $R$, \alg{AdaGreedy} takes the set of already activated nodes $A_{t-1}$ 
	as the feedback from the previous rounds, and aims at finding the seed set $S_t$
	of size $k$ to maximize the expected marginal gain $\Delta((S_{t},t) | \psi)$, which
	is the expected number of newly activated nodes in round $t$.
However, this problem is NP-hard, so we use a Monte Carlo greedy approximation
	$\alg{MC-Greedy}$ algorithm to find an approximate solution. 
$\alg{MC-Greedy}$ greedily finds the seed with the maximum estimated marginal influence spread until $k$ seeds being selected, where the marginal influence spread of adding an unselected seed is estimated by simulating the propagation $R$ times.
In \alg{AdaGreedy}, $\alg{MC-Greedy}$ won't count the influence of a node if it has been activated in previous rounds. 
The rationale is that maximizing the expected marginal gain $\Delta((S_{t},t) | \psi)$
	is equivalent to the weighted influence maximization task in which we treat nodes in $A_{t-1}$ with
	weight $0$ and other nodes with weight $1$, and we maximize the expected total
	weight of the influenced nodes.
By \cite{mossel2007}, we know that the weighted version is also monotone and submodular, 
so we could use a greedy algorithm to obtain a seed set $S_t$
as a $(1-1/e -\varepsilon)$ approximation of the best seed set for round $t$.
We could use $R$ Monte Carlo simulations to estimate the weighted influence spread,
and $R$ is determined by the desired approximation accuracy $\varepsilon$.
Once the seed set $S_t$ is selected for round $t$, the actual propagation from $S_t$
	will be observed, and the active node set $A_t$ will be updated as the feedback for
	the next round.

The following theorem summarizes the correctness and the time complexity of \alg{AdaGreedy}.

\begin{algorithm}[t] 
	%\SetKwComment{tcp}{\tiny // }{}%
	\caption{\alg{AdaGreedy}: Adaptive Greedy for Round $t$} \label{alg:adaptivegreedy}
	\KwIn{Graph $G=(V,E)$, integers $T$, $k$ and $R$, triggering set distributions, 
		active node set $A_{t-1}$ by round $t-1$.}
	\KwOut{Seed set $S_t$, updated active nodes $A_t$}
	
	$S_t\leftarrow $ \alg{MC-Greedy($G, A_{t-1}, k, R$)}\tcp*{Monte Carlo Greedy} %Algorithm to find $k$ seeds with influence spread outside $A_{t-1}$}
%	$S_i \leftarrow \argmax_{S\subseteq V: |S|\le k} \Delta((S,i) | \psi) $\;
	Observe the propagation of $S_t$, update activated nodes $A_t$\;
	\textbf{return} $(S_t,t)$, $A_t$.
\end{algorithm}

%
%
%Influence maximization of ARIM is also hard to compute.
%Then, we introduce a greedy approach to partly overcome the combinatorial source of hardness, 
%and use Monte Carlo simulations to overcome the influence computation source of hardness.
%
%The greedy algorithm may not perform well in general, but when set function $f$ is monotone
%and submodular, it provides an approximation guarantee, as shown by the following classic
%theorem. Since this is a crucial theorem for our algorithm design, we reproduce the proof below.
%
%\wei{This is the citation for the general greedy approximation when we could assign
%    different weights to the nodes: \cite{mossel2007}
%}


\begin{restatable}{theorem}{adagreedy} \label{thm:AdaGreedy}
	Let $\pi^{\ag}$ represents the policy corresponding to the \alg{AdaGreedy} algorithm. 
	For any $\varepsilon > 0$ and $\ell > 0$, 
		if we use $R=\lceil 31 k^2n\log(2kn^{\ell+1} T)/\varepsilon^2 \rceil$ simulations
		for each influence spread estimation, then
		with probability at least $1-\frac{1}{n^\ell}$, 
	\begin{equation*}
f_{\avg}(\pi^{\ag}) \geq \left(1 - e^{-(1-\frac{1}{e})}-\varepsilon \right) f_{\avg}(\pi^*).
\end{equation*}
 In this case, the total running time for $T$-round \alg{AdaGreedy}
 	is $O(k^3\ell Tn^2m\log(n T)/\varepsilon^2)$.
\end{restatable}





%\begin{theorem}
%    Fix any $\alpha \geq 1$. If $f(\cdot)$ is adaptive monotone and adaptive submodular with respect to the distribution $f(\pi)$, 
%    and $\pi$ is an $\alpha$-approximate greedy policy, then for all policies $\pi^*$
%    
%    % Let $\cS = \{S_1,S_2,...,S_T\}$, 
%    %     where $S_i$ is selected by policy $\pi$ and previous records $\psi$ and $|S_i| \leq k$.
%    % $\pi^* \in argmax_{|\cS| \leq k}\; \rho(\cS)$ be the set maximizing
%    % $f(\pi)$ among all super multi-sets with size at most $k$.
%    % If set function $\rho$ is monotone and submodular and $\rho({\emptyset,\emptyset,...,\emptyset}) = 0$,
%    % then for the set $S^g$ computed by Greedy$(k; \rho)$, we have
%    
%    \begin{equation}
%    f(\pi^g) \geq (1 - \frac{1}{e^{\alpha}}) f(\pi^*).
%    \end{equation}
%    
%    where $e$ is the base of natural logarithm.
%\end{theorem}
%

%\wei{
%    There is an algorithm design problem. 
%    How to use RR-set (Reverse Reachable set) approach to efficiently do ARIM, and the idea
%    is to reuse the RR-sets of the first round to all later rounds.
%    For RR-set algorithm, please use the IMM algorithm in \cite{tang15}, which is also based
%    on prior work \cite{tang14,BorgsBrautbarChayesLucier}.
%}


==> sec_wrimm.tex <==
\wei{The statement and the proof of the following lemma is very confusing. Need significant revision of this lemma.
	This lemma is supposed to be the one for the NodeSelection procedure. But the NodeSelection procedure for
	the within-round algorithm seems to be missing!
	Similarly, Lemma~\ref{lem:crtime} should be re-written in the same way.
}

\begin{lemma} \label{lem:wrrtime}
	In the $t$-th round, node selection algorithm \alg{\WRNS} returns the multi-round sets $\cS_t$ which covers the multi-round RR set with $(1 - \frac{1}{e})$-approximate optimal solution. Its execution time is $O(kn + \sum_{\cR \in \cM} |\cR|)$.
\end{lemma}

\begin{proof}
	In $t$-th round, node selection algorithm \alg{\WRNS} is the multi-round RR set implementation of the \alg{\WRGreedy}.
	Due to the property of monotone and submodular, we know the greedy soluction returns a $(1-1/e)$-approximate solution.
	
	About time complexity, in each iteration, it takes $O(\sum_{\cR \in \cM} |\cR|)$ to generate the count array $c[(u, t)]$ and RR set link $RR[(u, t)]$ for each node in lines \ref{line:wrgen1} and \ref{line:wrgen2} of \alg{\WRNS}.
	In next $k$ seed selection in $t$-th round, every time it takes $O(n)$ for every avaliable seed with the maximum influence, and so the total time is $O(kn)$.
	The rest part of \alg{\WRNS} adjusts the $c[(u, t)]$ and $covered[\cR]$ (from lines \ref{line:wrfor2} to \ref{line:wrfor3}).
	While $v$ is a chosen seed, each multi-round RR set is traversed at most once for updating both $c[(u, t)]$ and $covered[\cR]$, so it takes $O(\sum_{\cR \in \cM} |\cR|)$ for the rest part.
	So, in $t$-th round, the total execution time of $\alg{\WRNS}$ is $O(kn + \sum_{\cR \in \cM} |\cR|)$.
\end{proof}

For within-round non-adaptive algorithm based on multi-round RR set, we actually estimate the conditional marginal reward for every round, so let
\begin{align*}
\nu_t(\cS_t) &= n \cdot \E[\I\{ \cS_t \cap \cR_t \ne \emptyset \mid \cS^{t-1} \cap \cR^{t-1} = \emptyset \} \\
&= \frac{\rho(\cS^{t-1}\cup \cS_t) - \rho(\cS^{t-1})}{\Pr\{(\cS^{t-1} \cap \cR^{t-1} = \emptyset\}},
\end{align*}
where $\nu_t$ denotes the conditional marginal reward in round $t$.
Note that the interpretation of the above formula means that, we uniformly at random select a root $v$
from the nodes set $V$, generate multi-round RR set for all $t$ rounds $(\cR_1, \ldots, \cR_t)$, and
then check the condition $\cS^{t-1} \cap \cR^{t-1} = \emptyset$: if the condition holds, we use 
$\cR_t$ as a valid RR set for round $t$; if the condition does not hold, this multi-round RR set
is invalid and we should remove it and re-sample another root from scratch, and repeat this process until a valid RR set is found.
Then the definition of $\nu_t(\cS_t)$ above corresponds to the valid RR set generated in this way.
For convenience, we remove the subscript $t$ from $\nu_t$ since it is clear that we are working on the
$t$-th round.

From now on, we focus on the analysis for round $t$ of the within-round algorithm \alg{\WRIMM}.
For this purpose, we assume that for the first $t-1$ rounds, the seed sets $\cS^o_1, \ldots, \cS^o_{t-1}$
have been selected and fixed. 
Moreover, the RR sets used for selecting these seed sets in \alg{\WRIMM} have also been fixed, and
after the first $t-1$ rounds, the remaining roots $Root_{t-1}$ to be used for round $t$ is also
fixed.

Let $\cS_t^*$ be the optimal solution of $\nu(\cS_t)$, so $\cS_t^* = \argmax_{\cS_t \subseteq \cV_t, |\cS_t| \leq k} \nu(\cS_t)$, and  $\OPT_t = \nu(\cS_t^*)$. 	
In the $t$-th round, for a given seed set $\cS_t$ and a given collection of RR sets $\cM$, 
we use 	$\hat{\nu}(\cS_t, \cM)$ to denote the random estimation of $\nu(\cS_t)$ based on $\cM$, i.e.
$\hat{\nu}(\cS_t, \cM) = n\cdot \sum_{\cR\in \cM} \I\{\cS_t \cap \cR \ne \emptyset \}
/ |\cM| $.
For the analysis of algorithm \alg{\WRIMM}, we consider two specific collections of RR sets,
$\cM_0$ and $\cM_1$,
where $\cM_0$ is the collection of valid RR sets generated in round $t$ based on the condition
$\cS^{t-1} \cap \cR^{t-1} = \emptyset$, as described above; and
$\cM_1$ is the actual RR sets generated by \alg{\WRIMM} using 
the remaining roots from the previous round, $Root_{t-1}$ in approximation of the conditional distribution of the RR sets.
Then by Lemma~\ref{lem:wrimm}, we can see that $\hat{\nu}(\cS_t, \cM_0)$ is an unbiased estimator
of $\nu(\cS_t)$, while  $\hat{\nu}(\cS_t, \cM_1)$ is an approximation of $\hat{\nu}(\cS_t, \cM_0)$
but it may not be an unbiased estimator for $\nu(\cS_t)$.

%Note that in our  algorithm \alg{\WRIMM}, we use the remaining roots from the previous round, $Root_{t-1}$, 
%	to generate RR sets for round $t$ in approximation of the conditional distribution of the RR sets
%	(with the condition $\cS^{t-1} \cap \cR^{t-1} = \emptyset$).
%Therefore, let $\cM_1$ be the actual RR sets generated from the $Root_{t-1}$, and 
%	$\hat{\nu}'(\cS_t, \cM_1)$ be the estimate of $\nu(\cS_t)$ under such RR sets.
%That is, $\hat{\nu}'(\cS_t, \cM_1) = n\cdot \sum_{\cR\in \cM_1} \I\{\cS_t \cap \cR \ne \emptyset \}
%/ |\cM_1| $.
%
%	For an $\varepsilon > 0$, we have say that a solution $\cS_t$ is bad under $\varepsilon$,
%	if $\nu(\cS_t)< (1- 1/e - \varepsilon) \cdot \OPT_t$. 
%

%	and $\omega$ is a random sample in space $\Omega$. Let $S_t^*$ be the optimal solution of $\nu(S_t)$, so $S_t^* = \argmax_{S_t \subset V, |S_t| \leq k} \nu(S_t)$, and  $\OPT_t = \nu(S_t^*)$. For a random sample $\omega \in \Omega$, let $\hat{S}_t^g(\omega)$ be the solution of the greedy algorithm of $\hat{\nu}(\cdot, \omega)$. 
For an $\varepsilon > 0$, we have a bad solution $\cS_t$ under $\varepsilon$, if $\nu(\cS_t)< (1- 1/e - \varepsilon) \cdot \OPT_t$. 
%	However, in practice, the within-round algorithm \alg{\WRIMM} randomly selects the root from the remaining roots after the previous $t-1$ rounds for multi-round RR set generation, denoted as $\hat{\nu}'(\cS_t, \cM_1)$. 
%	The real conditional marginal influence spread function is the expectation of $\hat{\nu}'(\cdot, \omega)$, denoted as $\upsilon(\cdot)$. 
Next, we give the theoretical guarantee about the approximate solution of the greedy algorithm. 

%\begin{lemma} \label{lem:wrtime}
%	For each round, every iteration of \alg{\WRIMM} returns the multi-round sets $\cS$ which covers the multi-round RR set with $1-\frac{1}{e}$ rate of optimal $\cS^*$. The execution time is $O(kn + \sum_{\cR \in \cM} |\cM|)$ for each iteration.
%\end{lemma}
%
%\begin{proof}
%	Each iteration of \alg{\WRIMM} is the multi-round RR set implementation of the \alg{\WRGreedy}.
%	Due to the property of partition matroid, we know the greedy soluction returns a $\frac{1}{2}$-approximate solution.
%	
%	About time complexity, in each iteration, it takes $O(\sum_{\cR \in \cM} |\cM|)$ to generate each multi-round RR set in lines \ref{line:csample1} and \ref{line:cgsample1} of \alg{\CRIMM}.
%	In next $Tk$ round, every time it takes $O(Tn)$ for every avaliable seed with the maximum influence,
%	and so the total time is $O(T^2kn)$.
%	The rest part of \alg{\CRIMM} adjusts the $F_\cM(\cdot)$ which counts the number of covered multi-round RR of each node, and the $\cM$ which saves the multi-round RR of each node. 
%	While $v$ is a chosen seed, each multi-round RR set is traversed at most once for updating both  $F_\cM(\cdot)$ and $\cM$, so it takes $O(\sum_{\cR \in \cM} |\cM|)$ for the rest part.
%	So, the total execution time of each iteration $\alg{\CRIMM}$ is $O(T^2kn + \sum_{\cR \in \cM} |\cM|)$.
%	
%\end{proof}

\begin{lemma} \label{lem:wrerror}
	For any $\varepsilon$, $\varepsilon_1 \in (0, \varepsilon/(1-1/e))$, and any $\delta_1, \delta_2 > 0$,
	if (a) $\Pr\{\hat{\nu}(\cS_t^*, \cM_1)) \geq (1 - \varepsilon_1) \cdot \OPT_t\} \geq 1 - \delta_1$, and
	(b) for every bad $\cS_t$ under $\varepsilon$, 
	$\Pr\{\hat{\nu}(\cS_t, \cM_1)) \geq (1 - \frac{1}{e})(1 - \varepsilon_1) \cdot \OPT_t\} \leq \delta_2 / {\binom{n}{k}}$, then the greedy solution $\cS_t^o(\cM_1)$ on the function
	$\hat{\nu}(\cdot, \cM_1)$ is a $(1 - \frac{1}{e} - \varepsilon)$-approximate solution 
	to $\OPT_t$ with at least $1-\delta_1-\delta_2$ probability.
\end{lemma}

\begin{proof}
	Note that $\hat{\nu}(\cS_t, \cM_1) = n\cdot \sum_{\cR\in \cM_1} \I\{\cS_t \cap \cR \ne \emptyset \}
	/ |\cM_1| $.
	Since function $\I\{\cS_t \cap \cR \ne \emptyset \}$ with respect to $\cS_t$ is monotone and 
	submodular, we know that $\hat{\nu}(\cS_t, \cM_1)$ is monotone and submodular with 
	respect to $\cS_t$. Therefore we have
	\begin{equation}
	\hat{\nu}(\cS_t^o(\cM_1), \cM_1) \geq \left(1 - \frac{1}{e} \right) \cdot \hat{\nu}(\cS_t^*, \cM_1) \nonumber.
	\end{equation}
	Due to condition $(a)$, we know that
	\begin{equation}
	\hat{\nu}(\cS_t^o(\cM_1), \cM_1) \geq \left(1- \frac{1}{e} \right)\cdot \hat{\nu}(\cS_t^*) \geq 
	\left(1- \frac{1}{e} \right)(1 - \varepsilon_1) \cdot \OPT_t \nonumber,
	\end{equation} 
	with at least $1-\delta_1$ probability.
	
	Due to condition $(b)$, since there are at most ${\binom{n}{k}}$ bad $k$-seed sets in round $t$,
	we know that the probability of existing a bad solution $\cS_t$ under $\varepsilon$ 
	satisfying $\hat{\nu}(\cS_t, \cM_1)) \geq (1 - \frac{1}{e})(1 - \varepsilon_1) \cdot \OPT_t$
	is 
	at most $\delta_2$.
	Therefore, by union bound, with probability at least $1-\delta_1-\delta_2$, 
	$\cS_t^o(\cM_1)$ is not a bad solution, that is, 
	${\nu}(\cS_t^o(\cM_1)) \geq (1- 1/e - \varepsilon) \cdot \OPT_t$.
\end{proof}

%\begin{lemma} \label{lem:wrerror}
%	For any $\varepsilon >0$, $\varepsilon_1 \in (0, \varepsilon/(1-1/e))$, and any $\delta_1, \delta_2 > 0$,
%	if (a) $\Pr_{\cM_1}\{\hat{\nu}'(\cS_t^*, \cM_1) \geq (1 - \varepsilon_1) \cdot \OPT_t\} \geq 1 - \delta_1$;
%	(b) for any bad solution $\cS_t$ under $\varepsilon$, $\Pr_{\cM_1}\{\hat{\nu}'(\cS_t, \cM_1) \geq (1 - \frac{1}{e}) (1 - \varepsilon_1) \cdot \OPT_t\} \leq \delta_2 / {\binom{n}{k}}$;
%	(c) for any $\cM_1$, $\hat{\nu}'(\cS_t, \cM_1)$ is a nonnegative, monotone and submodular function on $\cS_t$, then the greedy solution of $\cS_t^o$ is a $(1 - \frac{1}{e})$-approximate solution with probability at least
%	$1-\delta_1-\delta_2$ .
%\end{lemma}
%%\begin{lemma} \label{lem:wrerror}
%%	For any $\varepsilon$, $\varepsilon_0 >0$, $\varepsilon_1 \in (0, \varepsilon/(1-1/e))$, and any $\delta_0, \delta_1, \delta_2 > 0$,
%%	if (a) $\Pr\{\hat{\nu}'(S_t^*) \geq (1 - \varepsilon_0) \cdot \hat{\nu}(S_t^*)\} \geq 1 - \delta_0$;
%%	(b) $\Pr\{\hat{\nu}(S_t^*) \geq (1 - \varepsilon_1) \cdot \OPT_t\} \geq 1 - \delta_1$.
%%	(c) $\Pr\{\hat{\nu}(S_t^*) \leq (1 + \varepsilon_1) \cdot \OPT_t\} \geq 1 - \delta_1$.
%%	(d) $\Pr\{\hat{\nu}'(S_t) \geq (1 - \frac{1}{e}) (1 - \varepsilon_0)(1 - \varepsilon_1) \cdot \OPT_t\} \leq \delta_2 / {\binom{n}{k}}$;
%%	(e) For any $S_t$, $\hat{\nu}'(S_t)$ is a coditional random esitimation which holds monotone and submudolar, and the greedy soluction of $S_t^g$ holds at least $(1 - \frac{1}{e})$-approximate solution with $1-\delta_0-\delta_1-\delta_2$ probability.
%%\end{lemma}
%\begin{proof}
%	Since $\hat{\nu}'(S_t)$ holds monotone and submudolar, by lemma \ref{lem:wrerror}, we know
%	\begin{equation}
%	\hat{\nu}'(S_t^g) \geq (1-\frac{1}{e}) \cdot \hat{\nu}'(S_t^*) \nonumber.
%	\end{equation}
%	Due to condition $(a), (b)$, we know
%	\begin{align*}
%	\hat{\nu}'(S_t^g) \geq (1-&\frac{1}{e}) \cdot \hat{\nu}'(S_t^*) \geq (1-\frac{1}{e})(1 - \varepsilon_0) \cdot \hat{\nu}(S_t^*) \\ \geq  &(1-\frac{1}{e})(1 - \varepsilon_0)(1 - \varepsilon_1) \cdot \OPT_t \nonumber,
%	\end{align*} 
%	with at least $1-\delta_0-\delta_1$ probability.
%	
%	Due to condition $(c)$, we know that a bad $S_t$ causing $\hat{\nu}'(S_t, \omega) \geq (1-\frac{1}{e})(1 - \varepsilon_0)(1 - \varepsilon_1) \cdot \OPT_t$ with at most $\delta_2$ probability.
%	Because of at most ${\binom{n}{k}}$ bad samples for $k$ seeds in every round,
%	the probability of each bad $S_t$ is at most $\delta_2/{\binom{n}{k}}$.
%	By using union bound, we know that ${\nu}(S_t^g(\omega)) \geq (1-\frac{1}{e}-\varepsilon) \cdot \OPT_t$ with at least $1-\delta_0-\delta_1-\delta_2$ probability.
%	
%\end{proof}

From Lemma \ref{lem:randhistory} to \ref{lem:wrrnum1}, 
we show how to estimate the number of RR sets of \WRIMM.
Since we can not directly estimate $\hat{\nu}(\cS_t, \cM_1)$, we study the relation between $\hat{\nu}(\cS_t, \cM_1)$ and $\hat{\nu}(\cS_t, \cM_0)$ by Lemma \ref{lem:randhistory} and \ref{lem:randhistory2},
and the esitimate $\hat{\nu}(\cS_t, \cM_0)$ by Lemma \ref{lem:wrrnum}. 
Finally, we can estimate the number of RR sets of {\WRIMM} by Lemma \ref{lem:wrrnum1}. 



We want the following results.
Let $P$ be a distribution on the set of nodes $V$, i.e. for all $v\in V$, $P(v) \ge 0$, and 
$\sum_{v\in V} P(v) = 1$.
For two distributions $P_1$ and $P_2$ on $V$, we say that $P_1$ is $\eta$-close to $P_2$, 
if for all $v\in V$, $|P_1(v) - P_2(v)| \le \eta \cdot P_2(v)$.
\wei{I am not sure whether we want relative or absolute closeness here. Let's try relative closeness
	first.}

For the \alg{\WRIMM} algorithm, let $\cH_{t-1}$ be the history of all the randomness occurred in rounds
$1, 2, \ldots, t-1$ in the algorithm, namely the randomness used to generate RR sets in these rounds.
Thus, history $\cH_{t-1}$ determines the seed sets $\cS_1, \ldots, \cS_{t-1}$, and the remaining
roots $Root_{t-1}$.
Let $P_{t,1}(\cH_{t-1})$ be the distribution on $V$ generated based on $Root_{t-1}$, and this
distribution is used to generate the RR sets $\cM_1$ in round $t$ in the \alg{\WRIMM} algorithm.
Let $P_{t,0}(\cH_{t-1})$ be the distribution on $V$ generated based on the condition
$\cS^{t-1} \cap \cR^{t-1} = \emptyset$, that is, we uniformly at random pick a $v\in V$, then
generates RR sets $\cR_1, \ldots, \cR_{t-1}$, and if for all $j \in [t-1]$, 
$\cS_j \cap \cR_j = \emptyset$, then $v$ is one sample in the distribution of $P_{t,0}(\cH_{t-1})$;
otherwise, we throw away $v$ and redo the above process until we find a $v$ satisfying the above
condition.
In this sense, $P_{t,0}(\cH_{t-1})$ is the ideal distribution we want the roots of RR sets in round $t$
to be selected from, while $P_{t,1}(\cH_{t-1})$ is an approximation of $P_{t,0}(\cH_{t-1})$.

Let $\xi_t(\eta)$ be the event that $P_{t,1}(\cH_{t-1})$ is $\eta$-close to $P_{t,0}(\cH_{t-1})$.
Let $\xi(\eta) = \xi_1(\eta) \cap \cdots \cap \xi_T(\eta)$.
We first want a result showing that event $\xi(\eta)$ holds with high probability, if each round
generates enough number of RR sets.

%\wei{The following will be my new attempt.
%I think the original proof structure is good in general, but I want to replace it with absolute error
%	to incorporate $\OPT_t$ later.
%I also want to use conditional probability and induction.
%The following setup and Lemma~\ref{lem:errorinduction} is the general result to be used for the 
%	induction.
%Hope that you can see the correspondence with our algorithm \alg{\WRIMM}.
%The statement of Lemma~\ref{lem:errorinduction} may not be correct yet, especially I am not sure about
%	the absolute error term for $\tQ$.
%}
%
%\begin{proposition}[Hoeffding Inequality]
%Let $X_1, \ldots, X_n$ be independent random variables bounded in the interval $[0,1]$.
%Let $\bar{X} = \frac{1}{n} \sum_{i=1}^n X_i$.
%Then
%\begin{align*}
%	\Pr\{|\bar{X} - \E[\bar{X}]| \ge t \} \le 2 e^{-2nt^2}.
%\end{align*}
%\end{proposition}

\wei{
	The following is my attempt to derive a general condition to be used for the induction steps between different rounds (Lemma~\ref{lem:errorinduction}).
	However, so far it is only partially successful.
	What it achieves is (a) addressing the approximation ratio related to the conditional probability
	(derivations for Eq.~\eqref{eq:derivecond1} and \eqref{eq:derivecond2})); and
	(b) deriving the amplification of approximation ratio, from $\eta$ to $3\eta$, which could be used in the induction steps for
	multiple round analysis.
	However, it has several serious issues.
	First, it is still on the pure relative error, such that the $\ttheta$ bound depending on some minimum probability. I am not sure how to connect it to $\OPT_t$.
	Second, the amplification of relative error grows exponentially. By the following derivation, if at the beginning the relative error is $\eta$, then
	at the end the relative error must be greater than $2\eta$, and I used $3\eta$ for convenience. 
	This implies that if we want to apply it to induction on $T$ rounds, then the error at the last round can only be bounded by $3^T \eta$.
	I am not sure if such an exponential amplification is avoidable, and if not, it may kill the entire approach.
}

Let $P$ be a distribution over node set $V$.
Let $\tP$ be another distribution on $V$ that is $\eta$ close to $P$.
Let $Z$ denote the random sample of $V$ according to the distribution $P$, and
$\tZ$ denote the random sample of $V$ according to distribution $\tP$.
For every $v\in V$, let $F(v)$ be a Bernoulli random variable called filter variable, and
$F(v)$'s are mutually independent, and they are independent of sampling events, i.e.
independent of $Z$ and $\tZ$.

We define a conditional distribution $Q$ to be the distribution of $P$ conditioned on the filter $F$,
that is, if a sample according to $P$ passes the filter, then we keep this sample; otherwise,
we re-sample again.
Mathematically, for every $v\in V$, $Q(v) = \Pr\{Z = v \wedge F(Z) \mid F(Z) \} = \frac{P(v)\cdot \E[F(v)]}{\E[F(Z)]}$.
Finally, define another conditional distribution $\tQ$ as follows.
Let $\ttheta$ be a positive integer, and $\tZ_1, \tZ_2, \ldots, \tZ_{\ttheta}$ be $\ttheta$ 
i.i.d.\ samples according to distribution $\tP$.
Let $\cF$ be the filtered multi-set of the above samples, i.e. $\cF = \{\tZ_j\mid F(\tZ_j) = 1 \}$. 
Note that $\cF$ is a multi-set, that is, we keep all copies of the same node samples in the set;
also $\cF$ is a random multi-set, and its randomness comes from both the randomness of
the samples $\tZ_1, \ldots, \tZ_{\ttheta}$ and the randomness of the filter $F(\cdot)$.
Finally, we define another distribution $\tQ$ to be the result of a uniform sampling
from $\cF$, that is, for all $v\in V$, 
\begin{align*}
\tQ(v) & = \frac{1}{|\cF|} \sum_{\tZ \in \cF} \I\{ \tZ = v \} \\
& = \frac{\sum_{j=1}^{\ttheta} \I\{\tZ_j = v \} \cdot F(\tZ_j)}
{\sum_{j=1}^{\ttheta} F(\tZ_j) }.
\end{align*}

\wei{The correspondence between the above abstract formulation and our {\WRIMM} algorithm should not be very hard to see.
	\begin{itemize}
		\item $P$ corresponds to the true root distribution for a round $t$, i.e. $P_{t,0}(\cH_{t-1})$.
		
		\item $\tP$ corresponds to the actual root distribution from $Root_{t-1}$ used by the algorithm, i.e. $P_{t,1}(\cH_{t-1})$.
		
		\item $Z$ corresponds to a root sample drawn from $P_{t,0}(\cH_{t-1})$, and $\tZ$ corresponds to a root sample drawn from
		$P_{t,1}(\cH_{t-1})$.
		
		\item Filter $F(v)$ corresponds to the RR-set generated from root $v$ intersecting with the round $t$ seed set $\cS_t$, so $v$ would be left
		as a root in $Root_t$.
		
		\item $\ttheta$ is the number of RR-sets needs to be generated after $\cS_t$ is determined, to generate $Root_t$.
		
		\item $\tZ_1, \tZ_2, \ldots, \tZ_{\ttheta}$ corresponds to the $\ttheta$ roots sampled from $Root_{t-1}$.
		
		\item $\cF$ corresponds to the root multi-set $Root_{t}$, which is obtained by removing those roots in $\tZ_1, \tZ_2, \ldots, \tZ_{\ttheta}$ that
		do not intersect with $\cS_t$, i.e. $F(\tZ_j) = 0$.
		
		\item $Q$ corresponds to the true root distribution for the next round, i.e. $P_{t,0}(\cH_{t})$. 
		
		\item $\tQ$ corresponds to the root distribution from $Root_t$.
	\end{itemize}
	
	Finally, the following lemma can be interpreted as if $P_{t,1}(\cH_{t-1})$ is $\eta$-close $P_{t,0}(\cH_{t-1})$, then 
	for large enough sample size $\ttheta$, $P_{t,1}(\cH_{t})$ is $3\eta$-close $P_{t,0}(\cH_{t})$ with probability at least $1-\delta_0$.
}

\begin{lemma} \label{lem:errorinduction}
	For $\delta_0 > 0$, if $\tP$ is $\eta$-close to $P$, 
	then when 
	\begin{equation} \label{eq:tthetaLB}
	\ttheta \ge \frac{3(1+\eta)^2}{(\eta' - \eta)^2 (1-\eta) \min_{v\in V} P(v) \cdot \E[F(v)]} \ln\left(\frac{2n}{\delta_0}\right) 
	\end{equation}
	where $\eta' = \frac{3\eta}{2+3\eta}$ $\tQ$ is $3\eta$-close to $Q$ 
	with probability at least $1-\delta_0$.
\end{lemma}
\begin{proof}
	Fix a node $v\in V$.
	For every $j \in [\ttheta]$, define Bernoulli random variable $\tY_j = \I\{\tZ_j = v \} \cdot F(\tZ_j) $.
	Then $\E[\tY_j] = \E[\I\{\tZ_j = v \} \cdot F(\tZ_j)] = 
	\sum_{u\in V} \tP(u) \E[\I\{u = v \} \cdot F(u)] = \tP(v) \cdot \E[F(v)]$.
	%Note that the above derivation users the fact that for any fixed $v$, $\I\{\tZ_j = v \}$ is independent
	%	of $F(v)$.
	
	For $\eta' > \eta$, we have the following (we will fix the actual value of $\eta'$ later):
	\begin{align}
	& \Pr \left\{ \sum_{j=1}^{\ttheta} \I\{\tZ_j = v \} \cdot F(\tZ_j) \ge (1+\eta') \ttheta \cdot  P(v)\cdot \E[F(v)] \right\} \nonumber \\
	&\le \Pr \left\{ \sum_{j=1}^{\ttheta} \I\{\tZ_j = v \} \cdot F(\tZ_j) \ge \frac{1+\eta'}{1+\eta} \ttheta \cdot  \tP(v)\cdot \E[F(v)] \right\} \nonumber \\
	& = \Pr \left\{ \sum_{j=1}^{\ttheta} \tY_j - \ttheta \E[\tY_1] \ge \frac{\eta' - \eta}{1+\eta} \ttheta \cdot \E[\tY_1] \right\}  \nonumber \\
	& \le \exp\left( - \frac{\left( \frac{\eta' - \eta}{1+\eta} \right)^2}{2+\frac{2}{3}\cdot \frac{\eta' - \eta}{1+\eta}} \ttheta \cdot \E[\tY_1]  \right)  \nonumber \\
	& \le \exp\left( - \frac{1}{3} \cdot \left( \frac{\eta' - \eta}{1+\eta} \right)^2 \left(\frac{3(1+\eta)^2}{(\eta' - \eta)^2 \E[\tY_1]} \ln\left(\frac{2n}{\delta_0} \right) \right) \cdot \E[\tY_1]  \right)  \nonumber \\
	& = \frac{\delta_0}{2n},  \label{eq:numeratorUB}
	\end{align}
	where the last inequality uses Eq.~\eqref{eq:tthetaLB} and the fact that $(1-\eta) \min_{v\in V} P(v) \cdot \E[F(v)] \le \min_{v\in V} \tP(v) \cdot \E[F(v)] \le \E[\tY_1]$.
	Similarly, we have
	\begin{align}
	& \Pr \left\{ \sum_{j=1}^{\ttheta} \I\{\tZ_j = v \} \cdot F(\tZ_j) \le (1-\eta') \ttheta \cdot  P(v)\cdot \E[F(v)] \right\} \nonumber \\
	&\le \Pr \left\{ \sum_{j=1}^{\ttheta} \I\{\tZ_j = v \} \cdot F(\tZ_j) \le \frac{1-\eta'}{1-\eta} \ttheta \cdot  \tP(v)\cdot \E[F(v)] \right\} \nonumber \\
	& = \Pr \left\{ \sum_{j=1}^{\ttheta} \tY_j - \ttheta \E[\tY_1] \le -\frac{\eta' - \eta}{1-\eta} \ttheta \cdot \E[\tY_1] \right\}  \nonumber \\
	& \le \exp\left( -  \frac{(\eta' - \eta)^2}{2(1-\eta)^2} \ttheta \cdot \E[\tY_1]  \right)  \nonumber \\
	& \le \exp\left( - \frac{(\eta' - \eta)^2}{2(1-\eta)^2}  \left(\frac{3(1+\eta)^2}{(\eta' - \eta)^2 \E[\tY_1]} \ln\left(\frac{2n}{\delta_0} \right) \right) \cdot \E[\tY_1]  \right)  \nonumber \\
	& \le \frac{\delta_0}{2n}.  \label{eq:numeratorLB}
	\end{align}
	
	Combining inequalities~\eqref{eq:numeratorUB} and~\eqref{eq:numeratorLB}, and taking union bound for all $v$, we know that with at least 
	probability $1 - \delta_0$, for all $v$, 
	\[
	(1-\eta') \ttheta \cdot  P(v)\cdot \E[F(v)] \le \sum_{j=1}^{\ttheta} \I\{\tZ_j = v \} \cdot F(\tZ_j) \le (1+\eta' ) \ttheta \cdot  P(v)\cdot \E[F(v)].
	\]
	
	Summing up the above inequalities over all $v\in V$, we have
	\[
	(1-\eta') \ttheta \E[F(Z)] \le \sum_{j=1}^{\ttheta} F(\tZ_j) \le (1+\eta' ) \ttheta \E[F(Z)].
	\]
	Under the above condition, we can show that 
	\begin{align}
	&\tQ(v) = \frac{\sum_{j=1}^{\ttheta} \I\{\tZ_j = v \} \cdot F(\tZ_j)}
	{\sum_{j=1}^{\ttheta} F(\tZ_j) } \nonumber \\
	&\le \frac{(1+\eta' ) \ttheta \cdot  P(v)\cdot \E[F(v)]}
	{(1-\eta') \ttheta \E[F(Z)] } \nonumber \\
	& = \frac{1+\eta'}{1-\eta'} Q(v) = \left(1 + \frac{2\eta'}{1-\eta'}  \right) Q(v). \label{eq:derivecond1}
	\end{align}
	
	\begin{align}
	&\tQ(v) = \frac{\sum_{j=1}^{\ttheta} \I\{\tZ_j = v \} \cdot F(\tZ_j)}
	{\sum_{j=1}^{\ttheta} F(\tZ_j) }  \nonumber \\
	&\ge \frac{(1-\eta' ) \ttheta \cdot  P(v)\cdot \E[F(v)]}
	{(1+\eta') \ttheta \E[F(Z)] } \nonumber \\
	& = \frac{1-\eta'}{1+\eta'} Q(v) = \left(1 - \frac{2\eta'}{1 + \eta'}  \right) Q(v). \label{eq:derivecond2}
	\end{align}
	
	Since $\frac{2\eta'}{1-\eta'} \ge \frac{2\eta'}{1+\eta'}$, we want to set $\frac{2\eta'}{1-\eta'} $
	to $3\eta$.
	Then we need to set $\eta' = \frac{3\eta}{2+3\eta} $.
	Note that when $\eta < 1/3$, we have $\eta' > \eta$, so it satisfies the requirement.
	%\begin{align*}
	%&|\tQ(v) - Q(v)| \\
	%& = \left| \frac{\sum_{j=1}^{\ttheta} \I\{\tZ_j = v \} \cdot F(\tZ_j)}{\sum_{j=1}^{\ttheta} F(\tZ_j) } 
	%	-   \frac{\ttheta P(v)\cdot \E[F(v)]}{\ttheta\E[F(Z)]} \right|	 \\
	%& = \left| \frac{\left(\sum_{j=1}^{\ttheta} \I\{\tZ_j = v \} \cdot F(\tZ_j) \right)(\ttheta\E[F(Z)])
	%	- \left( \sum_{j=1}^{\ttheta} F(\tZ_j) \right)(\ttheta P(v)\cdot \E[F(v)])}
	%	{\left( \sum_{j=1}^{\ttheta} F(\tZ_j) \right) \cdot \ttheta\E[F(Z)]}
	%\right| \\
	%& \le \frac{\sum_{j=1}^{\ttheta} \I\{\tZ_j = v \} \cdot F(\tZ_j) }{\left( \sum_{j=1}^{\ttheta} F(\tZ_j) \right) \cdot \ttheta\E[F(Z)]} \left| \sum_{j=1}^{\ttheta} F(\tZ_j) - \ttheta\E[F(Z)]
	%\right | \\
	%& \quad  + \frac{1}{\ttheta\E[F(Z)]} \left|\sum_{j=1}^{\ttheta} \I\{\tZ_j = v \} \cdot F(\tZ_j) 
	%	-  \ttheta P(v)\cdot \E[F(v)] \right|
	%\end{align*}
	%
\end{proof}


\begin{lemma}
	Given any $\eta > 0$, any $\delta_0 > 0$, let 
	\begin{align*}
	\theta^{(0)} = ???,
	\end{align*}
	
	If for every round $t$, the number of RR sets generated in round $t$ is at least $\theta^{(0)}$, then
	with probability at least $1-\delta_0$, event $\xi(\eta)$ holds, i.e.
	\[
	\Pr\{ \xi(\eta) \} \ge 1 - \delta_0,
	\]
	where the probability is taken over all randomness used in all $T$ rounds of the algorithm \alg{\WRIMM}.
\end{lemma}

Next, we want to show that when event $\xi(\eta)$ holds, with high probability the 
estimates $\hat{\nu}(\cS_t^*,\cM_1)$ and $\hat{\nu}(\cS_t^*,\cM_0)$ are close enough, where
$\cM_1$ and $\cM_0$ are RR sets generated in round $t$ based on root distributions
$P_{t,1}(\cH_{t-1})$ and $P_{t,0}(\cH_{t-1})$, respectively.


\begin{lemma}\label{lem:randiff}
	Suppose that $\xi(\eta)$ holds while $\eta > 0$.
	Fix a round $t$ and a history $\cH_{t-1}$ that satisfies $\xi(\eta)$.
	Let $\cM_1$ and $\cM_0$ be the RR sets generated in round $t$ based on root distributions
	$P_{t,1}(\cH_{t-1})$ and $P_{t,0}(\cH_{t-1})$, respectively.
	Given any multi-round RR sets $\cS_t$, we have 
	\[
	\left |\E[X_1^{\cM_1}(\cS_t)\mid \cH_{t-1}] - \E[X_1^{\cM_0}(\cS_t)\mid \cH_{t-1}]  \right | \le \eta \E[X_1^{\cM_0}(\cS_t) \mid \cH_{t-1} ]
	\]
\end{lemma}
\begin{proof}
	Let $\cR_{v,t}$ be a random RR set generated in round $t$ rooted at node $v$.
	Since $\xi(\eta)$ holds, we have that for all $v\in V$, 
	$| P_{t,1}(\cH_{t-1})(v) -  P_{t,0}(\cH_{t-1})(v)| \le \eta P_{t,0}(\cH_{t-1})(v)$.
	Then, we can derive the following:
	\begin{align}
	&\left |\E[X_1^{\cM_1}(\cS_t)\mid \cH_{t-1}] - \E[X_1^{\cM_0}(\cS_t)\mid \cH_{t-1}]  \right | \nonumber \\
	& \quad = \left |\sum_{v\in V} P_{t,1}(\cH_{t-1})(v) \cdot 
	\Pr\{ \cR_{v,t} \cap \cS_t \ne \emptyset \} -  \right. \nonumber \\
	& \quad \quad \left. \sum_{v\in V} P_{t,0}(\cH_{t-1})(v) \cdot 
	\Pr\{ \cR_{v,t} \cap \cS_t \ne \emptyset \} \right | \nonumber \\
	& \quad \le  \sum_{v\in V}  \left | P_{t,1}(\cH_{t-1})(v) -  P_{t,0}(\cH_{t-1})(v) \right| \cdot 
	\Pr\{ \cR_{v,t} \cap \cS_t \ne \emptyset \}  \nonumber \\
	& \quad \le \sum_{v\in V} \eta P_{t,0}(\cH_{t-1})(v)  \cdot 
	\Pr\{ \cR_{v,t} \cap \cS_t \ne \emptyset \} \nonumber \\
	& = \eta \E[X_1^{\cM_0}(\cS_t) \mid \cH_{t-1} ]. \label{eq:meandiff0}
	\end{align}
\end{proof}

\wei{
	The following is my old plan, which may not work.
	I leave it here for now before my new plan work out.
	Instead of the following corollary, I think we want the following relaxed version
	\begin{align}
	& |\E[\hat{\nu}(\cS_t, \cM_1)] - \E[\hat{\nu}(\cS_t, \cM_0)]| \le \eta \cdot \OPT_t. \label{eq:relaxedest}
	\end{align}
	We want the above inequality holds for every bad $\cS_t$ and for the optimal $\cS^*_t$.
	I think that by putting the relative error to be relative to $\OPT_k$ instead of 
	$\E[\hat{\nu}(\cS_t, \cM_0)]$, I hope to avoid the third issue in my note, that is we have
	to be very accurate relative to a very small true value.
	I think the above inequality would carry through for the remaining lemma (perhaps even make them easier).
	
	However, the issue is that if we want find a sufficiently large $\theta$ to prove the above inequality,
	it looks like we cannot go through Lemma~\ref{lem:randiff} and the derivation of 
	Eq.~\eqref{eq:meandiff0}.
	How to prove Inequality~\eqref{eq:relaxedest}?
	
	Actually, the expression of Inequality~\eqref{eq:relaxedest} is not accurate.
	What we really mean is that
	\begin{align}
	& \Pr\{|\E[\hat{\nu}(\cS_t, \cM_1)] - \E[\hat{\nu}(\cS_t, \cM_0)]| \le \eta \cdot \OPT_t \} \ge 1 - \delta_0. \label{eq:relaxedest2}
	\end{align}
	In the above inequality, we need to be clear what are fixed and what are random.
	We assume that the previous seed sets up to round $t-1$, $\cS^{t-1}$ are fixed, so is $\cS_t$ fixed.
	Then $ \E[\hat{\nu}(\cS_t, \cM_0)]$ is a fixed number.
	Moreover, $\cM_1$ is sampled from $Root_{t-1}$, so once $Root_{t-1}$ is fixed, $\E[\hat{\nu}(\cS_t, \cM_1)]$
	is also a fixed number.
	Therefore, when $Root_{t-1}$ is random, $\E[\hat{\nu}(\cS_t, \cM_1)]$ is random due to $Root_{t-1}$.
	For our analysis, I think we need to assume that after seed set $\cS_{t-1}$ is selected in round $t-1$,
	we need to regenerate $\ttheta$ RR-sets $\tR^{t-1}_1, \ldots, \tR^{t-1}_{\ttheta}$ in round $t-1$ to generate $Root_{t-1}$.
	However, generating these RR-sets need $Root_{t-2}$.
	So, in general, we assume that in each round $i \le t-1$, after seed set $\cS_i$ is selected in round 
	$i$, we regenerate $\ttheta$ RR-sets $\tR^{i}_1, \ldots, \tR^{i}_{\ttheta}$ based on the roots
	in $Root_{i-1}$; and use these RR-sets to find $Root_{i}$ --- remove those RR-sets that are covered
	by $\cS_i$, and the set of roots of the remaining RR sets form $Root_{i}$.
	Therefore, $\E[\hat{\nu}(\cS_t, \cM_1)]$ is random, and its randomness is determined by 
	$Root_1, \ldots, Root_{t-1}$, the randomness of which is in turn determined by 
	all those RR sets $\{R^i_j \mid 1\le i \le t-1, 1\le j \le \ttheta\}$.
	Hence, in Inequality~\eqref{eq:relaxedest2}, the probability is taken over all the above randomness.
	
	To prove Inequality~\eqref{eq:relaxedest2}, we want to apply Chernoff bound (or martingale tail bound).
	That means we want to define a series of random variables $Y_j$, such that $\E[Y_j] = \E[\hat{\nu}(\cS_t, \cM_0)]$, and $\E[\hat{\nu}(\cS_t, \cM_1)] = \sum_j Y_j$.
	It looks to me that these $Y_j$'s should be connected with those RR-sets 
	$\{R^i_j \mid 1\le i \le t-1, 1\le j \le \ttheta\}$ in some way. 
	However, I am not clear how to do it now.
}


\begin{corollary} \label{cor:randiff}
	Assume Lemma \ref{lem:randiff} holds, for any multi-round RR set $\cS_t$, we have 
	\begin{align}
	& \E[\hat{\nu}(\cS_t, \cM_1)] \le \E[(1+\eta)\hat{\nu}(\cS_t, \cM_0)] \label{eq:poseta}\\
	& \E[\hat{\nu}(\cS_t, \cM_1)] \ge \E[(1-\eta)\hat{\nu}(\cS_t, \cM_0)] \label{eq:negeta}	
	\end{align}
\end{corollary}
\begin{proof}
	%	We have $\hat{\nu}(\cS_t, \cM_1) = X_1^{\cM_1}(\cS_t)$ and $\hat{\nu}(\cS_t, \cM_0) = X_1^{\cM_0}(\cS_t)$ under histotry condition $\cH_{t-1}$.
	
	$\left |\E[X_1^{\cM_1}(\cS_t)] - \E[X_1^{\cM_0}(\cS_t)  \right | \le \eta \E[X_1^{\cM_0}(\cS_t)]$ under history condition $ \cH_{t-1}$ holds by Lemma \ref{lem:randiff}.
	
	Equation \ref{eq:poseta} is shown as follows:
	\begin{align*}
	& \E[\hat{\nu}(\cS_t, \cM_1)] =  n\E[X_1^{\cM_1}(\cS_t) \mid \cH_{t-1} ]\\
	\le & (1+\eta)n\E[X_1^{\cM_0}(\cS_t) \mid \cH_{t-1} ] = \E[(1+\eta)\hat{\nu}(\cS_t, \cM_0)]
	\end{align*}
	
	Next, we show Equation \ref{eq:negeta} as follows:
	\begin{align*}
	& \E[\hat{\nu}(\cS_t, \cM_1)] =  n\E[X_1^{\cM_1}(\cS_t) \mid \cH_{t-1} ] \\
	\ge & (1-\eta)n\E[X_1^{\cM_0}(\cS_t) \mid \cH_{t-1} ] = \E[(1-\eta)\hat{\nu}(\cS_t, \cM_0)]	
	\end{align*}
\end{proof}

\begin{lemma} \label{lem:randhistory}
	Fix any $\varepsilon_1 >0$ and any $\delta_1 > 0$.
	Suppose  that $\xi(\eta)$ holds for some $\eta < \varepsilon_1$.
	Fix a round $t$ and a history $\cH_{t-1}$ that satisfies $\xi(\eta)$.
	Let $\cM_1$ and $\cM_0$ be the RR sets generated in round $t$ based on root distributions
	$P_{t,1}(\cH_{t-1})$ and $P_{t,0}(\cH_{t-1})$, respectively.
	If we generate at least $\theta^{(1)}$ RR sets in round $t$ as defined below,
	%	\[
	%	\theta^{(1)} = \max{\left(\frac{(2+\frac{2}{3}\gamma_0)n \cdot \ln(4/\delta_1)}{\OPT_t  \cdot \gamma_0^2},  \frac{2n \cdot \ln(4/\delta_1)}{(1-\eta)\OPT_t  \cdot \gamma_0^2}\right)},\\
	%	\]
	\[
	\theta^{(1)}  =	\frac{2n(1+\eta) \cdot \ln(1/\delta_1)}{(\eta-\varepsilon_1)^2\cdot \OPT_t},
	\]
	%	where 
	%	%$\mu_0 =  \E[X_1^{\cM_0}(\cS_t^*) ]$ %$ = \Pr_{v \sim P_{t,0}(\cH_{t-1})}\{ \cS_t^* \cap \cR_{v,t} \ne \emptyset \}$, 
	%	%$\mu_1 = \E[X_1^{\cM_1}(\cS_t^*) ] $, and 
	%	$\gamma_0 =  \frac{ \varepsilon_0 - \eta}{2 - \eta -\varepsilon_0}$,
	then we have
	\[
	\Pr \{ \hat{\nu}(\cS_t^*,\cM_1) < (1-\varepsilon_1)\cdot \OPT_t \}  \le \delta_1.
	\]
\end{lemma}
\begin{proof}
	%	Let $\cR_{v,t}$ be a random RR set generated in round $t$ rooted at node $v$.
	%	Since $\xi(\eta)$ holds, we have that for all $v\in V$, 
	%	$| P_{t,1}(\cH_{t-1})(v) -  P_{t,0}(\cH_{t-1})(v)| \le \eta P_{t,0}(\cH_{t-1})(v)$.
	%	Then, we can derive the following:
	%	\begin{align}
	%	&\left |\E[X_1^{\cM_1}(\cS_t^*)\mid \cH_{t-1}] - \E[X_1^{\cM_0}(\cS_t^*)\mid \cH_{t-1}]  \right | \nonumber \\
	%	& \quad = \left |\sum_{v\in V} P_{t,1}(\cH_{t-1})(v) \cdot 
	%	\Pr\{ \cR_{v,t} \cap \cS_t^* \ne \emptyset \} -  \right. \nonumber \\
	%	& \quad \quad \left. \sum_{v\in V} P_{t,0}(\cH_{t-1})(v) \cdot 
	%	\Pr\{ \cR_{v,t} \cap \cS_t^* \ne \emptyset \} \right | \nonumber \\
	%	& \quad \le  \sum_{v\in V}  \left | P_{t,1}(\cH_{t-1})(v) -  P_{t,0}(\cH_{t-1})(v) \right| \cdot 
	%	\Pr\{ \cR_{v,t} \cap \cS_t^* \ne \emptyset \}  \nonumber \\
	%	& \quad \le \sum_{v\in V} \eta P_{t,0}(\cH_{t-1})(v)  \cdot 
	%	\Pr\{ \cR_{v,t} \cap \cS_t^* \ne \emptyset \} \nonumber \\
	%	& = \eta \E[X_1^{\cM_0}(\cS_t^*) \mid \cH_{t-1} ]. \label{eq:meandiff}
	%	\end{align}
	
	%	Next, we want to $\Pr \{ \hat{\nu}(\cS_t^*,\cM_1) < (1-\varepsilon_1)\cdot \OPT_t \}  \le \delta_1$.
	%	$\E[\hat{\nu}(\cS_t^*, \cM_1)] =  n\E[X_1^{\cM_1}(\cS_t^*) ] \le (1+\eta)n\E[X_1^{\cM_0}(\cS_t^*) ] = (1+\eta)\E[\hat{\nu}(\cS_t^*, \cM_0)]$, and
	%	$\E[\hat{\nu}(\cS_t^*, \cM_1)] =  n\E[X_1^{\cM_1}(\cS_t^*)] \ge (1-\eta)n\E[X_1^{\cM_0}(\cS_t^*) ] = (1-\eta)\E[\hat{\nu}(\cS_t^*, \cM_0)]$ by Equation \ref{eq:meandiff0}. Set $\varepsilon_2 = \eta - \varepsilon_1$, we have
	
	By Corllary \ref{cor:randiff}, $\E[\hat{\nu}(\cS_t^*, \cM_1)] \le (1+\eta)\E[\hat{\nu}(\cS_t^*, \cM_0)]$, and
	$\E[\hat{\nu}(\cS_t^*, \cM_1)] \ge (1-\eta)\E[\hat{\nu}(\cS_t^*, \cM_0)]$. 
	Set $\varepsilon_2 = \eta - \varepsilon_1$, we have
	\begin{align*}
	& \Pr \{ \hat{\nu}(\cS_t^*,\cM_1) < (1-\varepsilon_1)\cdot \OPT_t \}  \le \delta_1 \\
	= & \Pr\left\{\sum_{i=1}^{\theta}X_i^{\cM_1}(\cS_t^*) - \frac{\theta \E[\hat{\nu}(\cS_t^*, \cM_1)]}{n} \geq \right.\\
	& \qquad \left. \frac{\theta}{n} \cdot \left((1-\varepsilon_1)\cdot \OPT_t -  \E[\hat{\nu}(\cS_t^*, \cM_1)]\right) \right\}\\
	\le & \Pr\left\{\sum_{i=1}^{\theta}X_i^{\cM_1}(\cS_t^*) - \frac{\theta \E[\hat{\nu}(\cS_t^*, \cM_1)]}{n} \geq \right.\\
	& \qquad \left. \frac{\theta}{n} \cdot \left((1-\varepsilon_1)\cdot \OPT_t - (1-\eta) \E[\hat{\nu}(\cS_t^*, \cM_0)]\right) \right\}\\
	= & \Pr\left\{\sum_{i=1}^{\theta}X_i^{\cM_1}(\cS_t^*) - \frac{\theta \E[\hat{\nu}(\cS_t^*, \cM_1)]}{n} \geq \frac{\theta}{n} \cdot (\eta-\varepsilon_1)\cdot \OPT_t \right\}\\
	= & \Pr\left\{\sum_{i=1}^{\theta}X_i^{\cM_1}(\cS_t^*) - \frac{\theta \E[\hat{\nu}(\cS_t^*, \cM_1)]}{n} \geq \frac{\theta}{n} \cdot \varepsilon_2\cdot \OPT_t \right\}\\
	= & \Pr\left\{\sum_{i=1}^{\theta}X_i^{\cM_1}(\cS_t^*) - \frac{\theta \E[\hat{\nu}(\cS_t^*, \cM_1)]}{n} \geq  \frac{\varepsilon_2\cdot \OPT_t}{\E[\hat{\nu}(\cS_t^*, \cM_1)]} \cdot \frac{\theta \E[\hat{\nu}(\cS_t^*, \cM_1)]}{n}\right\}\\
	\leq & \exp\left(- \frac{\left(\varepsilon_2\cdot \OPT_t \right)^2}{2\E[\hat{\nu}(\cS_t^*, \cM_1)]} \cdot \theta \cdot 1 / n \right) \\
	\leq & \exp\left(- \frac{\left((\eta - \varepsilon_1)\cdot \OPT_t\right)^2}{2(1+\eta)\OPT_t} \cdot \theta \cdot 1 / n \right) \\
	\leq & \exp\left(- \frac{\left((\eta - \varepsilon_1)^2\cdot \OPT_t\right)}{2n(1+\eta)} \cdot \frac{2n(1+\eta) \cdot \ln(1/\delta_1)}{(\eta-\varepsilon_1)^2\cdot \OPT_t} \right) \\
	\leq & \delta_1. 
	\end{align*}
	
\end{proof}

%\begin{lemma} \label{lem:randhistory}
%Fix any $\varepsilon_0 >0$ and any $\delta_1 > 0$.
%Suppose  that $\xi(\eta)$ holds for some $\eta < \varepsilon_0$.
%Fix a round $t$ and a history $\cH_{t-1}$ that satisfies $\xi(\eta)$.
%Let $\cM_1$ and $\cM_0$ be the RR sets generated in round $t$ based on root distributions
%$P_{t,1}(\cH_{t-1})$ and $P_{t,0}(\cH_{t-1})$, respectively.
%If we generate at least $\theta^{(1)}$ RR sets in round $t$ as defined below,
%\[
%\theta^{(1)} = \max{\left(\frac{(2+\frac{2}{3}\gamma_0)n \cdot \ln(4/\delta_1)}{\OPT_t  \cdot \gamma_0^2},  \frac{2n \cdot \ln(4/\delta_1)}{(1-\eta)\OPT_t  \cdot \gamma_0^2}\right)},\\
%\]
%where 
%%$\mu_0 =  \E[X_1^{\cM_0}(\cS_t^*) ]$ %$ = \Pr_{v \sim P_{t,0}(\cH_{t-1})}\{ \cS_t^* \cap \cR_{v,t} \ne \emptyset \}$, 
%%$\mu_1 = \E[X_1^{\cM_1}(\cS_t^*) ] $, and 
%$\gamma_0 =  \frac{ \varepsilon_0 - \eta}{2 - \eta -\varepsilon_0}$,
%	then we have
%\[
%\Pr\{\hat{\nu}(\cS_t^*,\cM_1) < (1-\varepsilon_0) \hat{\nu}(\cS_t^*,\cM_0) \mid \cH_{t-1} \} \le \delta_1/2.
%\]
%
%\end{lemma}
%\begin{proof}
%Let $\cR_{v,t}$ be a random RR set generated in round $t$ rooted at node $v$.
%Since $\xi(\eta)$ holds, we have that for all $v\in V$, 
%	$| P_{t,1}(\cH_{t-1})(v) -  P_{t,0}(\cH_{t-1})(v)| \le \eta P_{t,0}(\cH_{t-1})(v)$.
%Then, we can derive the following:
%\begin{align}
%	&\left |\E[X_1^{\cM_1}(\cS_t^*)\mid \cH_{t-1}] - \E[X_1^{\cM_0}(\cS_t^*)\mid \cH_{t-1}]  \right | \nonumber \\
%	& \quad = \left |\sum_{v\in V} P_{t,1}(\cH_{t-1})(v) \cdot 
%	\Pr\{ \cR_{v,t} \cap \cS_t^* \ne \emptyset \} -  \right. \nonumber \\
%	& \quad \quad \left. \sum_{v\in V} P_{t,0}(\cH_{t-1})(v) \cdot 
%	\Pr\{ \cR_{v,t} \cap \cS_t^* \ne \emptyset \} \right | \nonumber \\
%	& \quad \le  \sum_{v\in V}  \left | P_{t,1}(\cH_{t-1})(v) -  P_{t,0}(\cH_{t-1})(v) \right| \cdot 
%	\Pr\{ \cR_{v,t} \cap \cS_t^* \ne \emptyset \}  \nonumber \\
%	& \quad \le \sum_{v\in V} \eta P_{t,0}(\cH_{t-1})(v)  \cdot 
%	\Pr\{ \cR_{v,t} \cap \cS_t^* \ne \emptyset \} \nonumber \\
%	& = \eta \E[X_1^{\cM_0}(\cS_t^*) \mid \cH_{t-1} ]. \label{eq:meandiff}
%\end{align}
%
%Next, we want to separate the event 
%	$\hat{\nu}(\cS_t^*,\cM_1) < (1-\varepsilon_0) \hat{\nu}(\cS_t^*,\cM_0) \mid \cH_{t-1}$
%	as two events so that we can apply concentration bounds for each of them.
%To do so, we want to properly select a parameter $c_0$ as follows:
%\begin{align*}
%	& \Pr\{\hat{\nu}(\cS_t^*,\cM_1) < (1-\varepsilon_0) \hat{\nu}(\cS_t^*,\cM_0) \mid \cH_{t-1} \}  \\
%	& = \Pr \left\{\sum_{i=1}^{\theta}X_i^{\cM_1}(\cS_t^*) < (1-\varepsilon_0) \sum_{i=1}^{\theta}X_i^{\cM_0}(\cS_t^*) \right \} \\
%	& \le  \Pr \left\{\sum_{i=1}^{\theta}X_i^{\cM_1}(\cS_t^*) < c_0 \vee
%	\sum_{i=1}^{\theta}X_i^{\cM_0}(\cS_t^*) > c_0 / (1-\varepsilon_0)
%	\right\} \\
%	& \le \Pr \left\{\sum_{i=1}^{\theta}X_i^{\cM_1}(\cS_t^*) < c_0 \right\} + 
%	\Pr \left\{ \sum_{i=1}^{\theta}X_i^{\cM_0}(\cS_t^*) > c_0 / (1-\varepsilon_0)
%	\right\}.
%\end{align*}
%
%
%We want to find some $\gamma > 0$, such that 
%%\[
%%c_0 = (1-\gamma) \theta \E[X_i^{\cM_1}(\cS_t^*) ] \wedge  \frac{c_0}{1-\varepsilon_0} = (1 + \gamma) \theta \E[X_i^{\cM_0}(\cS_t^*) ]
%%\]
%
%\[
%c_0 = (1-\gamma) \theta \E[X_1^{\cM_1}(\cS_t^*) ] \wedge  \frac{c_0}{1-\varepsilon_0} = (1 + \gamma) \theta \E[X_1^{\cM_0}(\cS_t^*) ]
%\]
%
%Let $\mu_0 =  \E[X_1^{\cM_0}(\cS_t^*) ]$, $\mu_1 = \E[X_1^{\cM_1}(\cS_t^*) ] $.
%Then we have
%\[
%\gamma = \frac{\mu_1 - (1-\varepsilon_0) \mu_0}{\mu_1 + (1-\varepsilon_0) \mu_0}.
%\]
%Note that by the inequality derived in Eq.~\eqref{eq:meandiff}, we know that $|\mu_1-\mu_0| \le \eta \mu_0$.
%Together with $\eta < \varepsilon_0$, we have $\gamma > 0$.
%Moreover, since $\mu_1 \ge (1-\eta) \mu_0$, we have
%\[
%\gamma \ge \frac{ \varepsilon_0 - \eta}{2 - \eta -\varepsilon_0} = \gamma_0 > 0.
%\]
%
%%Set $\eta = \varepsilon_0$, $c_0 = (1-\gamma) \theta \E[X_i^{\cM_1}(\cS_t^*) ]$, $\mu_0 =  \E[X_i^{\cM_0}(\cS_t^*) ]$, $\mu_1 = \E[X_i^{\cM_1}(\cS_t^*) ] $, and $\gamma = \frac{\mu_1 - (1-\varepsilon_0) \mu_0}{\mu_1 + (1-\varepsilon_0) \mu_0}$.
%
%We can now apply the martingale inequalities, and obtain
%\begin{align*}
%	& \Pr \left\{\sum_{i=1}^{\theta}X_i^{\cM_1}(\cS_t^*) < c_0 \right\}  \\
%	= &	\Pr\left\{\sum_{i=1}^{\theta}X_i^{\cM_1}(\cS_t^*) -  \theta \E[X_1^{\cM_1}(\cS_t^*) ] < -\gamma \theta \E[X_1^{\cM_1}(\cS_t^*)]\right\} \\
%%	= &	\Pr\left\{\sum_{i=1}^{\theta}X_i^{\cM_1}(\cS_t^*) -  \theta \hat{\nu}(\cS_t^*, M_1)/n ] < -\gamma \hat{\nu}(\cS_t^*, M_1)/n\right\} \\
%	\leq & \exp\left(- \frac{\gamma^2}{2} \cdot \theta \cdot \E[X_1^{\cM_1}(\cS_t^*) ] \right) \\
%	\leq & \exp\left(- \frac{\gamma^2}{2} \cdot \frac{2n \cdot \ln(4/\delta_1)}{(1-\eta)\OPT_t  \cdot \gamma_0^2} \cdot 
%	(1-\eta) \E[X_1^{\cM_0}(\cS_t^*) ] \right) \\
%	\le & \delta_1/4.
%\end{align*}
%The last inequality above uses the fact that $\E[X_1^{\cM_0}(\cS_t^*) ] = \OPT_t /n$ and $\gamma \ge \gamma_0$.
%Similarly, 
%\begin{align*}
%	& \Pr \left\{\sum_{i=1}^{\theta}X_i^{\cM_0}(\cS_t^*) > c_0/(1-\varepsilon_0) \right\}  \\
%	= &	\Pr\left\{\sum_{i=1}^{\theta}X_i^{\cM_0}(\cS_t^*) -  \theta \E[X_i^{\cM_0}(\cS_t^*) ] > \gamma \theta \E[X_i^{\cM_0}(\cS_t^*)]\right\} \\
%%	= &	\Pr\left\{\sum_{i=1}^{\theta}X_i^{\cM_0}(\cS_t^*) -  \theta \hat{\nu}(\cS_t^*, M_0)/n ] > \gamma \hat{\nu}(\cS_t^*, M_0)/n\right\} \\
%	\leq & \exp\left(- \frac{\gamma^2}{2+\frac{2}{3}\gamma} \cdot \theta \cdot \E[X_i^{\cM_0}(\cS_t^*) ] \right) \\
%	\leq & \exp\left(- \frac{\gamma^2}{2+\frac{2}{3}\gamma} \cdot \frac{(2+\frac{2}{3}\gamma_0)n \cdot \ln(4/\delta_1)}{\OPT_t  \cdot \gamma_0^2} \cdot \E[X_i^{\cM_0}(\cS_t^*) ]  \right) \\
%	\le & \delta_1/4.
%\end{align*}
%The last inequality above uses the fact that $\gamma^2 / (2+\frac{2}{3}\gamma)$ is monotonically increasing with $\gamma>0$, so $\gamma^2 / (2+\frac{2}{3}\gamma) \ge \gamma_0^2 / (2+\frac{2}{3}\gamma_0)$.
%\end{proof}
%\wei{The following part should not be in the above proof.
%If we want to do some tuning of the parameters, we can do it at the end and reflect it in the algorithm and
%	the final analysis.
%}
%
%Suppose that $\varepsilon_1$ is a very small number.  Set $\varepsilon_1 = 2\varepsilon_0 + 1$ and $\varepsilon_0 = 7\eta$, and then we have
%\[
%\theta^{(1)} = \frac{50n \cdot \ln(4/\delta_1)}{\OPT_t  \cdot \varepsilon_1^2}.
%\]





\begin{lemma} \label{lem:randhistory2}
	Fix any $\varepsilon_2 >0$ and any $\delta_2 > 0$.
	Suppose  that $\xi(\eta)$ holds for some $\eta < \varepsilon_2$.
	Fix a round $t$ and a history $\cH_{t-1}$ that satisfies $\xi(\eta)$.
	Let $\cM_1$ and $\cM_0$ be the RR sets generated in round $t$ based on root distributions
	$P_{t,1}(\cH_{t-1})$ and $P_{t,0}(\cH_{t-1})$, respectively.
	If we generate at least $\theta^{(2)}$ RR sets in round $t$ as defined below,
	\[
	\theta^{(2)} = \frac{(1+\eta)^2(2-2/e) \cdot n \cdot \ln({\binom{n}{k}}/\delta_2)}{(\varepsilon- (1-1/e)\varepsilon_1)^2\cdot \OPT_t},
	\]
	%	\[
	%	\theta^{(2)} = \max{\left(\frac{(2+\frac{2}{3}\gamma_1)(1-1/e)n \cdot 
	%			\ln \left(\frac{4\binom{n}{k}}{\delta_2} \right)}{(1+\eta)\OPT_t  \cdot \gamma_1^2},  \frac{(2-2/e)n \cdot \ln \left(\frac{4\binom{n}{k}}{\delta_2} \right)}{\OPT_t  \cdot \gamma_1^2}\right)},
	%	\]
	%	where 
	%%	$\mu_0 =  \E[X_1^{\cM_0}(\cS_t) ]$ %$ = \Pr_{v \sim P_{t,0}(\cH_{t-1})}\{ \cS_t \cap \cR_{v,t} \ne \emptyset \}$, 
	%%	$\mu_1 = \E[X_1^{\cM_1}(\cS_t) ] $, and 
	%	$\gamma_1 = \frac{\varepsilon_2 - \eta }{2 + \eta + \varepsilon_2}$,
	then we have
	%	\[
	%	\Pr\{\hat{\nu}(\cS_t,\cM_1) \ge (1+\varepsilon_2) \hat{\nu}(\cS_t,\cM_0) \mid \cH_{t-1} \} \le \frac{\delta_2}{2{\binom{n}{k}}}.
	%	\]
	\[
	\Pr\{\hat{\nu}(\cS_t, \cM_1) \geq (1-\frac{1}{e})(1-\varepsilon_1)\cdot \OPT_t\} \leq \delta_2 / {\binom{n}{k}}.
	\]
	
\end{lemma}
\begin{proof}
	%	Let $\cR_{v,t}$ be a random RR set generated in round $t$ rooted at node $v$.
	%	Since $\xi(\eta)$ holds, we have that for all $v\in V$, 
	%	$| P_{t,1}(\cH_{t-1})(v) -  P_{t,0}(\cH_{t-1})(v)| \le \eta P_{t,0}(\cH_{t-1})(v)$.
	%	Then, we can derive the following:
	%	\begin{align}
	%	&\left |\E[X_1^{\cM_1}(\cS_t)\mid \cH_{t-1}] - \E[X_1^{\cM_0}(\cS_t)\mid \cH_{t-1}]  \right | \nonumber \\
	%	& \quad = \left |\sum_{v\in V} P_{t,1}(\cH_{t-1})(v) \cdot 
	%	\Pr\{ \cR_{v,t} \cap \cS_t \ne \emptyset \} -  \right. \nonumber \\
	%	& \quad \quad \left. \sum_{v\in V} P_{t,0}(\cH_{t-1})(v) \cdot 
	%	\Pr\{ \cR_{v,t} \cap \cS_t \ne \emptyset \} \right | \nonumber \\
	%	& \quad \le  \sum_{v\in V}  \left | P_{t,1}(\cH_{t-1})(v) -  P_{t,0}(\cH_{t-1})(v) \right| \cdot 
	%	\Pr\{ \cR_{v,t} \cap \cS_t \ne \emptyset \}  \nonumber \\
	%	& \quad \le \sum_{v\in V} \eta P_{t,0}(\cH_{t-1})(v)  \cdot 
	%	\Pr\{ \cR_{v,t} \cap \cS_t \ne \emptyset \} \nonumber \\
	%	& = \eta \E[X_1^{\cM_0}(\cS_t) \mid \cH_{t-1} ]. \label{eq:meandiff1}
	%	\end{align}
	
	%	Next, we want to $\Pr\{\hat{\nu}(\cS_t, \cM_1) \geq (1-\frac{1}{e})(1-\varepsilon_1)\cdot \OPT_t\} \leq \delta_2 / {\binom{n}{k}}$.
	%	 $\E[\hat{\nu}(\cS_t, \cM_1)] =  n\E[X_1^{\cM_1}(\cS_t) \mid \cH_{t-1} ] \le (1+\eta)n\E[X_1^{\cM_0}(\cS_t) \mid \cH_{t-1} ] = \E[(1+\eta)\hat{\nu}(\cS_t, \cM_0)]$ by Equation \ref{eq:meandiff1}. Set ${\nu}(\cS_t, \cM_0) < (1-1/e-\varepsilon)OPT_t$ for bad $\cS_t$ under $\varepsilon$ and $\varepsilon_2 = (1+\eta)\varepsilon- (1-1/e)(\varepsilon_1+\eta)$, we have
	
	By Corllary \ref{cor:randiff}, $\E[\hat{\nu}(\cS_t, \cM_1)] \le \E[(1+\eta)\hat{\nu}(\cS_t, \cM_0)]$.
	Set ${\nu}(\cS_t, \cM_0) < (1-1/e-\varepsilon)OPT_t$ for bad $\cS_t$ under $\varepsilon$ and $\varepsilon_2 = (1+\eta)\varepsilon- (1-1/e)(\varepsilon_1+\eta)$, we have
	\begin{align*}
	& \Pr\{\hat{\nu}(\cS_t, \cM_1) \geq (1-\frac{1}{e})(1-\varepsilon_1)\cdot \OPT_t\} \\
	= & \Pr\left\{\sum_{i=1}^{\theta}X_i^{\cM_1}(\cS_t) - \frac{\theta \E[\hat{\nu}(\cS_t, \cM_1)]}{n} \geq \right.\\
	& \qquad \left. \frac{\theta}{n} \cdot \left((1-\frac{1}{e})(1-\varepsilon_1)\cdot \OPT_t -  \E[\hat{\nu}(\cS_t, \cM_1)]\right) \right\}\\
	\le & \Pr\left\{\sum_{i=1}^{\theta}X_i^{\cM_1}(\cS_t) - \frac{\theta \E[\hat{\nu}(\cS_t, \cM_1)]}{n} \geq \right.\\
	& \qquad \left. \frac{\theta}{n} \cdot \left((1-\frac{1}{e})(1-\varepsilon_1)\cdot \OPT_t -  (1+\eta)\hat{\nu}(\cS_t, \cM_0)\right) \right\}\\
	\le & \Pr\left\{\sum_{i=1}^{\theta}X_i^{\cM_1}(\cS_t) - \frac{\theta \E[\hat{\nu}(\cS_t, \cM_1)]}{n} \geq \right.\\
	& \qquad \left. \frac{\theta}{n} \cdot \left((1-\frac{1}{e})(1-\varepsilon_1)\cdot \OPT_t -  (1+\eta)(1-1/e-\varepsilon)OPT_t\right) \right\}\\
	= & \Pr\left\{\sum_{i=1}^{\theta}X_i^{\cM_1}(\cS_t) - \frac{\theta \E[\hat{\nu}(\cS_t, \cM_1)]}{n} \geq \frac{\theta}{n} \cdot\varepsilon_2 OPT_t \right\}\\
	= &	\Pr\left\{\sum_{i=1}^{\theta}X_i^{\cM_1}(\cS_t) - \theta \cdot \frac{\E[\hat{\nu}(\cS_t, \cM_1)]}{n} \geq \right. \\
	& \qquad \left. \frac{\varepsilon_2\cdot \OPT_t}{\E[\hat{\nu}(\cS_t, \cM_1)]} \cdot \theta \cdot \frac{\E[\hat{\nu}(\cS_t, \cM_1)]}{n} \right\} \\
	\leq & \exp\left(- \frac{\left(\varepsilon_2\cdot \frac{\OPT_t}{\E[\hat{\nu}(\cS_t, \cM_1)]}\right)^2}{2+\frac{2}{3}\left(\varepsilon_2\cdot \frac{\OPT_t}{\E[\hat{\nu}(\cS_t, \cM_1)]}\right)} \cdot \theta \cdot \E[\hat{\nu}(\cS_t, \cM_1)] / n \right) \\
	\leq & \exp\left(- \frac{\left(\varepsilon_2\cdot \OPT_t\right)^2}{2\E[\hat{\nu}(\cS_t, \cM_1)]+\frac{2}{3}\left(\varepsilon_2\cdot \OPT_t\right)} \cdot \theta \cdot 1 / n \right) \\
	\leq & \exp\left(- \frac{\left(\varepsilon_2\cdot \OPT_t\right)^2}{2(1+\eta)(1-1/e - \varepsilon) \cdot \OPT_t+\frac{2}{3}\left(\varepsilon_2\cdot \OPT_t\right)} \cdot \theta \cdot 1 / n \right) \\
	\leq & \exp\left(- \frac{((1+\eta)\varepsilon- (1-1/e)(\varepsilon_1+\eta))^2\cdot \OPT_t}{(1+\eta)(2-2/e) \cdot n} \cdot \theta \right) \\
	\leq & \exp\left(- \frac{(\varepsilon- (1-1/e)(\varepsilon_1+\eta)/(1+\eta))^2\cdot \OPT_t}{(2-2/e) \cdot n} \cdot \theta \right) \\
	\leq & \exp\left(- \frac{(\varepsilon- (1-1/e)\varepsilon_1/(1+\eta))^2\cdot \OPT_t}{(2-2/e) \cdot n} \cdot \theta \right) \\
	\leq & \exp\left(- \frac{(\varepsilon- (1-1/e)\varepsilon_1/(1+\eta))^2\cdot \OPT_t}{(2-2/e) \cdot n} \cdot \right.\\
	& \qquad \left. \frac{(1+\eta)^2(2-2/e) \cdot n \cdot \ln({\binom{n}{k}}/\delta_2)}{(\varepsilon- (1-1/e)\varepsilon_1)^2\cdot \OPT_t} \right) \\
	\leq & \delta_2 / {\binom{n}{k}} 
	\end{align*}
	
	
	
\end{proof}
%\begin{proof}
%	Let $\cR_{v,t}$ be a random RR set generated in round $t$ rooted at node $v$.
%	Since $\xi(\eta)$ holds, we have that for all $v\in V$, 
%	$| P_{t,1}(\cH_{t-1})(v) -  P_{t,0}(\cH_{t-1})(v)| \le \eta P_{t,0}(\cH_{t-1})(v)$.
%	Then, we can derive the following:
%	\begin{align}
%	&\left |\E[X_1^{\cM_1}(\cS_t)\mid \cH_{t-1}] - \E[X_1^{\cM_0}(\cS_t)\mid \cH_{t-1}]  \right | \nonumber \\
%	& \quad = \left |\sum_{v\in V} P_{t,1}(\cH_{t-1})(v) \cdot 
%	\Pr\{ \cR_{v,t} \cap \cS_t \ne \emptyset \} -  \right. \nonumber \\
%	& \quad \quad \left. \sum_{v\in V} P_{t,0}(\cH_{t-1})(v) \cdot 
%	\Pr\{ \cR_{v,t} \cap \cS_t \ne \emptyset \} \right | \nonumber \\
%	& \quad \le  \sum_{v\in V}  \left | P_{t,1}(\cH_{t-1})(v) -  P_{t,0}(\cH_{t-1})(v) \right| \cdot 
%	\Pr\{ \cR_{v,t} \cap \cS_t \ne \emptyset \}  \nonumber \\
%	& \quad \le \sum_{v\in V} \eta P_{t,0}(\cH_{t-1})(v)  \cdot 
%	\Pr\{ \cR_{v,t} \cap \cS_t \ne \emptyset \} \nonumber \\
%	& = \eta \E[X_1^{\cM_0}(\cS_t) \mid \cH_{t-1} ]. \label{eq:meandiff1}
%	\end{align}
%	
%	Next, we want to separate the event 
%	$\hat{\nu}(\cS_t,\cM_1) \ge (1+\varepsilon_2) \hat{\nu}(\cS_t,\cM_0) \mid \cH_{t-1}$
%	as two events so that we can apply concentration bounds for each of them.
%	To do so, we want to properly select a parameter $c_1$ as follows:
%	\begin{align*}
%	& \Pr\{\hat{\nu}(\cS_t,\cM_1) \ge (1+\varepsilon_2) \hat{\nu}(\cS_t,\cM_0) \mid \cH_{t-1} \}  \\
%	& = \Pr \left\{\sum_{i=1}^{\theta}X_i^{\cM_1}(\cS_t) \ge (1+\varepsilon_2) \sum_{i=1}^{\theta}X_i^{\cM_0}(\cS_t) \right \} \\
%	& \le  \Pr \left\{\sum_{i=1}^{\theta}X_i^{\cM_1}(\cS_t) \ge c_1 \vee
%	\sum_{i=1}^{\theta}X_i^{\cM_0}(\cS_t) \le c_1 / (1+\varepsilon_2)
%	\right\} \\
%	& \le \Pr \left\{\sum_{i=1}^{\theta}X_i^{\cM_1}(\cS_t) \ge c_1 \right\} + 
%	\Pr \left\{ \sum_{i=1}^{\theta}X_i^{\cM_0}(\cS_t) \le c_1 / (1+\varepsilon_2)
%	\right\}.
%	\end{align*}
%	
%	We want to find some $\gamma' > 0$, such that 
%	%\[
%	%c_0 = (1-\gamma') \theta \E[X_i^{\cM_1}(\cS_t) ] \wedge  \frac{c_0}{1+\varepsilon_2} = (1 + \gamma') \theta \E[X_i^{\cM_0}(\cS_t) ]
%	%\]
%	
%	\[
%	c_1 = (1+\gamma') \theta \E[X_1^{\cM_1}(\cS_t) ] \wedge  \frac{c_1}{1+\varepsilon_2} = (1 - \gamma') \theta \E[X_1^{\cM_0}(\cS_t) ]
%	\]
%	
%	Let $\mu_0 =  \E[X_1^{\cM_0}(\cS_t) ]$, $\mu_1 = \E[X_1^{\cM_1}(\cS_t) ] $.
%	Then we have
%	\[
%	\gamma' = \frac{(1+\varepsilon_2)\mu_0 -  \mu_1}{(1+\varepsilon_2)\mu_0 +  \mu_1}.
%	\]
%	Note that by the inequality derived in Eq.~\eqref{eq:meandiff1}, we know that $|\mu_1-\mu_0| \le \eta \mu_0$.
%	Together with $\eta < \varepsilon_2$, we have $\gamma' > 0$.
%	Moreover, since $\mu_1 \le (1+\eta) \mu_0$, we have
%	\[
%\gamma' \ge \frac{\varepsilon_2 - \eta}{2 + \varepsilon_2 + \eta } = \gamma_1 > 0.
%	\]
%%	Due to $\gamma > 0$, we have $(1 + \varepsilon_2)(1-\eta) - 1$, and then $\varepsilon_2 > \frac{\eta}{1-\eta}  > \eta$.
%	%Set $\eta = \varepsilon_2$, $c_0 = (1-\gamma') \theta \E[X_i^{\cM_1}(\cS_t) ]$, $\mu_0 =  \E[X_i^{\cM_0}(\cS_t) ]$, $\mu_1 = \E[X_i^{\cM_1}(\cS_t) ] $, and $\gamma' = \frac{\mu_1 - (1-\varepsilon_2) \mu_0}{\mu_1 + (1-\varepsilon_2) \mu_0}$.
%	
%	We can now apply the martingale inequalities, and obtain
%	\begin{align*}
%	& \Pr \left\{\sum_{i=1}^{\theta}X_i^{\cM_1}(\cS_t) \ge c_0 \right\}  \\
%	= &	\Pr\left\{\sum_{i=1}^{\theta}X_i^{\cM_1}(\cS_t) -  \theta \E[X_1^{\cM_1}(\cS_t) ] \ge \gamma' \theta \E[X_1^{\cM_1}(\cS_t)]\right\} \\
%	%	= &	\Pr\left\{\sum_{i=1}^{\theta}X_i^{\cM_1}(\cS_t) -  \theta \hat{\nu}(\cS_t, M_1)/n ] < -\gamma' \hat{\nu}(\cS_t, M_1)/n\right\} \\
%	\leq & \exp\left(- \frac{\gamma'^2}{2+\frac{2}{3}\gamma'} \cdot \theta \cdot \E[X_1^{\cM_1}(\cS_t) ] \right) \\
%	\leq & \exp\left(- \frac{\gamma'^2}{2+\frac{2}{3}\gamma'} \cdot \frac{(2+\frac{2}{3}\gamma_1)(1-1/e)n \cdot \ln(4\binom{n}{k}/\delta_2)}{(1+\eta)\OPT_t  \cdot \gamma_1^2} \cdot 
%	(1+\eta) \E[X_1^{\cM_0}(\cS_t) ] \right) \\
%	& = \delta_2/(4\binom{n}{k}).
%	\end{align*}
%\wei{Why does the above use $1+\eta$? Should it be $1-\eta$?}
%
%	The last inequality above uses the fact that $\E[X_1^{\cM_0}(\cS_t) ] = \OPT_t /n$.
%	
%	\wei{The above statement is wrong. The fix does not look easy. We may need to use the assumption that
%		$\cS_t$ is bad, and redo the analysis.}
%	
%	Let $\varepsilon_2 = \varepsilon - (1-1/e) \varepsilon_1/2$. Let a $\cS_t$ is bad under $\varepsilon$, thus $\hat{\nu}(\cS_t,\cM_0) < (1-1/e-\varepsilon) \cdot \OPT_t$.
%	Similarly, 
%	\begin{align*}
%	& \Pr \left\{\sum_{i=1}^{\theta}X_i^{\cM_0}(\cS_t) \le c_0/(1-\varepsilon_2) \right\}  \\
%	= &	\Pr\left\{\sum_{i=1}^{\theta}X_i^{\cM_0}(\cS_t) -  \theta \E[X_i^{\cM_0}(\cS_t) ] \le -\gamma' \theta \E[X_i^{\cM_0}(\cS_t)]\right\} \\
%	%	= &	\Pr\left\{\sum_{i=1}^{\theta}X_i^{\cM_0}(\cS_t) -  \theta \hat{\nu}(\cS_t, M_0)/n ] > \gamma' \hat{\nu}(\cS_t, M_0)/n\right\} \\
%	\leq & \exp\left(- \frac{\gamma'^2}{2} \cdot \theta \cdot \E[X_i^{\cM_0}(\cS_t) ] \right) \\
%	\leq & \exp\left(- \frac{\gamma'^2}{2} \cdot \frac{2(1-1/e)n \cdot \ln(4\binom{n}{k}/\delta_2)}{\OPT_t  \cdot \gamma_1^2} \cdot \E[X_i^{\cM_0}(\cS_t) ]  \right) \\
%	& = \delta_2/(4{\binom{n}{k}}).
%	\end{align*}
%	
%Suppose that $\varepsilon_1$ is a very small number.  Set $\varepsilon_1 = 2\varepsilon_0 + 1$ and $\varepsilon_0 = 7\eta$, and then we have
%\[
%\theta^{(2)} = \frac{50(1-1/e)n \cdot \ln(4\binom{n}{k}/\delta_2)}{\OPT_t  \cdot \varepsilon_1^2}.
%\]
%
%	
%\end{proof}

%\begin{lemma} \label{lem:wrrnum}
%	Assume a set $\cM_0 = \{\cR_1, \cR_2, \ldots, \cR_{\theta}\}$ satisfies the martingale condition,
%	and $X_i^{\cM_0}(\cS_t) = \I\{\cR_i \cap \cS_t \ne \emptyset \}$.	For any $\varepsilon > 0$, $\varepsilon_1 \in (0, (1-\frac{1}{e}) \cdot \varepsilon)$, and any $\delta_1, \delta_2 > 0$,
%	let
%	\begin{align*}
%	\theta^{(3)} = \frac{8 n \cdot \ln(2/\delta_1)}{\OPT_t \cdot \varepsilon_1^2},
%%	\theta^{(4)} = \frac{(2-2/e)\cdot  n \cdot \ln(2\binom{n}{k}/\delta_2)}{\OPT_t \cdot (\varepsilon - (1-\frac{1}{e})\varepsilon_1/2)^2}. \nonumber
%	\end{align*}
%	If $\theta \geq \theta^{(3)}$, $\Pr\{\hat{\nu}(\cS_t^*, \cM_0) \geq (1-\varepsilon_1)\cdot \OPT_t\} \geq 1 - \delta_1/2$;
%%	If $\theta \geq \theta^{(4)}$, for any bad $\cS_t$ under $\varepsilon$, $\Pr\{\hat{\nu}(\cS_t, \cM_0) \geq (1-\frac{1}{e})(1-\varepsilon_1/2)\cdot \OPT_t\} \leq \delta_2 / (2{\binom{n}{k}})$;
%\end{lemma}
%
%\begin{proof}
%	\begin{align*}
%	& \Pr\{\hat{\nu}(\cS_t^*,\cM_0) < (1-\varepsilon_1/2)\cdot \OPT_t\} \\
%	= &	\Pr\left\{n \cdot \frac{\sum_{i=1}^{\theta}X_i^{\cM_0}(\cS_t^*)}{\theta} < (1-\varepsilon_1/2)\cdot \nu(\cS_t^*)\right\} \\
%	= &	\Pr\left\{\sum_{i=1}^{\theta}X_i^{\cM_0}(\cS_t^*) - \theta \cdot \nu(\cS_t^*) / n< 
%	- \frac{\varepsilon_1}{2} \left(\theta \cdot\nu(\cS_t^*)/n\right) \right\} \\
%	\leq & \exp\left(- \frac{\varepsilon_1^2}{8} \cdot \theta \cdot \nu(\cS_t^*) / n \right) \\
%	\leq & \exp\left(- \frac{\varepsilon_1^2}{8} \cdot \frac{8n \cdot \ln(2/\delta_1)}{\OPT_t \cdot \varepsilon_1^2} \cdot \frac{\nu(\cS_t^*)}{n} \right) = \delta_1/2.
%	\end{align*}
%	
%%Let $\varepsilon_2 = \varepsilon - (1-1/e) \varepsilon_1/2$. Let a $\cS_t$ is bad under $\varepsilon$, thus $\hat{\nu}(\cS_t,\cM_0) < (1-1/e-\varepsilon) \cdot \OPT_t$.
%%Then, we have
%%	\begin{align*}
%%	& \Pr\left\{\hat{\nu}(\cS_t,\cM_0) \geq (1-1/e)(1-\varepsilon_1/2)\cdot \OPT_t\right\} \\
%%	= &	\Pr\left\{\sum_{i=1}^{\theta}X_i^{\cM_0}(\cS_t) - \frac{\theta \cdot \hat{\nu}(\cS_t,\cM_0)}{n} \geq \right.\\ & \qquad \left. \frac{\theta}{n} \cdot \left( (1-\frac{1}{e})(1-\varepsilon_1/2)\cdot \OPT_t- \hat{\nu}(\cS_t,\cM_0)\right) \right\} \\
%%	\leq &	\Pr\left\{\sum_{i=1}^{\theta}X_i^{\cM_0}(\cS_t) - \theta \cdot \frac{\hat{\nu}(\cS_t,\cM_0)}{n} \geq \frac{\theta}{n} \cdot \varepsilon_2 \cdot OPT_t \right\} \\
%%	= &	\Pr\left\{\sum_{i=1}^{\theta}X_i^{\cM_0}(\cS_t) - \theta \cdot \frac{\hat{\nu}(\cS_t,\cM_0)}{n} \geq \frac{\varepsilon_2\cdot \OPT_t}{\hat{\nu}(\cS_t,\cM_0)} \cdot \theta \cdot \frac{\hat{\nu}(\cS_t,\cM_0)}{n} \right\} \\
%%	\leq & \exp\left(- \frac{\left(\varepsilon_2\cdot \frac{\OPT_t}{\hat{\nu}(\cS_t, \cM_0)}\right)^2}{2+\frac{2}{3}\left(\varepsilon_2\cdot \frac{\OPT_t}{\hat{\nu}(\cS_t, \cM_0)}\right)} \cdot \theta \cdot \hat{\nu}(\cS_t, \cM_0) / n \right) \\
%%	\leq & \exp\left(- \frac{\left(\varepsilon_2\cdot \OPT_t\right)^2}{2\hat{\nu}(\cS_t, \cM_0)+\frac{2}{3}\left(\varepsilon_2\cdot \OPT_t\right)} \cdot \theta \cdot 1 / n \right) \\
%%	\leq & \exp\left(- \frac{\left(\varepsilon_2\cdot \OPT_t\right)^2}{2(1-1/e - \varepsilon) \cdot \OPT_t+\frac{2}{3}\left(\varepsilon_2\cdot \OPT_t\right)} \cdot \theta \cdot 1 / n \right) \\
%%	\leq & \exp\left(- \frac{(\varepsilon - (1-1/e) \varepsilon_1/2)^2\cdot \OPT_t}{(2-2/e) \cdot n} \cdot \theta \right) \\
%%	\leq & \exp\left(- \frac{(\varepsilon - (1-1/e) \varepsilon_1/2)^2\cdot \OPT_t}{(2-2/e) \cdot n} \cdot \frac{(2-2/e) \cdot n \cdot \ln({2\binom{n}{k}}/\delta_2)}{\OPT_t \cdot (\varepsilon - (1-1/e)\varepsilon_1/2)^2} \right) \\
%%	= & \delta_2/(2{\binom{n}{k}}).
%%	\end{align*}	
%\end{proof}

\begin{lemma} \label{lem:wrrnum1}
	Assume a set $\cM_1 = \{\cR_1, \cR_2, \ldots, \cR_{\theta}\}$ satisfies the martingale condition.
	For any $\varepsilon > 0$, $\varepsilon_1 \in (0, (1-\frac{1}{e}) \cdot \varepsilon)$, and any $\delta_1, \delta_2 > 0$,
	let \wei{Need to fix the parameters $\varepsilon_0$, $\varepsilon_2$, $\eta$}
	%	\begin{align*}
	%		\theta^{(5)} = \theta^{(1)} + \theta^{(3)}, \nonumber
	%		\theta^{(6)} = \theta^{(2)} + \theta^{(4)} \nonumber
	%	\end{align*}
	
	If $\theta \geq \theta^{(1)}$, $\Pr\{\hat{\nu}(\cS_t^*, \cM_1) \geq (1-\varepsilon_1)\cdot \OPT_t\} \geq 1 - \delta_1$;
	If $\theta \geq \theta^{(2)}$, for any bad $\cS_t$ under $\varepsilon$, $\Pr\{\hat{\nu}(\cS_t, \cM_1) \geq (1-\frac{1}{e})(1+\varepsilon_1)\cdot \OPT_t\} \leq \delta_2 / {\binom{n}{k}}$.
\end{lemma}

\begin{proof}
	%	Comparing to cross-round algorithm, we need to show four different $\theta$ of within-round algorithm for satisifiying all the assumptions and conditions.
	
	Since $\cM_1$ satisfies the martingale condition, by using Corollary \ref{cor:ineq}, set $\varepsilon_0 \le \frac{\varepsilon_1}{2- \varepsilon_1}$, then $1-\varepsilon_1 < (1-\varepsilon_0)(1-\varepsilon_1/2)$ and we have
	\begin{align*}
	\Pr \{ \hat{\nu}(\cS_t^*,\cM_1) < (1-\varepsilon_1)\cdot \OPT_t \}  \le \delta_1,
	\end{align*}
	%	\begin{align*}
	%	& \Pr \{ \hat{\nu}(\cS_t^*,\cM_1) < (1-\varepsilon_1)\cdot \OPT_t \} \\
	%	& \le \Pr \{ \hat{\nu}(\cS_t^*,\cM_1) < (1-\varepsilon_0)(1-\varepsilon_1/2)\cdot \OPT_t \} \\
	%	& \le \Pr\{\hat{\nu}(\cS_t^*,\cM_1) < (1-\varepsilon_0) \hat{\nu}(\cS_t^*,\cM_0) \, \vee \\
	%	& \qquad 
	%		 \hat{\nu}(\cS_t^*,\cM_0) <  (1-\varepsilon_1/2)\cdot \OPT_t\} \\
	%	& \le \Pr\{\hat{\nu}(\cS_t^*,\cM_1) < (1-\varepsilon_0) \hat{\nu}(\cS_t^*,\cM_0) \} + \\
	%	& \quad \Pr\{ \hat{\nu}(\cS_t^*,\cM_0) <  (1-\varepsilon_1/2)\cdot \OPT_t \} \\
	%	& \le \frac{\delta_1}{2} + \frac{\delta_1}{2} = \delta_1,
	%	\end{align*}
	where the last inequality is by Lemmas \ref{lem:randhistory}, %and~\ref{lem:wrrnum}.
	%
	%We want $\Pr\{\hat{\nu}(\cS_t^*,\cM_1) < (1-\varepsilon_0) \hat{\nu}(\cS_t^*,\cM_0) \} \le \delta_1/2$.
	%which is proved in Lemma \ref{lem:randhistory} and $\Pr\{\hat{\nu}(\cS_t^*,\cM_0) < (1-\varepsilon_1/2) OPT_t \} \le \delta_1/2$. which is proved in Lemma \ref{lem:wrrnum}.\\
	%Set $\varepsilon_2 \le  \frac{\varepsilon_1}{2- \varepsilon_1}$, then $1+\varepsilon_1 > (1+\varepsilon_2)(1-\varepsilon_1/2)$ and 
	and we also have
	\begin{align*}
	& \Pr \{ \hat{\nu}(\cS_t,\cM_1) \ge (1-1/e)(1-\varepsilon_1)\cdot \OPT_t \}  \le \frac{\delta_2}{{\binom{n}{k}}},
	\end{align*}
	%	\begin{align*}
	%	& \Pr \{ \hat{\nu}(\cS_t,\cM_1) \ge (1-1/e)(1+\varepsilon_1)\cdot \OPT_t \} \\
	%	& \le \Pr \{ \hat{\nu}(\cS_t,\cM_1) \ge (1-1/e)(1+\varepsilon_2)(1-\varepsilon_1/2)\cdot \OPT_t \} \\
	%	& \le \Pr\{\hat{\nu}(\cS_t,\cM_1) \ge (1+\varepsilon_2) \hat{\nu}(\cS_t,\cM_0) \vee \\
	%	 & \quad
	%	\hat{\nu}(\cS_t,\cM_0) \ge  (1-1/e)(1-\varepsilon_1/2)\cdot \OPT_t\} \\
	%	& \le \Pr\{\hat{\nu}(\cS_t,\cM_1) \ge (1+\varepsilon_2) \hat{\nu}(\cS_t,\cM_0) \} + \\
	%	& \quad \Pr\{ \hat{\nu}(\cS_t,\cM_0) \ge  (1-1/e)(1-\varepsilon_1/2)\cdot \OPT_t \} \\
	%	& \le \frac{\delta_2}{2{\binom{n}{k}}} + \frac{\delta_2}{2{\binom{n}{k}}} = \frac{\delta_2}{{\binom{n}{k}}},
	%	\end{align*}
	where the last inequality is by Lemmas \ref{lem:randhistory2}.% and~\ref{lem:wrrnum}
	%
	%We want $\Pr\{\hat{\nu}(\cS_t,\cM_1) \ge (1-\varepsilon_2) \hat{\nu}(\cS_t,\cM_0) \} \le \delta_2/(2{\binom{n}{k}})$.
	%which is proved in Lemma \ref{lem:randhistory2} and $\Pr\{\hat{\nu}(\cS_t,\cM_0) \ge (1-1/e)(1-\varepsilon_1/2) \cdot OPT_t \} \le \delta_2/(2{\binom{n}{k}})$.
	%which is proved in Lemma \ref{lem:wrrnum}.\\
	%----
	%
	%	
\end{proof}


%\begin{lemma} \label{lem:wrrnum}
%	Assume a set $\cM = {\cR_1, \cR_2, \ldots, \cR_{\theta}}$ satisfies the martingale condition.
%	For any $\varepsilon, \varepsilon_0 > 0$, $1/2 \varepsilon_0  = \varepsilon_1 \in (0, (1-\frac{1}{e}) \varepsilon)$, and any $\delta_0,\delta_1, \delta_2 > 0$,
%	let
%	\begin{align*}
%	& \theta^{(0)} = \frac{2 n \cdot \ln(1/\delta_0)}{\OPT_t \cdot \varepsilon_1^2}, 
%	\theta^{(1)} = \frac{2 n \cdot \ln(1/\delta_1)}{\OPT_t \cdot \varepsilon_1^2}, \\
%	& \theta^{(-1)} = \frac{2 n \cdot \ln(1/\delta_1)}{\OPT_t \cdot \varepsilon_1^2},
%	\theta^{(2)} = \frac{(2-2/e)\cdot  n \cdot \ln(\binom{n}{k}/\delta_2)}{\OPT_t \cdot (\varepsilon - (1-\frac{1}{e})\varepsilon_1)^2}. \nonumber
%	\end{align*}
%	If $\theta \geq \theta^{(0)}$, $\Pr\{\hat{\nu}'(S_t^*) \geq (1-\varepsilon_0)\cdot \hat{\nu}(S_t^*)\} \geq 1 - \delta_0$;
%	If $\theta \geq \theta^{(1)}$, $\Pr\{\hat{\nu}(S_t^*) \geq (1-\varepsilon_1)\cdot \OPT_t\} \geq 1 - \delta_1$;
%	If $\theta \geq \theta^{(-1)}$, $\Pr\{\hat{\nu}(S_t^*) \leq (1+\varepsilon_1)\cdot \OPT_t\} \geq 1 - \delta_1$;
%	If $\theta \geq \theta^{(2)}$, for any bad $S_t$ under $\varepsilon$, $\Pr\{\hat{\nu}(S_t) \geq (1-\frac{1}{e})(1-\varepsilon_1)\cdot \OPT_t\} \leq \delta_2 / {\binom{n}{k}}$;
%\end{lemma}
%
%\begin{proof}
%	Comparing to cross-round algorithm, we need to show four different $\theta$ of within-round algorithm for satisifiying all the assumptions and conditions.
%	
%	Since $\cM$ satisfies the martingale condition, by using Corollary \ref{cor:ineq}, we have
%	\begin{align*}
%		& \Pr\{\hat{\nu}(S_t^*,\cR) < (1-\varepsilon_1)\cdot \OPT_t\} \\
%		= &	\Pr\left\{n \cdot \frac{\sum_{i=1}^{\theta}X_i^{\cM}(S_t^*)}{\theta} < (1-\varepsilon_1)\cdot \nu(S_t^*)\right\} \\
%		= &	\Pr\left\{\sum_{i=1}^{\theta}X_i^{\cM}(S_t^*) - \theta \cdot \nu(S_t^*) / n< - \varepsilon_1 \left(\theta \cdot\nu(S_t^*)/n\right) \right\} \\
%		\leq & \exp\left(- \frac{\varepsilon_1^2}{2} \cdot \theta \cdot \nu(S_t^*) / n \right) \\
%		\leq & \exp\left(- \frac{\varepsilon_1^2}{2} \cdot \frac{2n \cdot \ln(1/\delta_1)}{\OPT_t \cdot \varepsilon_1^2} \cdot \frac{\nu(S_t^*)}{n} \right) = \delta_1.
%	\end{align*}
%	Let $\varepsilon_2 = \varepsilon - (1-1/e) \varepsilon_1$. Let a $S_t$ is bad under $\varepsilon$, thus $\nu(S) < (1-1/e - \varepsilon) \cdot \OPT_t$.
%	Then, we have
%	\begin{align*}
%		& \Pr\left\{\hat{\nu}(S_t,\cR) \geq (1-1/e)(1-\varepsilon_1)\cdot \OPT_t\right\} \\
%		= &	\Pr\left\{\sum_{i=1}^{\theta}X_i^{\cM}(S_t) - \theta \cdot \nu(S_t)/n \geq \theta/n \cdot \left( (1-1/e)(1-\varepsilon_1)\cdot \OPT_t- \nu(S_t)\right) \right\} \\
%		\leq &	\Pr\left\{\sum_{i=1}^{\theta}X_i^{\cM}(S_t) - \theta \cdot \nu(S_t)/n \geq \theta/n \cdot \varepsilon_2 \cdot \nu(S_t) \right\} \\
%		= &	\Pr\left\{\sum_{i=1}^{\theta}X_i^{\cM}(S_t) - \theta \cdot \nu(S_t)/n \geq (\varepsilon_2\cdot \OPT_t/\nu(S_t)) \cdot \theta \cdot \nu(S_t)/n \right\} \\
%		\leq & \exp\left(- \frac{\left(\varepsilon_2\cdot \frac{\OPT_t}{\nu(S_t)}\right)^2}{2+\frac{2}{3}\left(\varepsilon_2\cdot \frac{\OPT_t}{\nu(S_t)}\right)} \cdot \theta \cdot \nu(S_t) / n \right) \\
%		\leq & \exp\left(- \frac{\left(\varepsilon_2\cdot \OPT_t\right)^2}{2\nu(S_t)+\frac{2}{3}\left(\varepsilon_2\cdot \OPT_t\right)} \cdot \theta \cdot 1 / n \right) \\
%		\leq & \exp\left(- \frac{\left(\varepsilon_2\cdot \OPT_t\right)^2}{2((1-1/e) - \varepsilon) \cdot \OPT_t+\frac{2}{3}\left(\varepsilon_2\cdot \OPT_t\right)} \cdot \theta \cdot 1 / n \right) \\
%		\leq & \exp\left(- \frac{(\varepsilon - (1-1/e) \varepsilon_1)^2\cdot \OPT_t}{n} \cdot \theta \right) \\
%		\leq & \exp\left(- \frac{(\varepsilon - (1-1/e) \varepsilon_1)^2\cdot \OPT_t}{n} \cdot \frac{n \cdot \ln({\binom{n}{k}}/\delta_2)}{\OPT_t \cdot (\varepsilon - (1-1/e)\varepsilon_1)^2} \right) = \delta_2/{\binom{n}{k}}.
%	\end{align*}
%
%	Let $\varepsilon' = \varepsilon_0 - \varepsilon_1 + \varepsilon_0 \cdot \varepsilon_1$, with at least $1 - \delta_1$ probability,
%	we have
%	\begin{align*}
%		& \Pr\{\hat{\nu}'(S_t^*)  > (1+\varepsilon_1)\cdot \hat{\nu}(S_t^*)\} \\
%		= &	\Pr\left\{n \cdot \frac{\sum_{i=1}^{\theta}X_i^{\cM}(S_t^*)}{\theta} > (1-\varepsilon_0)\cdot (1+\varepsilon_1)\cdot \nu(S_t^*)\right\} \\
%		= &	\Pr\left\{n \cdot \frac{\sum_{i=1}^{\theta}X_i^{\cM}(S_t^*)}{\theta} > (1-\varepsilon')\cdot \nu(S_t^*)\right\} \\
%		= &	\Pr\left\{\sum_{i=1}^{\theta}X_i^{\cM}(S_t^*) -  \theta \cdot \nu(S_t^*)/n > - \varepsilon' \left( \theta \cdot\nu(S_t^*)/n\right) \right\} \\
%		\leq & \exp\left(- \frac{\varepsilon'^2}{2+\frac{2}{3}\varepsilon'} \cdot \theta \cdot \nu(S^*_t) / n \right) \\
%		\leq & \exp\left(- \frac{{\varepsilon'}^2}{2+\frac{2}{3}\varepsilon' } \cdot \frac{2n \cdot \ln(1/\delta_1)}{\OPT_t \cdot \varepsilon'^2} \cdot \nu(S^*_t) / n \right) = \delta_1.
%	\end{align*}
%	
%	With at least $1-\delta_1$ probability, we have
%	\begin{align*}
%		& \Pr\{\hat{\nu}'(S_t^*)   < (1-\varepsilon_0)\cdot \hat{\nu}(S_t^*)\} \\
%		= & \Pr\{\hat{\nu}'(S_t^*)  < (1-\varepsilon_0)\cdot (1-\varepsilon_1)\cdot \nu(S_t^*)\} \\
%		= &	\Pr\left\{n \cdot \frac{\sum_{i=1}^{\theta}X_i^{\cM}(S_t^*)}{\theta} < (1-\varepsilon_0)\cdot (1+\varepsilon_1)\cdot \nu(S_t^*)\right\} \\
%		= &	\Pr\left\{n \cdot \frac{\sum_{i=1}^{\theta}X_i^{\cM}(S_t^*)}{\theta} < (1-\varepsilon')\cdot \nu(S_t^*)\right\} \\
%		= &	\Pr\left\{\sum_{i=1}^{\theta}X_i^{\cM}(S_t^*) - \theta \cdot \nu(S_t^*)/n< - \varepsilon' \left( \theta \cdot\nu(S_t^*)/n\right) \right\} \\
%		\leq & \exp\left(- \frac{{\varepsilon'}^2}{2} \cdot \theta \cdot \nu(S_t^*) / n \right) \\
%		\leq & \exp\left(- \frac{{\varepsilon'}^2}{2} \cdot \frac{2n \cdot \ln(1/\delta_0)}{\OPT_t \cdot {\varepsilon'}^2} \cdot \frac{\nu(S_t^*)}{n} \right) = \delta_0.
%	\end{align*}
%
%	$\theta^{(1)}, \theta^{(2)}$ are the same as \alg{IMM} algorithm.
%%	\begin{align*}
%%		& \Pr\{\hat{\rho}(S^*) < (1-\varepsilon_1)\cdot \OPT_t\} \\
%%		= &	\Pr\left\{n \cdot \frac{\sum_{i=1}^{\theta}X_i^{\cM}(\cS^*)}{\theta} < (1-\varepsilon_1)\cdot \rho(\cS^*)\right\} \\
%%		= &	\Pr\left\{\sum_{i=1}^{\theta}X_i^{\cM}(\cS^*) - \theta \cdot \rho(\cS^*)< - \varepsilon_1 \left(\theta \cdot\rho(\cS^*)/n\right) \right\} \\
%%		\leq & \exp\left(- \frac{\varepsilon_1^2}{2} \cdot \rho(\cS^*) / n \right) \\
%%		\leq & \exp\left(- \frac{\varepsilon_1^2}{2} \cdot \frac{2n \cdot \ln(1/\delta_1)}{\OPT_t \cdot \varepsilon_1^2} \cdot \frac{\rho(\cS^*)}{n} \right) = \delta_1.
%%	\end{align*}
%%	Let $\varepsilon_2 = \varepsilon - (1-\frac{1}{e}) \varepsilon_1$. Let a $\cS$ is bad under $\varepsilon$, thus $\rho(S) < ((1-\frac{1}{e}) - \varepsilon) \cdot \OPT_t$.
%%	Then, we have
%%	\begin{align*}
%%		& \Pr\left\{\hat{\rho}(S) \geq (1-\frac{1}{e})(1-\varepsilon_1)\cdot \OPT_t\right\} \\
%%		= &	\Pr\left\{\sum_{i=1}^{\theta}X_i^{\cM}(\cS) - \theta \cdot \rho(\cS) \geq \theta/n \cdot \left( (1-\frac{1}{e})(1-\varepsilon_1)\cdot \OPT_t- \rho(\cS)\right) \right\} \\
%%		\leq &	\Pr\left\{\sum_{i=1}^{\theta}X_i^{\cM}(\cS) - \theta \cdot \rho(\cS) \geq \theta/n \cdot \varepsilon_2 \cdot \rho(\cS) \right\} \\
%%		= &	\Pr\left\{\sum_{i=1}^{\theta}X_i^{\cM}(\cS) - \theta \cdot \rho(\cS) \geq (\varepsilon_2\cdot \OPT_t/\rho(\cS)) \cdot \theta \cdot \rho(\cS)/n \right\} \\
%%		\leq & \exp\left(- \frac{\left(\varepsilon_2\cdot \frac{\OPT_t}{\rho(\cS)}\right)^2}{2+\frac{2}{3}\left(\varepsilon_2\cdot \frac{\OPT_t}{\rho(\cS)}\right)} \cdot \theta \cdot \rho(\cS) / n \right) \\
%%		\leq & \exp\left(- \frac{\left(\varepsilon_2\cdot \OPT_t\right)^2}{2\rho(\cS)+\frac{2}{3}\left(\varepsilon_2\cdot \OPT_t\right)} \cdot \theta \cdot 1 / n \right) \\
%%		\leq & \exp\left(- \frac{\left(\varepsilon_2\cdot \OPT_t\right)^2}{2((1-\frac{1}{e}) - \varepsilon) \cdot \OPT_t+\frac{2}{3}\left(\varepsilon_2\cdot \OPT_t\right)} \cdot \theta \cdot 1 / n \right) \\
%%		\leq & \exp\left(- \frac{(\varepsilon - (1-\frac{1}{e}) \varepsilon_1)^2\cdot \OPT_t}{n} \cdot \theta \right) \\
%%		\leq & \exp\left(- \frac{(\varepsilon - (1-\frac{1}{e}) \varepsilon_1)^2\cdot \OPT_t}{n} \cdot \frac{n \cdot \ln({\binom{n}{k}}/\delta_2)}{\OPT_t \cdot (\varepsilon - (1-\frac{1}{e})\varepsilon_1)^2} \right) = \delta_2/{\binom{n}{k}}.
%%	\end{align*}
%\end{proof}

\begin{corollary} \label{wcor:alphabeta}
	Assume $\cM$ satisfies the martingale condition. We set the parameters $\delta_0 = \delta_1 = \delta_2 = 1/(6Tn^\ell)$, and $\varepsilon_1 = \varepsilon \cdot \frac{\alpha}{(1-\frac{1}{e})\alpha+\beta}$ in Lemma \ref{lem:wrrnum}, where
	\begin{equation}
	\alpha = \sqrt{l \ln{n}+ \ln{6} + \ln{T}}, \beta = \sqrt{\left(1-\frac{1}{e}\right) \cdot \left(\ln\left(\binom{n}{m}\right)+ \alpha^2 \right)} \nonumber.
	\end{equation}
	While $\theta \geq \frac{2n\cdot ((1-\frac{1}{e})\alpha + \beta)^2}{\OPT_t \cdot \varepsilon^2}$, the \alg{\WRIMM} returns $((1-\frac{1}{e}) - \varepsilon)$-approximate solution with at least $1- 1 / (2n^\ell)$ probability.
\end{corollary}

\begin{proof}
	While $\delta_0 = \delta_1 = \delta_2 = 1/(6Tn^\ell)$, we set the $\theta^{(0)} = \theta^{(1)} =  \theta^{(-1)} = \theta^{(2)}$ in Lemma \ref{lem:wrrnum},
	then we can find
	$\theta^{(5)} = \theta^{(6)} = \frac{2n\cdot ((1-\frac{1}{e})\alpha + \beta)^2}{\OPT \cdot \varepsilon^2}$, while $\varepsilon_1 = \varepsilon \cdot \frac{\alpha}{(1-\frac{1}{e})\alpha+\beta}$ by calculation.
\end{proof}

\begin{lemma}(Correctness)\label{lem:wrcorrectness}
	For any $\varepsilon > 0$, $\ell > 0$, the output $\cS^o$ of the cross-round algorithm $\alg{\WRIMM}$ is $( 1 - e^(1-1/e) - \varepsilon)$-approximate solution with at least $1-\frac{1}{n^\ell}$ probability.
\end{lemma}	

\begin{proof}
	In each round, by using Lemma \ref{lem:lb} but replacing influence function $\upsilon(\cdot)$ proves that $LB \leq \OPT$ with at least $1 - \frac{1}{2n^\ell}$ probability. In this case, we have $\theta \geq \frac{2n((1-1/e)\cdot \alpha+\beta)^2}{\OPT\cdot \varepsilon^2}$. Lemma \ref{lem:crmatingale} proves the multi-round RR sets $\cM$ satisfies the martingale condition in each round. By using Colloary \ref{cor:alphabeta}, while $\theta \geq  \frac{2n((1-1/e)\cdot \alpha+\beta)^2}{\OPT\cdot \varepsilon^2}$, the within-round node selection \alg{\WRNS} returns a $(1-1/e-\varepsilon)$-approximate solution in each round. Overall, \alg{\WRIMM} returns $(1 - e^{(1 - 1/e - \varepsilon)} -\varepsilon_1)$-approximate solution $\hat{\cS}^g$ with at least $1 - \frac{1}{n^\ell}$ probability for $T$ rounds.
\end{proof}

\begin{lemma}(Time Complexity) \label{lem:wrtimecomplexity}
	While $k < n$, for any $\varepsilon, l > 0$, the total execution time of the \alg{\WRIMM} is $O(T(k+l)(m+n)\log{(Tn)}/\varepsilon^2).$
\end{lemma}

\begin{proof}
	By Lemma \ref{lem:wrrtime}, it shows that the time execution is $O(kn + \sum_{\cR \in \cM} |\cR|)$ for each iteration in any round as same as standard \alg{IMM}. 
	Due to total $T$ round and the maximum number of iteration in each round is $\log_2{n} =1$ in \alg{\WRIMM},
	the total execution time is $O(Tkn\log{n} + T \cdot \sum_{\cR \in \cM} |M|) = O(Tkn\log{n} + T\cdot (\E[\theta] \cdot(EPT_t+1)))$, where $EPT$ is the expectation time of multi-round RR set.
	
	By using the new $\alpha, \beta$ and new $\theta$, we recalucalte
	\begin{equation}
	\E[\theta] = O\left(\frac{(k + l) n \log{(Tn)}}{\OPT \cdot \varepsilon^2}\right) \nonumber.
	\end{equation} 
	
	The $EPT_t$ also can be estimated by a random node $\tilde{v}$ under history condition $ \cH_{t-1}$,
	\begin{equation}
	EPT_t = \frac{m}{n} \cdot \E_{\tilde{v}}[\nu(\tilde{v})] \nonumber.
	\end{equation}
	
	Due to $\E_{\tilde{v}}[\nu(\tilde{v})] \leq \OPT$, the total execution time is
	\begin{align*}
	&O(Tkn\log{n} + T \cdot (\E[\theta] \cdot(EPT_t+1))) \\
	= & O\left(Tkn\log{n} + \frac{T(k + l) n \log{(Tn)}}{\OPT \cdot \varepsilon^2} \cdot ( \frac{m}{n} \cdot \E_{\tilde{v}}[\nu(\tilde{v})] + 1)\right) \\
	= &  O\left(\frac{T(k+l)(m+n)\log{(Tn)}}{\varepsilon^2}\right).
	\end{align*}
\end{proof}

%\wrimmt*
%\begin{proof}
%	Let $\varepsilon_1 = e^{(1-1/e)} \varepsilon/2$, by Lemma \ref{lem:wrcorrectness}, we prove the correctness of the within-round algorithm \alg{\WRIMM}
%	that the output will hold $(1 - 1/e -\varepsilon)$-approximate solution to multi-round influence maximization.
%	By Lemma \ref{lem:wrtimecomplexity}, we show the time complexity of the algorithm \alg{\WRIMM} is $O\left(\frac{T(k+l)(m+n)\log{(Tn)}}{\varepsilon^2}\right)$.
%	Thus, the theorem holds.
%\end{proof}
%\begin{proof}[Proof (Sketch)]
%	Let $\varepsilon_1 = e^{(1-1/e)} \varepsilon/2$, 
%	$\ell' = \ell + \log (2T) / \log n $.
%	As explained already, one round \alg{\WRIMM} is essentially the same as \alg{IMM}
%	with parameters $\varepsilon_1$ and $\ell'$.
%	Thus, following the result in~\cite{tang15}, we know that for each round $t$,
%	with probability at least $ 1 - 2/n^{\ell'} = 1 - 1/(n^\ell T)$, 
%	output $S_t$ is a $(1 - 1/e - \varepsilon_1)$ approximation of the
%	best seed set for this round.
%	Then following the similar arguments as in Theorem~\ref{thm:nonadaptive},
%	we know that across all $T$ rounds, 
%	with probability at least $1 - 1/n^\ell$,
%	\begin{align*}
%	\rho(\cS^o)  &\geq \left(1 - e^{-(1-\frac{1}{e} - \varepsilon_1)}\right)\rho(\cS^*) \\
%	& \ge \left(1 - e^{-(1-\frac{1}{e})}-\varepsilon \right)\rho(\cS^*).
%	\end{align*}
%	Thus, the theorem holds.
%\end{proof}

%\adaimm*

%\begin{proof}
%	\begin{align}
%	& \E[\I\{ S\cap R^{-A_{i-1}} \ne \emptyset \}]  \nonumber \\
%	& = \sum_{v\in V\setminus A_{i-1}} \Pr\{v =\rroot(R^{-A_{i-1}}) \} \cdot \nonumber \\
%	& \quad \quad \E[\I\{ S\cap R^{-A_{i-1}} \ne \emptyset \} \mid v =\rroot(R^{-A_{i-1}})] 
%	\nonumber \\
%	& = \frac{1}{n-|A_{i-1}|} \sum_{v\in V\setminus A_{i-1}} 
%	\E[\I\{ S\cap R_v^{-A_{i-1}} \ne \emptyset \} ] \nonumber  \\
%	& = \frac{1}{n-|A_{i-1}|} \sum_{v\in V\setminus A_{i-1}} 
%	\E[\I\{ v\in \Gamma(L, S)\} ] \label{eq:RRset2L} \allowdisplaybreaks \\
%	& = \frac{1}{n-|A_{i-1}|} \E \left[ \sum_{v\in V\setminus A_{i-1}} \I\{ v\in \Gamma(L, S)\} \right] \nonumber \\
%	& = \frac{1}{n-|A_{i-1}|} \E[|\Gamma(L, S) \setminus A_{i-1} | ] \nonumber \\
%	& =  \frac{1}{n-|A_{i-1}|} \sigma^{-A_{i-1}}(S), \nonumber 
%	\end{align}
%	where Eq.~\eqref{eq:RRset2L} is based on the equivalence between RR sets and live-edge graphs,
%	and the expectation from this point on is taken over the random live-edge graphs $L$. 
%\end{proof}

%\adaimmt*
%\begin{proof}[Proof (Sketch)]
%	Let $\varepsilon_1 = e^{(1-1/e)} \varepsilon/2$, 
%	$\ell' = \ell + \log (2T) / \log n $.
%	As explained already, one round \alg{AdaIMM} is essentially the same as \alg{IMM}
%	with parameters $\varepsilon_1$ and $\ell'$.
%	Thus, following the result in~\cite{tang15}, we know that for each round $i$,
%	with probability at least $ 1 - 2/n^{\ell'} = 1 - 1/(n^\ell T)$, 
%	output $S_i$ is a $(1 - 1/e - \varepsilon_1)$ approximation of the
%	best seed set for this round.
%	Then following the similar arguments as in Theorems~\ref{thm:nonadaptive} and~\ref{thm:AdaGreedy},
%	we know that across all $T$ rounds, 
%	with probability at least $1 - 1/n^\ell$,
%	\begin{align*}
%	f_{\avg}(\pi^{\ai}) &  \geq \left(1 - e^{-(1-\frac{1}{e} - \varepsilon_1)}\right) f_{\avg}(\pi^*)\\
%	& \ge \left(1 - e^{-(1-\frac{1}{e})}-\varepsilon \right) f_{\avg}(\pi^*).
%	\end{align*}
%	Thus, the theorem holds.
%\end{proof}
